Simple, Fast, and Scalable Reachability Oracle

A reachability oracle (or hop labeling) assigns each vertex v two sets of vertices: Lout(v) and Lin(v), such that u reaches v iff Lout(u) \cap Lin(v) \neq \emptyset. Despite their simplicity and elegance, reachability oracles have failed to achieve efficiency in more than ten years since their introduction: the main problem is high construction cost, which stems from a set-cover framework and the need to materialize transitive closure. In this paper, we present two simple and efficient labeling algorithms, Hierarchical-Labeling and Distribution-Labeling, which can work onmassive real-world graphs: their construction time is an order of magnitude faster than the setcover based labeling approach, and transitive closure materialization is not needed. On large graphs, their index sizes and their query performance can now beat the state-of-the-art transitive closure compression and online search approaches.

==> Algorithm.tex <==
\section{Constructing Forests}
\label{algorithm}



==> Backbone.tex <==
\vspace*{-2.0ex}
\section{Reachability Backbone Definition}
\label{backbone}

In this section, we  formally define the reachability backbone which plays a central role in SCARAB for scaling the reachability computation. 
Intuitively,  it is designed to have a number of desired features: 
%1) the reachability backbone has be able to scale-down the original graphs so that the existing reachability index can be applied;
1) it should be much smaller than the original graph;
2) it should carry sufficient topological information to assist the reachability computation in the original graph; 
3) it should be easy to access for any vertex in the original graph. 
To satisfy these features, SCARAB explicitly separates {\em local} vertex pairs from {\em non-local} vertex pairs, and focuses on utilizing the backbone for recovering the reachability for non-local reachable pairs.  
For local pairs,
reachability can be computed directly online, so no global information is needed.
%no global topological information is needed to recover their reachability and can be dealt locally. 
Furthermore, the separation between {\em local} and {\em non-local} vertex pairs is determined through a threshold parameter $\epsilon$ which can be used not only to facilitate the access of backbone vertices, but also to help control the backbone size. 

Formally,  given a {\em locality threshold} $\epsilon$, for any pair of vertices $u$ and $v$, if $u$ can reach $v$ within $\epsilon$ intermediate vertices, i.e., the distance between from $u$ to $v$ is no \rw{longer}{greater} than $\epsilon$, then $(u,v)$ is referred to as a {\bf local pair}, and if $u$ can reach $v$ but through at least $\epsilon+1$ intermediate vertices, i.e., their distance is \rw{longer}{greater} than $\epsilon$, then $(u,v)$ is referred to as a {\bf non-local pair}. 
If $u$ cannot reach $v$, then, $(u,v)$ is referred to as a {\bf unreachable} pair. 
Given this, the reachability backbone is defined as follows: 

\bdefin({\bf Reachability Backbone}) 
\label{def:backbone}
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, a reachability backbone $G^\ast=(V^\ast,E^\ast)$, where $V^\ast \subseteq V$ and $E^\ast$ may contain edges not in $E$, has the following property: 
 for any non-local ({\em unreachable}) pair $(u,v)$ in graph $G$, there must ({\em not}) exist two vertices $u^\ast$ and $v^\ast$ in $V^\ast$, such that $(u,u^\ast)$ and $(v^\ast,v)$ are both local pairs in $G$ and $u^\ast$ can reach $v^\ast$ in $G^\ast$. 
\edefin

\begin{figure}
\centering
\begin{tabular}{c c}
\psfig{figure=Figures/RunningExample.eps,width=1.6in, height=2in} & \raisebox{0.5in}{\psfig{figure=Figures/GateGraph.eps,width=0.8in, height=0.8in}}  \\ 
(a) Original Graph $G$  & (b) $G$'s Reachability Backbone
\end {tabular}
\vspace*{-2.0ex}
\caption{Running Example}
\label{fig:runningexamples}
\vspace*{-3.0ex}
\end{figure}

\begin{example}
Figure~\ref{fig:runningexamples}(b) shows a reachability backbone of graph $G$ (Figure~\ref{fig:runningexamples}(a)) with $\epsilon=2$. 
As an example, for non-local vertex pair $(1,18)$, there is a backbone vertex $3$ where vertex $1$ reaches $3$ in 
one hop, there is another backbone vertex $10$ where vertex $10$ reaches $18$ in two hops, and vertex $3$ reaches $10$ in the reachability backbone. Indeed, for any non-local vertex pair in Figure~\ref{fig:runningexamples}(a), you can find their corresponding local backbone vertices and they are connected in the reachability backbone (Figure~\ref{fig:runningexamples}(b)). On the other hand, if two vertices cannot reach one another, no additional connection in the backbone will make them reachable from one to another. In other words, there are no false positives for reachability using the \rw{gate graph}{reachability backbone}.  
\end{example}

Clearly, the reachability backbone depends on the locality threshold $\epsilon$. As we will show in the empirical study Section~\ref{expr}, for any real and synthetic graphs, a reachability backbone with $\epsilon \leq 4$ can already significantly reduce the size of the original graph $G$ by an order of magnitude. More surprisingly, for almost all the real graphs which are publicly available for reachability study~\cite{Wang06,DBLP:conf/edbt/ChengYLWY08,DBLP:conf/sigmod/JinXRF09,yildirim:grail}, the reachability backbone even for $\epsilon=2$ can
\rw{achieve a reduction rate  ranging from one to two orders of magnitudes in terms of number of vertices.}
{reduce the number of vertices by one to two orders of magnitude.}
The detailed study on the selection of the locality threshold $\epsilon$ is discussed in Section~\ref{expr}. 

\noindent{\bf Reachability Backbone Edge Set:}
Given a DAG $G=(V,E)$ and its reachability backbone $G^\ast=(V^\ast,E^\ast)$, 
let $TC(V^\ast)$ be the transitive closure of $G$ on $V^\ast$, i.e., $TC(V^\ast)=\{(u^\ast,v^\ast) \in V^\ast \times V^\ast | u^\ast \rightarrow v^\ast \mbox{ in } $G$\}$. 
Furthermore, let $TC^\ast(V^\ast)$ be the {\bf transitive reduction}~\cite{AhoGU72} of $TC(V^\ast)$, i.e., $TC^\ast(V^\ast)$ contains the smallest edge set which preserve all reachability information between any two vertices in $V^\ast$. 
Given this, we make the following observation of the edge set $E^\ast$ in the reachability backbone: 

\blemma({\bf Backbone Edge Set}) 
\label{lemma:backboneedge}
Given any reachability backbone $G^\ast=(V^\ast,E^\ast)$ for $G=(V,E)$, $E^\ast \subseteq TC(V^\ast)$. 
In other words, $E^\ast$ does not introduce any additional reachability information beyond those between any two vertices of $V^\ast$ in the original graph $G$. 
Furthermore, ${\bf G^\ast}=(V^\ast,TC^\ast(V^\ast))$ is also a  reachability backbone of $G$, where $TC^\ast(V^\ast)$ is referred to as the {\em canonical} backbone edge set of the backbone vertex set $V^\ast$. 
\elemma

Clearly, if there is any additional reachability is introduced, then there is will be false positives. This violates the backbone definition. The complete proof of Lemma~\ref{lemma:backboneedge} is omitted due to space limitation.  Lemma~\ref{lemma:backboneedge} has the following important implication. 

\begin{corollary}
For any candidate reachability backbone graph $G^\ast=(V^\ast,E^\ast)$ in a given graph $G$, where $V^\ast \subseteq V$ and $E^\ast \subseteq TC(V^\ast)$, for any unreachable pair $(u,v)$ in $G$, it will remain unreachable using $G^\ast$. 
\end{corollary}
This is because no additional reachability information is added in $E^\ast$ besides those in the original graph $G$, i.e., $E^\ast \subseteq TC(V^\ast)$. 
Thus, we only need to focus on recovering the reachability for the non-local pairs in the original graph using the reachability backbone and do not have to deal with the non-reachable pairs. 
To facilitate our discussion, in the reminder of the paper,  any {\em valid} backbone edge set $E^\ast$ satisfies $TC^\ast(V^\ast)\subseteq E^\ast \subseteq TC(V^\ast)$. 

\begin{example}
In Figure~\ref{fig:runningexamples}(b), the edge set of the reachability backbone is a valid backbone edge set for the backbone vertex set $\{3,8$, $10,12,16\}$. However, it is not a canonical backbone edge set. 
If we remove the redundant edges ($(8,10)$ and $(8,12)$), then the resulting edge set is a canonical one as any further edge removal will disconnect some reachability pair in the original graph. Note since the transitive reduction of a given graph is unique~\cite{AhoGU72}, the {\em canonical} backbone edge set  is also unique.
\end{example}


\comment{
Lemma~\ref{lemma:backboneedge} suggests that any backbone edge set which is below the transitive reduction ($ E^\ast \subset TC^\ast(V^\ast)$) can always be expanded to become $TC^\ast(V^\ast)$, and thus without loss of generality, we can always assume the backbone edge set $E^\ast$ lies between the canonical edge set and the transitive closure ($TC^\ast(V^\ast) \subseteq E^\ast \subseteq TC(V^\ast)$). 
For simplicity, for any backbone vertex set, we can always choose its corresponding canonical backbone edge set $TC^\ast(V^\ast)$. }

%Given this, we have the following 




\noindent{\bf Minimal Reachability Backbone (MBR):}  
Since  the reachability backbone $G^\ast$ aims to scale-down the original graph $G$, its size should be as small as possible while still maintaining its property for reachability computation. 
%%Obvious%% Note by by definition, any graph is its own reachability backbone. But in this case, there is no reduction of the graph. 
Given this, we introduce the {\bf minimal reachability backbone} discovery problem: {\em given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, the minimal reachability backbone is the one with the smallest number of backbone vertices, i.e., $\arg\min_{|V^\ast|} G^\ast$. }
Since any reachability backbone edge set $E^\ast$ satisfies $E^\ast \subseteq TC(V^\ast)$, then, we can first discover the backbone vertex set $V^\ast$ on the graph $G$ without defining its edge set $E^\ast$. 
Once the backbone vertex set is discovered, we can always choose $E^\ast=TC^\ast(V^\ast)$ as the default edge set, which can be immediately computed. 
Thus, the MRB problem can be reformulated as follows: 

\bdefin({\bf Minimal Reachability Backbone Vertex Set (MRBVS) Discovery})
\label{def:backbonevertex}
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$,  we would like to find the {\em minimal} backbone vertex set $V^\ast \subseteq V$ such that for any non-local pair $(u,v)$ in graph $G$, there must exist two vertices $u^\ast$ and $v^\ast$ in $V^\ast$, such that $(u,u^\ast)$ and $(v^\ast,v)$ are both local pairs in $G$ and $u^\ast$ can reach $v^\ast$ in $G$. 
\edefin

%Given this, in the rest of the section, we focus on discovering the minimal reachability backbone vertex set (MRBVS). 
However, computing MRBVS is NP-hard.  

\bthm({\bf NP-hardness of MRBVS discovery problem})
\label{NPhardness}
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, computing its minimal backbone vertex set is NP-hard. 
\ethm 

We reduce the classical NP-hard problem, set-cover problem (SCP), to this problem and the proof can be found in Appendix. 




==> Backbone1.tex <==
\section{Reachability Backbone Definition}
\label{backbone}


% in Subsection~\ref{definition}, and then we discuss how to discover the reachability backbone in Subsection~\ref{backbonediscovery}. 

%\subsection{Reachability Backbone Definition}
%\label{definition}

In this section, we  formally define the reachability backbone which plays a center role in SCARAB for scaling the reachability computation. 
Intuitively,  it is designed to  a number of desired features: 
1)  first, the reachability backbone has be able to scale-down the original graphs so that the existing reachability index can be applied; 
2)  second, it has to carry sufficient topological information to help the reachability computation in the original graph; 
3)  third,  it should be easy to access for any vertex in the original graph. 
To satisfy these features, SCARAB explicitly separates the {\em local} vertex pair and {\em non-local} vertex pair, and focuses on utilizing the backbone for recovering the reachability for the non-local reachable pairs.  
For the local pairs, no global topological information is needed to recover their reachability and can be dealt locally. 
Furthermore, the separation measure between {\em local} and {\em non-local} vertex pairs is determined through a threshold parameter $\epsilon$ which can be used not only to facilitate the access of backbone vertices, but also to help control the backbone size. 

Formally,  given a {\em locality threshold} $\epsilon$, for any pair of vertices $u$ and $v$, if $u$ can reach $v$ within $\epsilon$ intermediate vertices, i.e., the distance between from $u$ to $v$ is no longer than $\epsilon$, then $(u,v)$ is referred to as a {\bf local pair}, and if $u$ can reach $v$ but through at least $\epsilon+1$ intermediate vertices, i.e., their distance is longer than $\epsilon$, then $(u,v)$ is referred to as a {\bf non-local pair}. 
If $u$ can not reach $v$, then, $(u,v)$ is referred to as a {\bf unreachable} pair. 
Given this, the reachability backbone is defined as follows: 

\bdefin({\bf Reachability Backbone}) 
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, a reachability backbone $G^\ast=(V^\ast,E^\ast)$, where $V^\ast \subseteq V$ and $E^\ast$ may contain edges not in $E$, has the following property: 
 for any non-local ({\em unreachable}) pair $(u,v)$ in graph $G$, there must ({\em not}) exist two vertices $u^\ast$ and $v^\ast$ in $V^\ast$, such that $(u,u^\ast)$ and $(v^\ast,v)$ are both local pairs in $G$ and $u^\ast$ can reach $v^\ast$ in $G^\ast$. 
\edefin

\begin{figure}
\centering
\begin{tabular}{c c}
\psfig{figure=Figures/RunningExample.eps,width=1.6in, height=2in} & \raisebox{0.5in}{\psfig{figure=Figures/GateGraph.eps,width=0.8in, height=0.8in}}  \\ 
(a) Original Graph $G$  & (b) $G$'s Reachability Backbone
\end {tabular}
\caption{Running Example}
\label{fig:runningexamples}
\end{figure}

Figure~\ref{fig:runningexamples} shows a reachability backbone of graph $G$ when $\epsilon=2$. 
As an example, for non-local vertex pair $(1,5)$, there is a backbone vertex $3$ where vertex $1$ reaches $3$ in 2 hops and there is another backbone vertex $4$ where vertex $4$ reaches $5$ in one hop, and vertex $3$ reaches $1$ in the reachability backbone. Indeed, for any non-local vertex pair in the Figure~\ref{fig:runningexamples}, you can find their corresponding local backbone vertices and they are connected in the reachability backbone (Figure~\ref{fig:backbonegraph}). On another hand, if two vertices cannot reach one another, no additional connection in the backbone will make them reachable from one to another. In other words, there is no false positives for reachability using the gate graph.  


Clearly, the reachability backbone depends on the locality threshold $\epsilon$. As we will show in the empirical study Section~\ref{expr}, for any real and synthetic graphs, a reachability backbone with $\epsilon \leq 4$ can already significantly reduce the size of the original graph $G$ by an order of magnitude. More surprisingly, for almost all the real graphs which are public available for reachability study~\cite{Wang06,DBLP:conf/edbt/ChengYLWY08,Jin:2009,yildirim:grail}, the reachability backbone even for $\epsilon=2$ can achieve a reduction rate  ranging from one to two orders of magnitudes in terms of number of vertices. The detailed study on the selection of the locality threshold $\epsilon$ is discussed in Section~\ref{expr}. 

\noindent{\bf Reachability Backbone Edge Set:}
Given a DAG $G=(V,E)$ and its reachability backbone $G^\ast=(V^\ast,E^\ast)$, 
let $TC(V^\ast)$ be the transitive closure of $G$ on $V^\ast$, i.e.,$TC(V^\ast)=\{(u^\ast,v^\ast) \in V^\ast \times V^\ast | u^\ast \rightarrow v^\ast \mbox{ in } $G$\}$. 
Furthermore, let $TC^\ast(V^\ast)$ be the {\bf transitive reduction}~\cite{AhoGU72} of $TC(V^\ast)$, i.e., $TC^\ast(V^\ast)$ contains the smallest edge set which preserve all reachability information between any two vertices in $V^\ast$. 
Given this, we make the following observation of the edge set $E^\ast$ in the reachability backbone: 

\blemma({\bf Canonical Backbone Edge Set}) 
\label{lemma:backboneedge}
Given any reachability backbone $G^\ast=(V^\ast,E^\ast)$ for $G=(V,E)$, $E^\ast \subseteq TC(V^\ast)$. 
In other words, $E^\ast$ do not introduce any additional reachability information beyond those between any two vertices of $V^\ast$ in the original graph $G$. 
Furthermore, ${\bf G^\ast}=(V^\ast,TC^\ast(V^\ast))$ is also a  reachability backbone of $G$, where $TC^\ast(V^\ast)$ is referred to as the {\bf canonical} backbone edge set of the backbone vertex set $V^\ast$. 
\elemma

The proof of Lemma~\ref{lemma:backboneedge} is in Appendix. 
Note that the edge set of the reachability backbone in Figure~\ref{fig:backbonegraph} is not a canonical backbone edge set of the backbone vertex set $\{3,8$, $9,10,5\}$. But any edge in Figure~\ref{fig:runningexample} (b)  corresponds a reachability pair in the original graph (Figure~\ref{fig:runningexample} (a)). If we the redundant edges ($(8,10)$ and $(8,12)$), then the resulting edge set is a canonical one as any further edge removal will disconnect some reachability pair in the original graph. Note since the transitive reduction of a given graph is unique~\cite{AhoGU72}, the {\bf canonical} backbone edge set  is also unique.

\comment{
Lemma~\ref{lemma:backboneedge} suggests that any backbone edge set which is below the transitive reduction ($ E^\ast \subset TC^\ast(V^\ast)$) can always be expanded to become $TC^\ast(V^\ast)$, and thus without loss of generality, we can always assume the backbone edge set $E^\ast$ lies between the canonical edge set and the transitive closure ($TC^\ast(V^\ast) \subseteq E^\ast \subseteq TC(V^\ast)$). 
For simplicity, for any backbone vertex set, we can always choose its corresponding canonical backbone edge set $TC^\ast(V^\ast)$. }

%Given this, we have the following 
Lemma~\ref{lemma:backboneedge} has the following important implication: 
{\em For any candidate reachability backbone graph $G^\ast=(V^\ast,E^\ast)$ in a given graph $G$, where $V^\ast \subseteq V$ and $E^\ast \subseteq TC(V^\ast)$, for any unreachable pair $(u,v)$ in $G$, it will remain to be unreachable using $G^\ast$}. This is because no additional reachability information is added in $E^\ast$ besides those in the original graph $G$, i.e., $E^\ast \subseteq TC(V^\ast)$. 
Thus, in the reminder of the paper, we only need to focus on recovering the reachability for the non-local pairs in the original graph using the reachability backbone. 

\noindent{\bf Minimal Reachability Backbone:}  
Since  the reachability backbone $G^\ast$ aims to scale-down the original graph $G$, its size should be as small as possible while still maintaining its property for reachability computation. 
Note by by definition, any graph is its own reachability backbone. But in this case, there is no reduction of the graph. 
Given this, we introduce the {\bf minimal reachability backbone} discovery problem: {\em given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, the minimal reachability backbone is the one with the smallest number of backbone vertices, i.e., $\arg\min_{|V^\ast|} G^\ast$. }
Since any reachability backbone edge set $E^\ast$ satisfy $E^\ast \subseteq TC(V^\ast)$, then, we can directly discover the backbone vertex set $V^\ast$ on the graph graph $G$ and  the MRB problem can be easily transformed into the following problem: 
%Since only the canonical backbone edge set is considered, 

\bdefin({\bf Minimal Reachability Backbone Vertex Set (MRBVS) Discovery})
\label{def:backbonevertex}
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$,  we would like to find the {\em minimal} backbone vertex set $V^\ast \subseteq V$ such that for any non-local pair $(u,v)$ in graph $G$, there must exist two vertices $u^\ast$ and $v^\ast$ in $V^\ast$, such that $(u,u^\ast)$ and $(v^\ast,v)$ are both local pairs in $G$ and $u^\ast$ can reach $v^\ast$ in $G$. 
\edefin

%Note that because we consider only the canonical reachability backbone edge set, the backbone vertex set can be directly %defined on top of the original graph $G$. 

Once the backbone vertex set is discovered, we can always choose $E^\ast=TC^\ast(V^\ast)$ as the default edge set, which can be immediately computed. Given this, in the rest of the section, we focus on discovering the minimal reachability backbone vertex set (MRBVS). 
Before we proceed, we note that computing MRBVS is a NP-hard problem. 

\bthm({\bf NP-hardness of MRBVS discovery problem})
\label{NPhardness}
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, computing its minimal backbone vertex set is NP-hard. 
\ethm 
We reduce the classical NP-hard problem, set-cover problem, to this problem and the proof can be found in Appendix. 

\section{Reachability Backbone Discovery}
\label{backbonediscovery}

Since discovering the minimal backbone vertex set (MRBVS) is NP-hard, we cannot expect to find a exact solution in polynomial time. 
Furthermore, based on Definition~\ref{def:backbonever}), the direct verification on whether a vertex subset in $V$ meets the backbone criterion is computationally expensive: the reachability for any non-local pair and any unreachable pair has to be explicitly verified. 
To deal with this problem, we consider a {\em local meeting criterion} in finding reachability backbone vertex set and then we utilize it to discover MRBVS. 

%Interestingly, such verification can be significantly reduced and the simplified criterion also leads to an efficient and scalable approach which can approximate the cardinality of MRBVS with guaranteed bound. 
%\noindent{\bf Local Criterion for Reachability Backbone Vertex Set:} 
%In the following, we describe a simplified criterion for the reachability backbone vertex set. 

\subsection{Minimal Reachability Backbone Vertex Set with Local Meeting Criterion}

We first make the following important observation: 
\blemma({\bf Local Meeting Criterion}) 
\label{important}
Given a DAG $G=(V,E)$ and a subset of vertices $V^\ast$, if $V^\ast$ satisfy the following {\em local meeting criterion}: for any vertex pair $(u,v)$ in $G$ where $u$ can reach  $v$ in $\epsilon+1$ hops, i.e., $d(u,v)=\epsilon+1$, there exists a vertex $x \in V^\prime$, such that $u$ can reach $x$ and $x$ can reach $v$ both within $\epsilon$ hops, i.e., $d(u,x)\leq\epsilon$ and $d(x,v)\leq\epsilon$, then $V^\ast$ is a reachability backbone vertex set. 
\elemma
%Since any vertex subset $V^\ast$ in the original graph $G$ will not introduce any additional reachability information, it can automatically reject any unreachable $(u,v)$ pair. 
%Given this, we only need to consider for any non-local pair $(u,v)$, we can discover $(u,u^\ast)$ and $(v^\ast,v)$, where $u^\ast \in V^\ast$, $v^\ast \in V^\ast$, $d(u,u^\ast)\leq \epsilon$, $d(v^\ast,v) \leq \epsilon$, and $u^\ast$ can reach $v^\ast$ in $G$. 
\bproof 
Clearly, when $d(u,v)=\epsilon+1$, the case is trivial and $u^\ast$=$v^\ast$=$x$.
Now, let $d(u,v)>\epsilon+1$. In that case, there is a vertex $w$ such that $d(u,w)=\epsilon+1$ and $w\rightarrow v$.
Based on the postulate, we can find a vertex $x\in V^\ast$ such that $d(u,x)\leq\epsilon$ and $d(x,w)\leq\epsilon$. 
Let $u^\ast=x$. 
If $d(x,v) \leq d$, then $v^\ast=x$. 
Otherwise, we can find $w^\prime$, such that $d(w^\prime,v)=\epsilon+1$ and $x \rightarrow w^\prime$. 
Based on the postulate, we can find a vertex $y \in V^\ast$ such that $d(w^\prime,y) \leq \epsilon$ and $d(y,v) \leq \epsilon$. 
There we have $v^\ast=y$. 
To sum, for any non-local pair $(u,v)$, we can find $u^\ast$ and $v^\ast$ in $V^\ast$, such that $d(u,u^\ast) \leq \epsilon$, $d(v^\ast,v) \leq \epsilon$, and $u^\ast \rightarrow v^\ast$. 
\eproof

Note that in the running example (Figure~\ref{fig:runningexample}), the vertex set $\{3,8,10,12,16\}$ actually satisfies the local meeting criterion.  
However, not every reachability backbone vertex set has to satisfy the local meeting criterion. 
For instance, consider graph $G$ contains two sets of vertices $A$ and $B$, and any vertex pair $(a,b)$ ($a \in A$ and $b \in B$, and $d(a,b)=\epsilon+1$), and these pairs are linked by vertex-disjoint paths (with length $\epsilon+1$) and any two paths can only meet at the ends. Clearly, $A\cup B$  backbone vertex set can be a reachability backbone vertex set (assuming there is no other vertices besides $A$, $B$ and intermediate vertices in the paths linking these two sets). 
Clearly, the local meeting criterion is much easier to manage and it also provides a good collection of backbone vertex sets to choose. Especially, we observe the simple bound: 
\blemma
Let $V^\ast_\epsilon$ be the minimal reachability backbone vertex set which satisfies the local meeting criterion with respect to the locality threshold $\epsilon$ and $V^\ast$ be  the overall minimal reachability backbone vertex set (not necessarily satisfying the local meeting criterion) with respect to the locality threshold $\epsilon$, then, $|V^\ast_\epsilon| \geq |V^\ast| \geq |V^\ast_{\epsilon+1}|$. 
\elemma
\bproof
It is easily to verify that any  reachability backbone vertex set (not  necessarily satisfying the local meeting criterion) the locality threshold $\epsilon$ is always a reachability backbone vertex set which satisfies the local meeting criterion with respect to the locality threshold $\epsilon+1$. 
Together with Lemma~\ref{important}, the bound holds. 
\eproof

Furthermore, in Section~\ref{expr}, we observe empirically $|V^\ast_\epsilon|/|V^\ast_{\epsilon+1}|$ is fairly small. 
Thus, $V^\ast_\epsilon$ can provide a good approximation of $V^\ast$. 
Formally, the problem of discovering the minimal reachability backbone vertex set with the local meeting criterion is referred to as the {\bf LMRBVS discovery} problem and we will focus on this problem for minimal reachability backbone vertex discovery. 

\bthm({\bf NP-hardness of LMRBVS discovery problem})
\label{NPhardnessL}
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, computing its minimal backbone vertex set which satisfies the local meeting criterion is NP-hard. 
\ethm 

Theorem~\ref{NPhardnessL} can be proved similarly as the proof of Theorem~\ref{NPhardness} and is thus omitted for simplicity. 
Though the LMRBVS discovery problem is still NP-hard, it does admit a fast approximation algorithm based on the set-cover framework. 

\subsection{A Fast Set-Cover Based Approach}
Based on the local meeting criterion, we make the following two observations:
1) each non-local vertex pair $(u,v)$ with distance $d(u,v)=\epsilon+1$ needs to be ``covered'', i.e., there is $x\in V^\ast$, such that $u \rightarrow x \rightarrow v$, and $d(u,x)\leq \epsilon$ and $d(x,v) \leq \epsilon$; 
2) any vertex $x \in V$ in the original graph can ``cover'' a list of non-local vertex pair $(u,v)$ with distance $d(u,v)=\epsilon+1$ which is centered around $x$. 
Specifically, any $(u,v)$ such that $u \rightarrow x \rightarrow v$, and $d(u,x)\leq \epsilon$ and $d(x,v) \leq \epsilon$ can be covered by $x$. 
Our goal is thus to select a minimal number of vertices which can cover all the non-local vertex pair $(u,v)$ with distance $d(u,v)=\epsilon+1$. 
 
\begin{figure}
\centering
\begin{tabular}{c c c}
\psfig{figure=Figures/Bipartite6.eps,width=0.8in, height=1.2in} & 
\psfig{figure=Figures/Bipartite10.eps,width=0.8in, height=1.2in} & 
\psfig{figure=Figures/MNfor6.eps,width=1.5in, height=1.2in} \\ 
(a) $C_6$  & (b) $C_{10}$ & (c) $N_\epsilon(6)$ and $N^\prime_\epsilon(6)$. 
\end {tabular}
\caption{Bipartite Graph Representation for Candidate Sets ($\epsilon=2$) and its Generation}
\label{fig:bipartitecandidate}
\end{figure}

Given this, we observe the  LMRBVS discovery problem can be directly coded as an instance of the set cover problem~\cite{Feige98}: 
Given DAG $G=(V,E)$ and the locality parameter $\epsilon$, let $\mathcal{U}=\{(u,v) | d(u,v) = \epsilon+1\}$ be the ground set, which includes all the non-local pairs with distance equal to $\epsilon+1$.
Each vertex $x$ in the graph is associated with a set of vertex pairs $C_x=\{(u,v) | d(u,x) \le \epsilon, d(x,v)\le \epsilon, d(u,v)=\epsilon+1\}$,
where $C_x$ includes all of the non-local pairs with distance equal to $\epsilon+1$, and $u$ can reach $x$ and $x$ can reach $v$ both within $\epsilon$ hops.  
Thus, we have a total of $|V|$ candidate sets $\mathcal{C}=\{C_x|x \in V\}$. 
Figure~\ref{fig:bipartitecandidate} shows the candidate sets of vertex $6$ and $10$ for the graph in Figure~\ref{fig:runningexample}(a). Here, each directed edge in the bipartite graph corresponds to a non-local pair with distance $3$ for locality parameter $\epsilon=2$. 
Now, in order to discover the LMRBVS, we seek the {\em a subset of vertices $V^\ast \subseteq V$, which has the minimal cardinality,  to cover the ground set, i.e., $\mathcal{U} = \bigcup_{v \in V^\ast} C_v$. }
Basically, $V^\ast$ serves as the index for the selected candidate sets to cover the ground set.

For this set cover instance, we may apply the classical greedy algorithm to find the minimal set cover, which essentially correspond to the LMRBVS: 
{\em
Let $R$ be the covered non-local pairs with distance $\epsilon+1$ (initially, $R=\emptyset$).
For each candidate set $C_x$ in $\mathcal{C}$ (corresponding vertex $x$ in $V$), we define the price of $H$ as:
\[\gamma(C_x)=\frac{1}{|C_x \backslash R|}.\]
At each iteration, the greedy algorithm picks up the candidate set $C_x$ (vertex $x$)with the minimum $\gamma (H)$ (the cheapest price) and put it into $V^\ast$.
Then, the algorithm will update $R$ accordingly, $R=R\cup C_x$.
The process continues until no element in the ground set is uncovered $R=\mathcal{U}$. 
It has been proved that the approximation ratio of this algorithm is
$ln(|\mathcal{U}|)+1$~\cite{Feige98}.}

The implementation of the above set-cover approach is quite straightforward and can be sketched in the following steps:

\noindent{\bf Step 1:} We perform a local BFS for each vertex $u$ to visit all its neighbors with distance no greater than $\epsilon+1$ and add the vertex pairs (starting from $u$) with distance equal to $\epsilon+1$ to the ground set $\mathcal{U}$.

\noindent{\bf Step 2:} To generate all candidate sets, for each vertex $u$, we perform two local BFS traversals, one is the standard (forward) BFS which follows the outgoing edges of any vertex and the other is the {\em reversed} BFS which follows the incoming edges. Both stop at the depth $\epsilon$.
Specifically, for each vertex $u$, let $N_\epsilon(u)$ ($N^\prime_{\epsilon}(u)$)  denotes the forward (reversed) $\epsilon$-neighborhood which include all vertices $u$ can reach (can reach $u$) within $\epsilon$ hops. 
Then, for vertex pair $(x,y) \in N^\prime_\epsilon(u) \times N_\epsilon(u)$, which belongs to ground set, i.e., their distance is $\epsilon+1$, then, it will be added to the candidate set $C_u$. 
Figure~\ref{fig:bipartitecandidate} (c) shows the forward and reversed $(\epsilon=2)$-neighborhood for vertex $6$ in the running example graph (Figure~\ref{fig:runningexample}(a)) and Figure~\ref{fig:bipartitecandidate} (a) is the resulting candidate set $C_6$. 

\noindent{\bf Step 3:} Apply the greedy set-cover algorithm to discover  LMRBVS. 

Putting these together, we claim the following optimality of our approach in discovering LMRBVS. Its proof is omitted for simplicity. 

\bthm 
\label{optimal}
The set-cover approach finds a reachability backbone vertex set with the local meeting criterion 
whose size is larger than the smallest cardinality of such a vertex set by at most $O(\ln(|\mathcal{U}|)=O(\ln n)$ factor where $n$ is the number of vertices in the original graph $G$. 
\ethm


\noindent{\bf Computational Complexity:}
The overall computational complexity of the set-cover approach is as follows. 
In Step 1, generating the ground set takes $O(\sum_{v \in V} (|N_{\epsilon+1}(v)|+|E_{\epsilon+1}(v))|)$, 
where $|N_{\epsilon+1}(v)|$ ($|E_{\epsilon+1}(v)|$) is the number of vertices (edges) in the $v$'s forward 
$(\epsilon+1)$-neighborhood. 
In Step 2, since using hash table, checking the existence of $(x,y)$ in the ground set takes constant time,
the candidate set computation takes $O(\sum_{v \in V}(|N_\epsilon(v)|+ |E_\epsilon(v)| + |N^\prime_\epsilon(v)|+ 
|E^\prime_\epsilon(v)| + |N_\epsilon(v)| \times |N^\prime_\epsilon(v)|)$ time,
where $|N^\prime_{\epsilon}(v)|$ ($|E^\prime_{\epsilon}(v)|$) is the number of vertices (edges) in the $v$'s reversed $\epsilon$-neighborhood.
In Step 3, the fastest set cover algorithm ~\cite{Cormode:2010} can perform in linear time with respect to the size of candidate sets, i.e., $O(\sum_{v \in V} |C_v|)$, where $|C_v|\leq |N_\epsilon(v)| \times |N^\prime_\epsilon(v)|$. 
Now, consider for the random DAG with $n$ vertices and each vertex has an average out-degree and also in-degree $d$. 
Then, the overall time complexity of the set-cover approach is $O(n d^{2\epsilon})$. 
Since $\epsilon$ is generally very small (less than $5$) and $d$ is constant (and also small) for very large graphs, the set-cover approach scales linearly with respect to the graph size.  

However, for the large scale-free graphs, since it may contain some vertices with high out-degree and/or in-degree,  and they may produce very large ground set and candidate sets and make their materialization very cost. 
This can become the scaling bottleneck of this approach. 
To deal with this problem, we adopt a simple {\em preselecting strategy} to effectively alleviate this problem and to significantly reduce the size of set cover instance.
Basically, for some ``important'' vertices, we will preselect them (even before constructing the set-cover instance) as the reachability backbone vertices. Once they are selected, during the first step in the ground set construction, the local BFS can recognize those preselected vertices and immediately remove those non-local pairs  which have been already covered by them. 
Since the preselected  reachability backbone vertices are intended to cover as many non-local pairs in the ground set as possible, we define the ``importance'' of any vertex $u$ to be the product of its in-degree $indeg(u)$ and out-degree $outdeg(u)$, i.e., $I(u) = indeg(u) \times outdeg(u)$.
Then, we pickup the top $\alpha$ of vertices to be the preselected ones. 
Generally, $\alpha$ is quite small (no more than $5\%$). 
In Section~\ref{expr}, the detailed empirical study will demonstrate the effectiveness of the preselection strategy with different $\alpha$. 

\comment{

We sort all vertices in the decreasing order of their importance and pick top $5\%$ vertices as gate vertices. 
In the following, two issues we have to addressed in order to make the method work:
1) how to evaluate the ``importance'' of vertex with respect to set cover framework?
2) given preselected gate vertices, how can we efficiently construct the set cover instance for remaining vertex pairs?
We focus on the first question here.
Intuitively, a vertex with a large number of incoming edges and outgoing edges has high probability to be the intermediate node of many paths.
Motivated by this intuition, we 





\comment{
\noindent{\bf Scalable Set-Cover based Discovery}
Given ground set and candidate set, the straightforward way is to apply greedy set cover algorithm to discover the gate vertex set.
However, a potential issue of this approach for handling large graph is that ground set and candidate set should be explicitly materialized,
which might be too large to be hold in the memory.
To deal with this challenge, we adopt preselecting strategy to highly reduce the size of set cover instance.
}


The basic idea is that some ``important'' vertices are preselected as gate vertices based on certain criteria with lower computational cost,
and then the remaining vertex pairs with distance $\epsilon+1$ which are not covered by those preselected ones will be processed in set cover framework.
In the following, two issues we have to addressed in order to make the method work:
1) how to evaluate the ``importance'' of vertex with respect to set cover framework?
2) given preselected gate vertices, how can we efficiently construct the set cover instance for remaining vertex pairs?
We focus on the first question here.
Intuitively, a vertex with a large number of incoming edges and outgoing edges has high probability to be the intermediate node of many paths.
Motivated by this intuition, we define the ``importance'' of vertex $u$ by the product of indegree $indeg(u)$ and outdegree $outdeg(u)$, i.e., $I(u) = indeg(u) \times outdeg(u)$.
We sort all vertices in the decreasing order of their importance and pick top $5\%$ vertices as gate vertices.

The second question is answered in Algorithm~\ref{alg:partialgset}.

\input{Figures/GroundSetwithPreselection.tex}


\noindent{Complexity Analysis: }
Given that the branching factor (density) of the graph is $b$, and the largest depth attainable by the algorithm is $2\alpha$, the running time complexity is $O(b^{2\alpha})$.

\subsubsection{Discovering Backbone Edge Set}
\label{backboneedge}

}

\subsection{Constructing Backbone Edge Set $E^\ast$}
Given a set of reachability backbone vertices $V^\ast$, which satisfy the local meeting criterion, we can employ the following method to produce the backbone edge set $E^\ast$: for each vertex $u \in V^\ast$, add only edges in $E^\ast$ linking $u$ to only vertices in its $\epsilon$-neighborhood. 
Note that in Figure~\ref{fig:runningexample}(b), the edge set for the highlighted backbone vertex set is generated based on this method. 
The following lemma guarantees that the produced graph ($V^\ast,E^\ast$) maintains the reachability information in $V^\ast$, and can be used for recovering reachability between any non-local pair of vertices in the original graph.

\blemma
\label{lemma2}
Let $V^\ast$ be the reachability backbone vertex set which satisfy the local meeting criterion in $G$ and $E^\ast$ contain the edges which directly link any local-pair in $V^\ast$. 
Then if $u \rightarrow v$ in $G$ ($u,v \in V^\ast$), the $u\rightarrow v$ in $G^*$=($V^*$,$E^*$).
In other words, $TC^\ast(V^\ast) \subseteq E^\ast \subseteq TC(V^\ast)$. 
\elemma
\bproof
Since $(u,v) \in E^\ast$ only if $(u,v)$ is local pair in $G$ ($u\rightarrow v$), therefore, $E^\ast \subseteq TC(V^\ast)$. 
Now, we show $TC^\ast(V^\ast) \subseteq E^\ast$, i.e.,  if $u \rightarrow v$ in $G$, the $u\rightarrow v$ in $G^*$=($V^*$,$E^*$).
If $d(u,v) \leq\epsilon$, then $u\rightarrow v$ in $G^*$=($V^*$,$E^*$) by definition.
If $d(u,v)=\epsilon+1$, then based on Lemma 2, there exists a $x\in V^*$ such that $d(u,x)\leq\epsilon$ and $d(x,v)\leq\epsilon$.
So, based on the definition of $G^*$, $u\rightarrow v$. Now, if $d(u,v)>\epsilon+1$, then there is a vertex $w$ such that $d(u,w)=\epsilon+1$ and $w\rightarrow v$.
Based on Lemma 2, we can find a vertex $x\in V^*$ such that $d(u,x)\leq\epsilon$ and $d(x,w)\leq\epsilon$.
So, the proof is reduced to $d(x,v)$. We apply the same procedure until we reach a vertex $y\in V^*$ with $d(y,v)\leq\epsilon$.
Then, based on the definition of $G^*$, $u\rightarrow v$.
\eproof



\comment{
For simplicity, for any vertex $u$ in DAG $G$, let $G_\epsilon^{+}(u)=(N_\epsilon^+(u),E_\epsilon(u)$
%\noindent{\bf Set Cover Instance Construction: }

In order to adopt the aforementioned set-cover based algorithm to discover the gate-vertex set, we first have to generate the ground set $U$ and each candidate subset $C_x$ associating with vertex $x$.
Though we only need the non-local pairs with distance $\epsilon+1$, whose number is much smaller than all non-local pairs,
the straightforward approach still needs to find and explicitly record all vertex pair with distance no greater than $\epsilon+1$,
and then apply such information to generate each candidate set.
For large graphs, such computational and memory cost can still be rather expensive.

Here, we introduce a method to generate ground set and candidate set individually.
More importantly, we do not need to explicitly store all vertex pair with distance no greater than $\epsilon+1$. 

The implementation of 
Specifically, we first perform a local BFS for each vertex to visit its neighbors with distance no greater than $\epsilon+1$ in order to collect entire ground set.
To generate candidate set, for each vertex, we perform two BFS traversals by considering incoming edges and outgoing edges, respectively.
For each vertex $u$, let us denote $N^\prime_{\epsilon}(u)$ and $N_\epsilon(u)$ to be a set of vertices which can reach $u$ with distance no greater than $\epsilon$,
and a set of vertices which is reachable from $u$ with distance no greater than $\epsilon$.
We also call them incoming $\epsilon$-neighborhood and outgoing $\epsilon$-neighborhood.
Then, we check each vertex pair $(x,y) \in N^\prime_\epsilon(u) \times N_\epsilon(u)$ to see if it belongs to ground set.
If so, this vertex pair is appended to candidate set $C_u$.
Note that, $N^\prime_\epsilon$ and $N_\epsilon$ only serve as temporary data structure and avoid the expensive memory cost.
The procedure is outlined in Algorithm~\ref{alg:candiateset}.
The implementation utilizes bit vector to represent $N_\epsilon$ in order to speedup checking operation.

\input{Figures/ComputeSCInstance.tex}

\noindent{\bf Complexity Analysis: }
}


==> ComputeReach.tex <==
\vspace*{-2.0ex}
\section{Reachability Computation via \\Reachability Backbone}
\label{computation}

%The basic reachability computation method of utilizing the reachability backbone $G^\ast$ for a reachability query $(? u \rightarrow v)$ consists of two steps: 
Using the reachability backbone $G^\ast$ to compute a reachability query consists of two basic steps:

\noindent{\bf 1. Local Search for Accessing Backbone:} First, we perform two local BFS (within $\epsilon$ depth from the starting vertex) in the original DAG $G$: the forward BFS from $u$  to collect $B_{out}^\epsilon(u)$, the set of all backbone vertices which $u$ can reach within $\epsilon$ hops, i.e. $B_{out}^\epsilon(u)=\{x \in V^\ast | d(u,x) \leq \epsilon\}=V^\ast \cap N_\epsilon(u)$; and the reversed BFS from $v$ to collect $B_{in}^\epsilon(v)$, the set of all backbone vertices which can reach $v$ within $\epsilon$ hops, i.e., $B_{out}^\epsilon(v)=\{ y \in V^\ast | d(y,v) \leq \epsilon\}=V^\ast \cap N_\epsilon^\prime(v)$. Note that during the forward BFS (or reversed BFS), we can also check whether $u$ reaches $v$ locally ($d(u,v) \leq \epsilon$), and if it is, we directly confirm the reachability. 
%Furthermore, during the local BFS traversal, if a backbone vertex is visited, then, there is also no need to further expand it.  

\noindent{\bf 2. Reachability Join Test $(B_{out}^\epsilon(u) \rightarrow B_{in}^\epsilon(v))$:} The reachability join test $B_{out}^\epsilon(u) \rightarrow B_{in}^\epsilon(v)$  in the reachability backbone $G^\ast$ determines whether there exists $x \in B_{out}^\epsilon(u)$ and $y \in B_{in}^\epsilon(v)$, such that $x \rightarrow y$ in $G^\ast$. If it is then $u \rightarrow v$ in $G$ and not otherwise.
Given this, we basically need to compute the reachability between any $(x,y) \in B_{out}^\epsilon(u) \times B_{in}^\epsilon(v)$.
\rw{Note that since the}{Due to the modest} size of the reachability  backbone, we can effectively utilize any of the existing reachability indices and computational methods. 

\input{Figures/OnlineQuery.tex}
The basic reachability computation scheme is sketched in Algorithm~\ref{alg:onlinequery}. Note that ${\bf Reach}(x,y|G^\ast)$ is the generic reachability computation method (such as those describe in Section~\ref{sec:intro}) in the reachability backbone $G^\ast$. 
In the following, we will discuss strategies and refinement to speed up the basic computation scheme. 
Specifically, in Subsection~\ref{speedupindex}, we discuss optimization strategies to utilizing the transitive closure compression and hop-labeling approach.  Then in Subsection~\ref{speeduponline}, we describe how online search and GRAIL can be better adopted in this query scheme. 

\vspace*{-2.0ex}
\subsection{Speed Up Query Processing}
\label{speedupindex}

In this subsection, we focus on optimization strategies for the reachability indexing approaches: the transitive closure compression (category I) and hop-labeling approach (category II) which are applied to the reachability backbone $G^\ast$. 
Specifically, for any method in the first category, each vertex $x$ in the reachability backbone $G^\ast$ is assigned a compressed transitive closure $TC(x)$ (different methods utilize different compression strategies)  
and to compute ${\bf Reach}(x,y|G^\ast)$, a search procedure quickly determines whether $y \in TC(x)$; 
for any method in the second category, each vertex $x$ is assigned two labeling sets $L_{out}(x) \subseteq V^\ast$ (some vertices which $x$ can reach)  and $L_{in}(x) \subseteq V^\ast$ (some vertices which reach $x$).  To compute ${\bf Reach}(x,y|G^\ast)$, $L_{out}(x)$ is searched against $L_{in}(y)$ to see whether there is a common vertex~\cite{cohen2hop} (or there is a common chain~\cite{DBLP:conf/sigmod/JinXRF09,Cai:2010}) which can link $x$ to $y$. 

Given this, we can observe the performance of Algorithm~\ref{alg:onlinequery} is determined by these two steps for any reachability query $(? u \rightarrow v)$: 
1)  the two local BFS compute the backbone access vertex sets $B^\epsilon_{out}(u)$ and $B^\epsilon_{in}(v)$ and one of them is used to determine whether the start vertex can reach the end vertex locally. 
Here, the potential problem is that BFS may potentially scan a large number of vertices and edges, especially when there are hub vertices (incoming or outgoing) in the $\epsilon$-neighborhood.  
2)  the cost of the reachability join test is determined by the number of reachability pair queries. In the basic scheme, we need to compute $|B^\epsilon_{out}(u)| \times |B^\epsilon_{in}(v)|$ pairs, which can be expensive.

\noindent{\bf Access Vertex Materialization and Reduction:} To address these two problems, our first strategy is to explicitly materialize the backbone access vertex sets for each vertex $u$. This is because the number of those vertices is generally quite small. Interestingly, the actual materialized vertex set can be even smaller: given DAG $G$ and its reachability backbone $V^\ast$, for each vertex $u$, the following two backbone access vertex sets need to be materialized: 
\beqnarr 
\boldsymbol{\mathcal{B}}^\epsilon_{out}(u)=\{v \in V^\ast| d(u,v) \leq \epsilon \mbox{ and  there is no other vertex $x$}, \nonumber \\ \mbox{   in $V^\ast$   such that }
d(u,x) \leq \epsilon \wedge d(x,v) \leq \epsilon  (u \rightarrow x \rightarrow v) \} \nonumber \\
\boldsymbol{\mathcal{B}}^\epsilon_{in}(u) = \{v \in V^\ast| d(v,u) \leq \epsilon \mbox{ and there is no other vertex $y$ }, \nonumber \\ \mbox{   in $V^\ast$   such that } 
d(v,y) \leq \epsilon \wedge d(y,u) \leq \epsilon (v \rightarrow y \rightarrow u) \} \nonumber
\eeqnarr

\blemma({\bf Access Vertex Reduction}) 
\label{accessvertex}
For any reachability query $(? u \rightarrow v)$, when $(u,v)$ is a non-local pair,
%($d(u,v) \leq \epsilon$),
it is sufficient to 
perform reachability join test between $\boldsymbol{\mathcal{B}}^\epsilon_{out}(u)$ and $\boldsymbol{\mathcal{B}}^\epsilon_{in}(v)$, i.e., $\boldsymbol{\mathcal{B}}^\epsilon_{out}(u) \rightarrow \boldsymbol{\mathcal{B}}^\epsilon_{in}(v)$, to determine whether $u$ can reach $v$. 
\elemma

\rw{Intuitively, Lemma~\ref{accessvertex} basically suggests that only a vertex in $V^\ast$ is ``first'' accessed, during the local BFS, meaning none of its predecessors (based on the visiting order) have been visited by the BFS, need to considered in the reachability join test.}
{Intuitively, Lemma~\ref{accessvertex} suggests that if a backbone vertex in $V^\ast$ is accessed, then none of its successors (according to visit order) need to be consider in the reachability join test.}
This is because those pruned vertices are already in the backbone and can be accessed by those ``first-accessed'' ones. Therefore there is no need to record or utilize them in the reachability join test. Due to the space limitation, we omit the proof of Lemma~\ref{accessvertex}.  
Since $|\boldsymbol{\mathcal{B}}^\epsilon_{out}(u)| \leq |B^\epsilon_{out}(u)|$ and $|\boldsymbol{\mathcal{B}}^\epsilon_{in}(v)| \leq |B^\epsilon_{in}(v)|$ for any vertex pair, this strategy
\rw{can not only help reduce the online search cost, but also can reduce the cost of reachability join test. }
{can reduce the cost not only of online search but also of reachability join test.}

\comment{%TOO DETAIL
Note that Lemma~\ref{accessvertex} can not only help reduce the materialization cost of access vertices, it also suggest when we can reduce the computational cost of the materialization. 
This is because the basic method of materialization is to perform both forward and reversed BFS locally for each vertex $u$ in order to collect $B^\epsilon_{out}(u)$ and $B^\epsilon_{out}(u)$}


\noindent{\bf Online Pruning:} The second strategy targets directly the reachability join test. 
\rw{The basic idea is that if}{If} we can quickly reject $x  \rightarrow y$ where  $x \in \boldsymbol{\mathcal{B}}^\epsilon_{out}(u)$ and $y \in \boldsymbol{\mathcal{B}}^\epsilon_{in}(v)$, then we do not need to actually perform ${\bf Reach}(x,y|G^\ast)$, which either involves searching through the compressed transitive closure of $x$, $TC(x)$ (in Category I) or comparing two labeling sets $L_{out}(x)$ and $L_{in}(y)$ (in Category II). 
Furthermore, if we can quickly reject $x \rightarrow v$, then we can even directly avoid the reachability tests against all vertices in $\boldsymbol{\mathcal{B}}^\epsilon_{in}(v)$. 

To achieve such goal, we utilize the interval labeling method in GRAIL~\cite{yildirim:grail}. 
Basically, each vertex $u$ in the entire graph $G$ is assigned multiple interval labels $\mathcal{I}_u$ which can help to determine quickly the non-reachability between two vertices.
These labels are generated by performing a constant number ($c$) of {\em random} depth-first traversals, i.e., the visiting order of the neighbors of each vertex is randomized in each traversal.
Each traversal will produce one interval for every vertex in the graph.
Such interval labeling has the property that
if $\mathcal{I}_v \nsubseteq \mathcal{I}_u$, then vertex $u$ cannot reach vertex $v$.
However, when $\mathcal{I}_v \subseteq \mathcal{I}_u$, we cannot determine whether $u$ can reach $v$.
GRAIL~\cite{yildirim:grail} utilizes this labeling in the depth-first search to prune the search space.
Such a labeling can be constructed very fast ($O(c(n+m))$) and its index size is only $O(cn)$, where $c$ \rw{is shown to be almost}{can be} quite small ($c=5$ is shown to be sufficient to provide good pruning)~\cite{yildirim:grail}. 

\rw{Here, we simply utilize}{We use} such labeling to help quickly reject any $(x,y)$ pairs in $\boldsymbol{\mathcal{B}}^\epsilon_{out}(u) \times \boldsymbol{\mathcal{B}}^\epsilon_{in}(v)$ and any vertex $x$ which cannot lead to $u \rightarrow v$. 
\rw{We would like to point out that here w}{W}e explicitly compute each ${\bf Reach}(x,y|G^\ast)$ only if we cannot simply prune such a test using the multi-interval labeling. 
Note that for the hop-labeling approach (Category II), an alternative strategy exists which can directly avoid the explicit the pair-wise reachability computation. 
The idea is to first merge all the $L_{out}(x)$ for $x \in \boldsymbol{\mathcal{B}}^\epsilon_{out}(u)$ and $L_{in}(y)$ for all $y \in  \boldsymbol{\mathcal{B}}^\epsilon_{in}(v)$, and then perform a comparison between the two merged lists. 
However, since the merge cost is actually quite expensive, we found this method is actually much slower than explicit pairwise comparison together with the online pruning method. 
\rw{Especially, we note that  the explicit pairwise comparison enables quick early termination (when the first $x \rightarrow y$ is confirmed), which}
{Explicit pairwise comparison's early termination (when the first $x \rightarrow y$ is confirmed)} turns out to be quite effective.
Thus, we do not adopt the merge strategy here. 

\noindent{\bf Bidirectional Local Search:}
Though there is no need to perform the online BFS to collect the reachability backbone access vertices, we still need to determine whether $u$ can reach $v$ locally, i.e., $d(u,v) \leq \epsilon$. 
To perform such a local test, we can utilize a bidirectional BFS to reduce the search space. 
Specifically, the forward BFS starting at $u$ needs to expand to at most $\lceil \epsilon/2 \rceil$ depth and 
the reversed BFS starting from $v$ needs to expand to $\lfloor \epsilon/2 \rfloor$ depth. 
Furthermore, in either BFS expansion, if a reachability backbone vertex (in $V^\ast$) is visited, then we do not have to further expand its outgoing (or incoming) vertices,
a considerable savings for hub vertices.
%obvious% This is because we do not want to expand any hub vertices and since they are in the backbone, we can leave the reachability computation involving them in the reachability join test (following similar idea in Lemma~\ref{accessvertex}). 
Hub vertices (a vertex either with high in-degree of out-degree) tend to be covered in the reachability backbone vertex set. Indeed, if they are not covered, we can explicitly add them to the reachability backbone. 
Since the number of hub vertices tend to be quite small~\cite{Newman03}, this strategy can help reduce the cost of local search while not greatly expanding the backbone size. 
%In the empirical study (Section~\ref{expr}),  the $0.1\%$ vertices with the highest in-degree and out-degree degree will be always added to the reachability backbone. 

\input{Figures/FastReach.tex}

The query processing algorithm which incorporates the above optimization strategies  is sketched in Algorithm~\ref{alg:fastreach}. Clearly, its worst case computational complexity can be partitioned into two parts ($O(T_1+T_2)$). $T_1$ comes from the bidirectional local search, where $T1=  \max_{u \in V} (|N_{\lceil \epsilon/2 \rceil}(u)| + |E_{\lceil \epsilon/2 \rceil}(u)|)+$ \\ $\max_{v \in V}$ $(|N^\prime_{\lfloor \epsilon/2 \rfloor}(v) | + |E^\prime_{\lfloor \epsilon/2 \rfloor}|)$. $T_2$ is the cost of the reachability join test, given by $\max_{u, v \in V} |\boldsymbol{\mathcal{B}}^\epsilon_{out}(u)| \times |\boldsymbol{\mathcal{B}}^\epsilon_{in}(v)| \times T_3 $ $\leq \max_{u, v \in V} |N_{\epsilon}(u)| \times |N_{\epsilon}(v)| \times T_3$, where $T_3$ is the worst case complexity of different reachability computational methods in the reachability backbone $G^\ast$.
Recall that $|N^\prime_{\epsilon}(v)|$ ($|E^\prime_{\epsilon}(v)|$) is the number of vertices (edges) in $v$'s reversed $\epsilon$-neighborhood. 
For instance, consider Agrawal {\em et al.}'s tree-interval~\cite{SIGMOD:AgrawalBJ:1989} is used to compress the transitive closure in the reachability backbone and let $n^\prime=|V^\ast|$, and assume the original graph is a random DAG with average in-degree and out-degree $d$, then the worst case computational complexity of {\em FastReach} can be simplified to $O(d^{\lceil \epsilon/2 \rceil}+ d^{2\epsilon} \dot  \log n^\prime)$.
As we will show in Section~\ref{expr},  the actual number of {\bf Reach} invocations is much smaller than $d^{2\epsilon}$ and can be treated as constant (it is also a local measure). 
Thus, the worst case query computational complexity can be effectively scaled down and directly relates to the size of the reachability backbone. 


\vspace*{-2.0ex}
\subsection{Speed Up Online Search}
\label{speeduponline}
The {\em FastReach} query processing scheme can be applied to the (refined) online search methods (Category III) such as GRAIL. 
Basically, each invocation of ${\bf Reach}(x,y|G^\ast)$ needs to perform an independent  GRAIL search. 
However, this is clearly very expensive as each search needs to travel a large search space in $G^\ast$ and the search spaces of different invocations can even overlap. 
Furthermore, assuming both $y_1$ and $y_2$ are in $\bold{\mathcal{B}}^\epsilon_{in}(v)$, and $x \in \bold{\mathcal{B}}^\epsilon_{out}(u)$, it may happen during ${\bf Reach}(x,y_1|G^\ast)$, it may reach $y_2$ even though $x$ cannot reach $y_1$. 
Finally, for the online search method, the cost of local online search (for collecting access vertices in the reachability backbone) compared with the search in the reachability backbone is quite small. 
Thus, the need to actually materialize them is small. 

Given this, {\em OnlineSearch} is proposed to deal with these issues and consists the following main steps: \\
{\em 
\noindent{\bf 1.} Perform a reversed BFS from $v$ and for each visited reachability backbone vertex $y \in V^\ast$, flag it to be ``target''. If $u$ is visited, return TRUE; \\
\noindent{\bf 2.} Perform a forward BFS from $u$ and if any visited vertex $x$ is a reachability backbone vertex $x  \in V^\ast$, then perform a online search (recursive) from $u$ in $G^\ast$: \\
\mbox{         } {\bf 2.1.} if the current visited vertex $x$ is already visited before ($visit[x]=TRUE$),  then return (trace back); \\
\mbox{         } {\bf 2.2.} if the current visited vertex $x$ is a target ($target[x]=TRUE$), then return TRUE;  \\
\mbox{         } {\bf 2.3.} recursively visited all $x$'s neighbors.  \\
\noindent{\bf 3.} return FALSE; 
}

Basically, all the different searches starting from different backbone access vertices (in {\bf 2.}) can be considered as a single recursive graph traversal. 
To answer a reachability query $(u,v)$, any vertex in $G^\ast$ will be visited at most once. 
This is because we first flag all the backbone vertices which reach $v$ within $\epsilon$ steps. 
Thus, if a vertex is already visited in the earlier search, then it basically has no chance to reach any of the flagged backbone vertices and no need to revisit them. 
Also, during the forward and reverse BFS, if a backbone vertex is visited, then there is no need to further explore it (similar to Lemma~\ref{accessvertex}). 
In addition, we note for the refined online search, such as GRAIL, we can also utilize the interval labeling in both BFS in the original graph and recursive search in the reachability backbone search. 
For instance, in the reversed BFS, we only need to visit vertex $y$ such that $\mathcal{I}_y \subseteq \mathcal{I}_u$, and in both forward BFS and online recursive search, we only need to visit vertex $x$ such that $\mathcal{I}_v \subseteq \mathcal{I}_x$. 
Finally, we note that if we focus on the computational cost of the online recursive search as it is usually the dominant one, then the worst-case computational complexity of {\em OnlineSearch} is $O(n^\prime+m^\prime)$, where $n^\prime=|V^\ast|$ and $m^\prime=|E^\ast|$ for any refined online search method~\cite{yildirim:grail,Chen05,Trissl07}.


\comment{

They share the same search space and each vertex  treated  
Note that the key feature of the {\em OnlineSearch} is 


}

 

\comment{


\section{Gate Graph Indexing and Reachability Querying}
\label{gateindexing}

Online query procedure actually offers a general search framework based on gate graph.
Its query performance highly depends on how to check reachability between a pair of gate vertices (Line 4 in Algorithm~\ref{alg:onlinequery}).
We know that many literatures have proposed different graph indexing schemes to improve the efficiency of query procedure.
Here, we utilize them to generate reachability index for each gate vertex in the gate graph.
Basically, two categories of algorithms are considered: 1) tree-based approaches, such as tree cover and path-tree;
2) hop-based approaches, such as 2hop.
Besides that, the corresponding querying procedure and some speedup strategies are also presented.
More importantly, we will introduce a scalable 2hop algorithm to handle large graphs in an efficient way.
Note that, since the reachability on ``local'' vertex pairs can be efficiently answered by local BFS under smaller value of $\epsilon$,
we concentrate on addressing the reachability query on ``non-local'' vertex pairs.


\comment{
\subsection{Tree-based Indexing}
\label{treeindexing}

As the basic ideas of tree cover indexing and path-tree indexing algorithm have been well surveyed in the related work,
we directly go to the query processing.
The most straightforward way is to apply query algorithm used in tree-based approaches to replace DFS search in Algorithm~\ref{alg:onlinequery}.
To further speedup the query efficiency, we will consider the reachability from set viewpoint,
i.e., from gate vertex set $N^{out}_\epsilon(s)$ to gate vertex set $N^{in}_\epsilon(t)$ instead of each pair of vertices.

\input{Figures/TreecoverQuery.tex}

\noindent{\bf Tree Cover: }
The query procedure is outlined in Algorithm~\ref{alg:treecoverquery}.
Firstly, we sort the intervals associated with local gate vertex sets based on interval's first value.
If one interval $[a,b]$ of $u$ is contained by another interval $[c,d]$ of $v$, the interval $[a,b]$ can be removed during sorting,
because the vertices which can be reached by $u$ are guaranteed to be reachable from $v$.
Also, the intervals of vertices $I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$ are sorted similarly.
Given this, we linearly scan those two interval lists to see if there is one interval from $I_s$ containing one interval from $I_t$.
If so, we say $s$ can reach $t$. Otherwise, vertex $t$ is not reachable from vertex $s$.
The sorting step takes $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$ time
and scanning step takes $O(|N_\epsilon^{out}(s)|+|N_\epsilon^{in}(t)|)$ time.
Therefore, the time complexity of query procedure is $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$.


\input{Figures/PathtreeQuery.tex}

{\bf Path-Tree: }
Each gate vertex $u$ in path-tree is assigned with 3 numbers and also records a list of vertices $L(u)$ which can be reached by $u$ while path-tree cover does not cover it.
To answer the reachability from vertex $u$ to vertex $v$, we need to check whether $u$ can reach $v$ by path-tree cover and whether any vertex $w$ in $L(u)$ can $v$.
An efficient query scheme based on interval tree is proposed in the paper to process each query in $O(\log^2 k)$ time, where $k$ is the number of paths in path decomposition.
Motivated by this method, we consider all vertices $I_s = \cup_{x \in N_\epsilon^{out}(s)} L(x)$ together to construct a ``large'' interval tree $T_s$.
Indeed, this is equivalent to creating a virtual node with all reachability information from $I_s$.
Then, for each vertex $y \in I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$, we can efficiently check whether it can be reached by some vertex from $I_s$ in $O(\log^2(dk))$ time,
where $d= |N_\epsilon^{out}(s)|$ and $k$ is the number of path generated by path decomposition on gate graph.
The time complexity of searching on interval tree is $O(d^\prime  \log^2 (dk))$ since the size of $N_\epsilon^{in}(t)$ is $d^\prime$ and we need to invoke such single query $d^\prime$ times.
Considering the sorting and interval tree building steps together, the running time is $O(d^\prime \log^2 (dk))$ in total.
We describe the procedure in Algorithm~\ref{alg:pathtreequery}.


\subsection{Hop-based Indexing (Scalable 2HOP)}
\label{hopindexing}

2-Hop is most well-known algorithm in this category.
However, due to its high computational and memory cost, it is even hard to apply it for medium sized graph with tens of thousands of vertices.
To deal with this challenge, we introduce a scalable 2hop approach based on bipartite set cover (BSC) framework and still achieve the logarithmic bound.

Before go to solution, we first introduce general concept of bipartite set cover framework.
Let $S$ be the ground set to be covered.
Let $\mathcal{G}=(A\cup B,\mathcal{E})$ be a bipartite graph where an edge in $\mathcal{E}$ connects two vertices from $A$ and $B$, respectively.
Each edge $e$ is associated with a subset $S_e \subseteq S$ and $S = \cup_{e \in \mathcal{E}} S_e$.
Let $\mathcal{X}$ and $\mathcal{Y}$ be subsets of $A$ and $B$, respectively.
Let $\mathcal{G}[\mathcal{X} \cup \mathcal{Y}]$ be the {\em induced} subgraph of $\mathcal{X}$ and $\mathcal{Y}$, i.e., it contains all the edges whose both ends are in $\mathcal{X} \cup \mathcal{Y}$.
Let $\mathcal{E}[\mathcal{X} \cup \mathcal{Y}]$ be the edge set of the induced subgraph $\mathcal{G}[\mathcal{X} \cup \mathcal{Y}]$.
Let $\mathcal{C}(\mathcal{E}[\mathcal{X} \cup \mathcal{Y}])$ be the union of sets covering all its edges, i.e.,
$\mathcal{C}(\mathcal{E}[\mathcal{X} \cup \mathcal{Y}])=\bigcup_{e \in \mathcal{E}[\mathcal{X} \cup \mathcal{Y}]} S_e$
Further, we associate a weight with each vertex $z$ in $A \cup B$, denoted as $cost(z)$.
Given this, the bipartite set cover problem is defined as follows.

\bdefin{\bf (Bipartite Set Cover (BSC) Problem)}
Given the ground set $S$ and a bipartite graph $\mathcal{G}=(A\cup B,\mathcal{E})$, where $S=\cup_{e \in \mathcal{E}} S_e$,
we seek vertex subsets $\mathcal{X} \cup \mathcal{Y}$ ($\mathcal{X} \subseteq A$ and $\mathcal{Y} \subseteq B$) to cover the ground set, i.e., $S=\mathcal{C}(\mathcal{E}[\mathcal{X} \cup \mathcal{Y}])$, with the minimal cost,
$\sum_{z \in \mathcal{X} \cup \mathcal{Y}} cost(z)$.
\edefin

By reducing the classical set-cover problem to BSC, we can prove that the bipartite set covering (BSC) problem is NP-hard.
Now, we transform the minimum 2-hop labeling problem to the simplified version of BSC problem as follows.

Let the ground set $S=TC(G)$, i.e., it contains any vertex pair $(u,v)$ in $G$, such as $u \rightarrow v$.
To cover a pair $(u,v)$ means we can restore their reachability in the labeling scheme.
We construct a bipartite graph $\mathcal{G}=(A\cup B,\mathcal{E})$ for the covering purpose:
a vertex in $A$ corresponds to a tuple: $(u, x_i)$, where $u$ is a starting vertex, $x_i$ is a candidate vertex can be reached from $u$;
a vertex in $B$ corresponds to a tuple: $(y_i, v)$, where $v$ is a destination vertex, $y_j$ is a candidate vertex which can reach $v$.
Given this, for any four vertices, $(u,x_i,y_j,v)$, if $x_i = y_j$,
we will add vertex $(u, x_i)$ to $A$, add vertex $(y_i,v)$ to $B$, and add an edge from the first vertex to the latter one.
In addition, in the edge, we will associate a singleton $\{(u,v)\}$.
Further, we assign a unit cost  to each vertex in the bipartite graph, i.e., $cost(e)=1$.
It is not hard to see that if we can find vertex subsets $\mathcal{X} \cup \mathcal{Y}$ ($\mathcal{X} \subseteq A$ and $\mathcal{Y} \subseteq B$) to cover the ground set, we basically are able to restore transitive closure matrix of graph $G$.
Specifically, we have the following relationship:
{\small
\beqnarr
(u,x_i) \in \mathcal{X} &\Longleftrightarrow&  x_i \in L_{out}(u); \nonumber \\
(y_i,v) \in \mathcal{Y} &\Longleftrightarrow&  y_i \in L_{in}(v). \nonumber
\eeqnarr}

\subsubsection{Bipartite Set Cover Algorithm}
\label{bscalg}

The bipartite set cover can be considered as a special case of set-cover-with-pairs problem~\cite{}.
From the perspective of graph formulation, the input of set-cover-with-pairs (SCP) problem is a complete graph while it is bipartite graph in BSC.
Therefore, we can directly apply the existing greedy algorithm for SCP~\cite{} to the BSC problem.
This greedy algorithm have been proved to yield an $O(\sqrt{N \log N})$ approximation ratio, where $N$ is the cardinality of the ground set $N=|U|$ for cardinality BSC problem.
Since $U=TC(G)$ and $N=|TC(G)|$ in 2-hop labeling problem, the approximation bound can be downgraded to $O(n \sqrt{\log n})$, which is not attractive.

Here, we present a fast greedy algorithm that yields $\frac{2}{1-\alpha}(\ln N+1) $ approximation ratio for our BSC problem. For simplicity, we focus on our special case, where each node has a unit cost and each edge is associated with only a singleton.
Our greedy algorithm works as follows: {\em each time we select a node in the bipartite graph $\mathcal{G}=(A \cup B, \mathcal{E})$ according to our defined criterion, until all the elements in the ground set, i.e.,  all pair shortest distance of $G$ in our HCL problem, have been covered.}
To describe our node-selection criterion, we introduce the following definitions:
Let $U$ be the ground set and $R$ be the set recording the already covered elements: $R\subseteq U$.
Let $S$ be the set of already selected nodes in the bipartite graph and let $\overline{S}$ denote the unused nodes in the bipartite graph, $\overline{S}=(A\cup B) \backslash S$.
Assume at some iteration, node $v$ is to be selected. Let $\mathcal{E}(v)$ be the set of edges in $\mathcal{G}$ adjacent to $v$. Then $\mathcal{E}(v)$ covers a set of elements in $U\backslash R$. We are classify these covered elements on the edges adjacent to $v$ into two parts:
1) one part is immediately covered by selecting $v$;
in other worlds, $v$ will work directly on those already selected nodes in $S$, denoted as $S_{v}$, to cover this part of the elements;
2) the other part is those elements which may be covered in the future when selecting nodes in $Z_{v}$, where $Z_{v}\subseteq \overline{S}$ and each node in $Z_{v}$ is adjacent to $v$.
It is easy to see $|S_{v}|$ is exactly how many new elements will be covered if we select $v$ at step $i$,
and $|Z_{v}|$ is how many new elements will be {\em potentially} covered as a consequence of selecting $v$.
In other words, $|S_{v}|+|Z_{v}|$ is the upper bound of the number of elements which can be covered by selecting node $v$.
In our algorithm, at each iteration, we select node $v$ from $\overline{S}$ with minimum $\frac{1}{|S_{v}|+|Z_{v}|}$.

\input{Figures/greedy.tex}

We describe the entire procedure in Algorithm~\ref{alg:greedyCover}.
This algorithm is proved to produce an $O(\frac{2}{1-\alpha}(\ln N+1))$ approximation bound, formally stated in theorem~\ref{approxbound}.

\bthm
\label{approxbound}
The greedyCover algorithm (Algorithm~\ref{alg:greedyCover}) has\\
$\frac{2}{1-\alpha}(\ln N+1) $ approximation ratio solution with respect to the optimal solution, where $\alpha=\frac{1}{|S|}\sum_{v\in S}\frac{|\Delta_{Z_v}|}{|S_v|+|Z_v|}$.
\ethm

The original 2-Hop labeling algorithm has prohibitive computational complexity $O(n^3|TC(G)|)$~\cite{DBLP:conf/sigmod/JinXRF09}.
Now, we can apply our general BSC solver to deal with the bipartite graph ($\mathcal{G}_0$) generated by $2$-hop.
We note that the greedy algorithm runs in $O(\sum_{u\in V} (|L_{out}(u)|+|L_{in}(u)|))$ steps.
Each step, using the speedup queue technique, assuming we only need visit $k<<|V|$ nodes in the queue, takes $O(k(\log |TC|+|V|))$ time to extract and update the queue.
In addition, maintaining the covered set takes $O(|TC|)$ time. Clearly, the time complexity is much lower than the original $2$-hop approach.

\subsubsection{Query Processing of 2HOP}
\label{2hopquery}

We apply above scalable 2hop labeling on gate graph, and each vertex $u$ will be assigned with a set of vertices $L_{out}(u)$ which can be reached by $u$ and a set of vertices $L_{in}(u)$ which can reach $u$.
The query scheme using both gate graph and 2hop labels is quite similar to query scheme of tree cover approach.
Specifically, to answer the reachability from vertex $s$ to vertex $t$, we first collect local gate vertex sets $N_\epsilon^{out}(s)$ and $N_\epsilon^{in}(t)$.
Then, we sort both sets and linearly scan them to check if there is one vertex $x$ in the path from $s$ to $t$, such that $x \in N_\epsilon^{out}(s) \cap N_\epsilon^{in}(t)$.


\subsection{Label Materialization}
\label{labelmater}

It is not hard to see that both gate materialization and pruning strategy for online query can be applied here to improve graph indexing-based query.
Even through, during the query answering process, we still need to access local gate vertices' labels for reachability checking.
To further improve the query efficiency, we can precollect the labels of each vertex's local gate vertex set and organize them in an appropriate way to facilitate online processing.
However, in most of cases, available memory resource is limited and it is impossible to explicitly record those labels for every vertex.
In this sense, a question is naturally arisen: given memory budget, how to select a set of most ``important'' vertices for precomputation where their computational cost fits into memory budget and overall online query performance will be maximally improved?


}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{
This category of algorithms uses the tree-like structure to compress the transitive closure of a DAG.
The representatives include tree cover, dual labeling and path-tree.
Those algorithms need to precompute the transitive closure which becomes memory bottleneck in processing large-scale graphs.
However, gate graph is supposed to be small under the appropriate parameter $\epsilon$,
thus memory issue on computing transitive closure can be omitted.

In these algorithms, a tree-like structure is extracted to compress the transitive closure matrix.
Basically, each vertex is assigned with several integers which is used to maintain reachability information within tree-like structure.
Besides that, each vertex $u$ needs to record a list of vertices $L(u)$ which are reachable from $u$ while their reachability are not covered in tree-like structure.
In contrast to transitive closure covered by tree-like structure, the union of $L(u)$ indicates the uncovered transitive closure.
We apply those methods to build index on gate graph.

\noindent{\bf Tree-based Query }
Instead of online checking reachability of gate vertex pair (Line 4 in Algorithm~\ref{alg:onlinequery}),
we use graph indices to quickly determine whether they are reachable.
The most straightforward way is to directly utilize the existing query methods based on corresponding graph indexing to answer reachability query.
However, it is worthwhile to note that, we actually want to check the reachability from a set of vertices $N^{out}_\epsilon(s)$ to another set of vertices $N^{in}_\epsilon(t)$.
We consider the query processing on two sets in the following.

\input{Figures/TreecoverQuery.tex}

{\bf Tree Cover: }
Each gate vertex is assigned with a pair of numbers (i.e., an interval $[a,b]$).
If gate vertex $u$ can reach gate vertex $v$, the interval of $u$ contains the interval of $v$.
Moreover, each gate vertex $u$ also records a list of vertices $L(u)$ which it can reach in the gate graph and their reachability are not covered in the tree.
Now, for starting vertex $s$, we consider all vertices $I_s = \cup_{x \in N_\epsilon^{out}(s)} L(x) $ together.
Firstly, we sort the intervals attached with those vertices based on their first value.
If one interval $[a,b]$ is contained by another interval $[c,d]$, the interval $[a,b]$ can be removed during sorting,
because the vertices which can be reached by this vertex are guaranteed to be reachable from the one with interval $[c,d]$.
Also, the intervals of vertices $I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$ are sorted similarly.
Given this, we can linearly scan those two interval lists to see if there is one interval from $I_s$ containing one interval from $I_t$.
If so, we say $s$ can reach $t$. Otherwise, vertex $t$ is not reachable from vertex $s$.
The query procedure is outlined in Algorithm~\ref{alg:treecoverquery}.
The sorting step takes $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$ time
and scanning step takes $O(|N_\epsilon^{out}(s)|+|N_\epsilon^{in}(t)|)$ time.
Therefore, the time complexity of query procedure is $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$.

\input{Figures/PathtreeQuery.tex}

{\bf Path-Tree: }
Each gate vertex $u$ in path-tree is assigned with 3 numbers and also records a list of vertices $L(u)$ which can be reached by $u$ and path-tree cover does not cover it.
To answer the reachability from vertex $u$ to vertex $v$, we need to check whether $u$ can reach $v$ by path-tree cover and whether any vertex $w$ in $L(u)$ can $v$.
An efficient query scheme based on interval tree is proposed to process each query in $O(\log^2 k)$ time, where $k$ is the number of paths in path decomposition.
Motivated by this method, we consider all vertices $I_s = \cup_{x \in N_\epsilon^{out}(s)} L(x)$ together to construct a ``large'' interval tree $T_s$.
Indeed, this is equivalent to creating a virtual node with all reachability information from $I_s$.
Then, for each vertex $y \in I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$, we can efficiently check whether it can be reached by some vertex from $I_s$ in $O(\log^2(dk))$ time,
where $d= |N_\epsilon^{out}(s)|$ and $k$ is the number of path generated by path decomposition on gate graph.
The time complexity of searching on interval tree is $O(d^\prime k \log^2 (dk))$ since the size of $N_\epsilon^{in}(t)$ is $d^\prime$ and we need to invoke such single query $d^\prime$ times.
Considering the sorting and interval tree building steps together, the running time is $O(d^\prime k \log^2 (dk))$ in total.
We describe the procedure in Algorithm~\ref{alg:pathtreequery}.


{\bf Speedup Tree-based Query Processing: }
To improve the query efficiency, we precompute some intermediate results and explicitly record them for online processing.
That is, local gate vertices collection and interval sorting in Algorithm~\ref{alg:treecoverquery},
and local gate vertices collection and interval tree building in Algorithm~\ref{alg:pathtreequery} can be performed beforehand.
Clearly, extra memory is needed to store those intermediate results.
For tree cover, each vertex $u$ needs to record sorted interval list of local gate vertices with size $O(dm)$, where $m=|L(u)|$.
For path tree, each vertex $u$ needs to record the interval tree build on top of local gate vertices with size $O(dk)$.
Furthermore, to fit those extra cost into available memory size, the partial materialization strategy introduced in subsection~\ref{speeduponline} can be applied here.
In other words, only the vertex whose local gate vertex sets' sizes are no greater than certain threshold will be preprocessed.
}




\comment{
To answer second question, a novel method based on two level BFS traversals is introduced.
For each unselected vertices, we will online perform local BFS within $\epsilon+1$ steps and add all vertex pairs which are not covered by existing gate vertices into ground set.
For each vertex $u$, assuming its $\epsilon+1$-neighborhood is $N_\epsilon(u)$,
our goal is to eliminate some vertices $x$ from them such that $(u,x)$ can be covered by existing gate vertices.
Two cases can lead to elimination of vertex $x$: 1) some gate vertices is in the shortest path from $u$ to $x$;
2) some gate vertices $v$ is not in the shortest path $P_{ux}$ but satisfies the condition $d(u,v) \le \epsilon$ and $d(v,x) \le \epsilon$.
The first case can be easily checked by local BFS, while the second case needs extra BFS from observed gate vertex to certain depth.
The entire procedure is described in Algorithm~\ref{alg:partialgset}.
In the algorithm, each vertex $u$ is associated with value $c(u)$ to indicate the closest gate vertex which can reach it.
For $u$'s any $\epsilon+1$-neighbor $x$, if its $c(x)$ is assigned with some value, then case 1 is discovered and vertex pair $(u,x)$ has been covered.
In order to check case 2, we need to perform local BFS from gate vertex to see if some $u$'s $\epsilon+1$-neighbors can be reached within $\epsilon$ steps.
If so, case 2 is observed and certain vertex pair can also be omitted in ground set.

\input{Figures/GroundSetwithPreselection.tex}
}

\comment{
The algorithms in this category employs intermediate hops (i.e., vertex in 2hop and chain in 3hop) to store reachability information.
In these methods, each vertex $u$ is assigned with a list of intermediate vertices $L_{out}(u)$ which it can reach and a list of intermediate vertices $L_{in}(u)$ which is reachable from this vertex.
To answer the reachability from source $s$ to destination $t$,
we perform join operation on $L_{out}(s)$ and $L_{in}(t)$ to check if there is some intermediate hops in the path from $s$ to $t$.
The minimization of total number of intermediate vertices builds on top of set cover framework, which is costly for very large graph.
As mentioned, gate graph is significantly smaller than original one, which is possible to be handled by those algorithms.
We apply hop-based indexing algorithm to assign each vertex two lists of vertices $L_{out}$ and $L_{in}$.

In the following, we discuss how to process queries based on gate graph in 2hop and 3hop schemes, respectively.
Basically, we still need to consider the query processing from source's local gate vertex set to target's local gate vertex set.
Assume we try to answer the reachability from $s$ to $t$.
For 2hop, we first collect local gate vertex sets $N_\epsilon^{out}(s)$ and $N_\epsilon^{in}(t)$.
Then, we sort both sets and linearly scan them to check if there is one vertex $x$ in the path from $s$ to $t$, such that $x \in N_\epsilon^{out}(s) \cap N_\epsilon^{in}(t)$.

For 3hop, we introduce our method in high-level by following the idea of query processing proposed in~\cite{}.
Let us assume the local gate vertex sets $N_\epsilon^{out}(s)$ and $N_\epsilon^{in}(t)$ have been extracted.
As we know, chain generated by graph decomposition is used as intermediate hop to serve the communication between source and destination,
as highway in the transportation system.
To tell if vertex $s$ can reach vertex $t$ in the graph, our query scheme generally consists of three steps:

\noindent 1) we collect the entry points $X$ on intermediate chains which can be reached by $s$ through its local gate vertex set;

\noindent 2) we collect the exit points $Y$ on intermediate chains which can reach $t$ through its local gate vertex set;

\noindent 3) we check if there is a pair $(x,y)$ such that $x \in X$, $y \in Y$ and $x$ can reach $y$ in one chain. If so, we say $x \rightarrow y$.
Otherwise, $y$ is not reachable from $x$.

The algorithm is quite similar to the 3hop contour query processing algorithm stated in the original paper.
The difference is that each entry point $x \in X$ is the smallest vertices in its chain which can be reached by all vertices in $N^{out}_\epsilon(s)$ through their out-anchor vertex
instead of only source $s$.

\subsection{Improvement on Indexing-based Query}
\label{improveindexquery}

Clearly, local gate vertex sets can be precomputed and stored to improve the performance of online processing by sacrificing some memory cost.
Another question is that do we need to broadcast the indices of local gate vertex set as well?
That is, for each vertex $u$, should we explicitly record all indices of local gate vertices instead of only gate vertices?
Supposing any pair of vertices has equal probability to be queried,
our goal is to select a set of vertices whose online cost is most expensive and precomputation can significantly improve their query performance.
To proceed, we first define an unified measure to evaluate the saving of each vertex achieved by precomputation as follows.
\beqnarr
S(u) = \sum_{x \in TC(u)} N^{in}_\epsilon(x) \nonumber
\eeqnarr
}


\comment{

In Subsection~\ref{online}, we will describe how we can 
For instance, to test whether vertex $1$ can reach vertex $2$, then, we need to test whether $\{3,5\}$ can reach $\{5,6\}$, where $B_{out}^2(1)=\{3,5\}$ and $B_{in}^2(2)=\{5,6\}$. 


First, we perform   {\em local gate vertex sets} $N^{out}_\epsilon(u) = \{x | u \rightarrow x, x \in V^\prime \mbox{ and } d(u,x) \le \epsilon \}$ and $N^{in}_\epsilon(u)=\{y | y \rightarrow t, y\in V^\prime \mbox{ and } d(y,u)\le \epsilon \}$.
The query procedure is composed of two steps: local gate vertices collection and reachability checking.
In the first step, we start from source $s$ and destination $t$, and try to collect the vertex set $N^{out}_\epsilon(s)$ and $N^{in}_\epsilon(t)$.
They can easily be collected by BFS.
Then, we need to check the reachability of every pair of vertices $(x,y)$ ($x\in N^{out}_\epsilon(s)$ and $y \in N^{in}_\epsilon$) only in the gate graph.
We say $s$ cannot reach $t$ if and only none vertex pair is reachable in the gate graph.



In other words, 

\subsection{Online Query}
\label{onlinequery}

In the following, we introduce the basic query answering scheme purely using gate graph.
That is, no indexing approach is employed.
Clearly, this is the most memory-efficient way as no index is assigned to each vertex,
however, this query performance would become slow compared to the approach utilizing graph indexing.

As discussed in the previous subsection, one of paths between any ``non-local'' vertex pair $(s,t)$ is guaranteed to be recovered.
Along this line, our online query processing actually tries to restore such paths $P_{s,t} = (s,u_1,..., u_k, t)$,
where distance between any two consecutive vertices is no greater than $\epsilon$,
and all vertices except source and target are gate vertices.
According to the definition of gate graph, we can see that subpath $P_{u_1,u_k}$ should exist in the gate graph.
Therefore, the main idea is to check whether there is a path $P_{u,v}$ in the gate graph such that $u$ can be reached from $s$ locally and $t$ is reachable from $v$ locally (i.e., $d(s,u) \le \epsilon$ and $d(v,t) \le \epsilon$).
If not, we can say $s$ cannot reach $t$ in the original graph.
It is not hard to see that the checking procedure can be achieved using any traverse method, like depth-first-search (DFS) or breath-first-search (BFS).


}

}

\comment{
prune all the vertices in $B^\epsilon_{out}(u)$ (or $B^\epsilon_{out}(v)$) which are visited by the local BFS only when one of their 
accessvertex


collecting gate vertices and online reachability checking.
To address this issue, two techniques are proposed to avoid fully online processing and eventually speedup the query.
For each vertex, the first method, namely gate materialization, is to explicitly record the gate vertices within $\epsilon$ steps away (precompute Line 1 in Algorithm~\ref{alg:onlinequery}).
The second method is to reduce the times of pairwise reachability checking by incorporating quick rejection idea from GRAIL~\cite{} (speedup Line 2 to 8 in Algorithm~\ref{alg:onlinequery}).


\noindent{\bf 1) Gate Materialization: }
Two strategies are considered in this method: full gate materialization and partial gate materialization.
In the first strategy, for each vertex $u$, we perform local BFS within $\epsilon$ steps to collect $N^{out}_\epsilon(u)$ and $N^{in}_\epsilon(u)$.
The basic idea of partial gate materialization strategy is that, instead of storing all vertices' local gate vertex set, we only explicitly record some vertices' local gate vertex set, where their gate vertices' size is no larger than certain value.
Especially, given a threshold $k$, we only collect vertex $u$'s $N^{out}_\epsilon(u)$ and $N^{in}_\epsilon(u)$ if  $|N^{out}_\epsilon(u)| \le k$ and $|N^{in}_\epsilon(u)| \le k$.
For remaining vertices, we still apply online collection process.
}



==> Figures/ApproxTree.tex <==
\begin{algorithm}
\caption{Approximate-Tree($G$, $T^{-1}$)}
\label{alg:approxst}
\begin{algorithmic}[1]
\STATE $S \leftarrow SampleVertices(V,n)$;
\STATE $V \leftarrow \mbox{Topological Order of} G$; \COMMENT{Perform topological sort of $G$}
\FOR{$i=1$ to $|V|$}
    \STATE $pred(v_i) \leftarrow \emptyset$;
    \IF{$v_i \in S$}
        \STATE $pred(v_i) \leftarrow \{v_i\}$;
    \ENDIF
    \FORALL{$e \in E(G)$ \{where $e=(u,v_i)$\}}
        \STATE $pred(v_i) \leftarrow pred(v_i) \cup pred(u)$;
    \ENDFOR
\ENDFOR
\STATE $T \leftarrow \emptyset$;
\FOR{$i=1$ to $N$}
    \STATE let $I$ be the immediate predecessors of $V[i]$ in $G$;
    \STATE $u \leftarrow argmax_{v \in I} |pred(V[i]) \cap pred(v) |$;
    \STATE add edge $u \rightarrow V[i]$ into $T$;
\ENDFOR
\RETURN spanning tree $T$;
\end{algorithmic}
\end{algorithm}


==> Figures/CHTree.tex <==
\begin{algorithm}
\caption{Chernoff-Hoeffding-Tree($G$, $T^{-1}$)}
\label{alg:sampling}
\begin{algorithmic}[1]
\STATE $n \leftarrow 0$ \COMMENT{$n_0$ is the initial sample size}
\REPEAT
    \STATE $S \leftarrow SampleVertices(V,n_0)$ \COMMENT{sample $n_0$ vertices in $V$}
    \STATE $n \leftarrow n + n_0$ \COMMENT{$n$ is the total number of samples}
    \FORALL{$v_i \in S$}
        \STATE $succ(v_i) \leftarrow \emptyset$;
        \STATE $SingleTC(T^{-1}, v_i, succ(v_i))$;
        \FORALL{$u \in succ(v_i)$}
            \FORALL{$v_j \in out\_edges(u)$}
                \IF{$v_j$ is not reachable from $v_i$ through $T^{-1}$}
                    \STATE $Y_{i,e} \leftarrow Y_{i,e} + 1$ where $e=(u,v_j)$;
                    \STATE Update $\sum_i Y_{i,e}$ and $\sum_e Y_{i,e}$;
                \ENDIF
            \ENDFOR
        \ENDFOR
    \ENDFOR
    \FORALL{$v_i \in V$}
        \STATE $\hat{X_{e,n}} = \frac{1}{n} \sum_i Y_{i,e}$;
    \ENDFOR
    \STATE $T \leftarrow MST(G,\hat{X_{e,n}})$;
    \FOR{$i = 1$ to $n$}
        \STATE Update $\sum_e Y_{i,e}$;
    \ENDFOR
\UNTIL{Condition \ref{condition} is satisfied}
\end{algorithmic}

\begin{algorithmic}[1]
\PROCEDURE{SingleTC($T^{-1}$, $v$, $succ$)}
\STATE $pre \leftarrow v$;
\STATE $visited(v) \leftarrow TRUE$
\FORALL{$v^\prime \in out\_edges(v)$}
     \IF{$v^\prime$ is not visited}
        \IF{$pre$ cannot reach $v^\prime$ through $T^{-1}$}
            \STATE $succ \leftarrow succ \cup \{v^\prime\}$;
        \ENDIF
        \STATE SingleTC($T^{-1}$,$v^\prime$,$succ$);
     \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> Figures/ComputeLin.tex <==
\begin{algorithm}
\caption{Compute\_Lin($G_i$, $v$, $L_{in}$, isBackbone, IDmap, epsilon)}
\label{alg:cl}
\begin{algorithmic}[1]
\STATE Perform BFS starting from $v$;
\FORALL {$u|(u,v) \in G_i$ and $distance(u,v) \leq epsilon$}
    \IF{isBackbone($u$)}
        \STATE $u \rightarrow L_{in}(v)$;
        \FORALL{$x| x \in L_{in}(u)$}
            \STATE $x \rightarrow L_{in}(v)$;
            \STATE contiue;
        \ENDFOR
    \ELSE
        \IF{$distance(u,v) \leq epsilon/2$}
            \STATE $u \rightarrow L_{in}(v)$;
        \ENDIF
        \STATE extend BFS from u;
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> Figures/ComputeSCInstance.tex <==
\begin{algorithm}
\caption{SetCoverInstConstruction($G=(V,E)$)}
\label{alg:candiateset}
\begin{algorithmic}[1]
\STATE $S \leftarrow \emptyset$; \COMMENT{$S$ is ground set}
\FORALL{$u \in V$}
    \STATE collect local neighbors $X$ with distance $\epsilon+1$;
    \FORALL{$x \in X$}
        \STATE $S \leftarrow S \cup \{(u,x)\}$;
    \ENDFOR
\ENDFOR
\FORALL{$u \in V$}
    \STATE collect incoming and outgoing $\epsilon$-neighborhood $N^\prime_\epsilon(v)$ and $N_\epsilon(v)$, respectively;
    \FORALL{$x \in N^\prime_\epsilon(v)$}
        \FORALL{$y \in N_\epsilon(v)$}
            \IF{$(x,y) \in S$}
                \STATE $C_u \leftarrow C_u \cup \{(x,y)\}$;
            \ENDIF
        \ENDFOR
    \ENDFOR
    \STATE clear $N^\prime_\epsilon(v)$ and $N^\prime_\epsilon(v)$;
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> Figures/Datasets.tex <==
\begin{table}[htbp]
\caption{Real Datasets}
\label{datasets}
\begin{tabular}{|l|r|r|r|r|}
\hline
Graph Name & \multicolumn{1}{l|}{\#V} & \multicolumn{1}{l|}{\#E} & \multicolumn{1}{l|}{DAG \#V} & \multicolumn{1}{l|}{DAG \#E} \\ \hline
AgroCyc & 13969 & 17694 & 12684 & 13408 \\ \hline
aMaze & 11877 & 28700 & 3710 & 3600 \\ \hline
Anthra & 13736 & 17307 & 12499 & 13104 \\ \hline
Ecoo157 & 13800 & 17308 & 12620 & 13350 \\ \hline
HpyCyc & 5565 & 8474 & 4771 & 5859 \\ \hline
Human & 40051 & 43879 & 38811 & 39576 \\ \hline
Kegg & 14271 & 35170 & 3617 & 3908 \\ \hline
Mtbrv & 10697 & 13922 & 9602 & 10245 \\ \hline
Nasa & 5704 & 7942 & 5605 & 7735 \\ \hline
Reactome & 3678 & 14447 & 901 & 846 \\ \hline
%string\_90\_normalized\_135146\_952940.gra & 135146 & 952939 & 14899 & 1 \\ \hline
%string\_95\_normalized\_75133\_207764.gra & 75133 & 207763 & 18105 & 1 \\ \hline
Vchocyc & 10694 & 14207 & 9491 & 10143 \\ \hline
Xmark & 6483 & 7654 & 6080 & 7028 \\ \hline
\end{tabular}
\label{}
\end{table}

==> Figures/DoubleTree.tex <==
\begin{algorithm}
\caption{DoubleTree($G$)}
\label{alg:doubletree}
\begin{algorithmic}[1]
\STATE $T \leftarrow OptimalTreeCover(G)$;
\REPEAT
    \STATE $T^{-1} \leftarrow OptimalCondReverseTreeCover(T,G)$;
    \STATE $c \leftarrow |\bigcup_{v \in V} succ(v | T, T^{-1})|$;
    \STATE $T \leftarrow OptimalCondTreeCover(T^{-1},G)$;
    \STATE $c^{-1} \leftarrow |\bigcup_{v \in V} pred(v|T^{-1},T)|$;
\UNTIL{$c \le c^{-1}$}
\RETURN $T^{-1}$ and $T$;
\end{algorithmic}
\end{algorithm}


==> Figures/DoubleTree_bak.tex <==
\begin{algorithm}
\caption{DoubleTree($G$)} \label{alg:doubletree}
\begin{algorithmic}[1]
\STATE $T \leftarrow \emptyset$; \STATE $T^{-1} \leftarrow \emptyset$; \WHILE{TRUE}
    \STATE $T^{-1} \leftarrow BuildReverseTree(T,G)$;
    \STATE let $c^{-1}$ be the compressed TC size based on $T^{-1}$;
    \STATE $T \leftarrow BuildTree(T^{-1}, G)$;
    \STATE let $c$ be the further compressed TC size based on $T$;
    \IF{$c^{-1} \le c$}
        \STATE apply interval labeling scheme on $T^{-1}$ such that each vertex is assign with two numbers as label;
        \STATE BREAK;
    \ENDIF
\ENDWHILE
\end{algorithmic}

\begin{algorithmic}[1]
\PROCEDURE{BuildTree($T^{-1}$,$G$)} \STATE $V \leftarrow \mbox{Topological Order of} G$ \COMMENT{Perform topological
sort of $G$} \STATE $N \leftarrow |V|$ \FOR{$i=1$ to $N$}
    \STATE $pred(V[i]) \leftarrow \{V[i]\}$;
    \FORALL{$v \in Parents(V[i])$}
        \FORALL{$v^\prime \in pred(v) \cup \{v\}$}
            \IF{$V[i]$ cannot be reached by $v^\prime$ in $T^{-1}$}
                \STATE $pred(V[i]) \leftarrow pred(V[i]) \cup \{v^\prime\}$;
            \ENDIF
        \ENDFOR
    \ENDFOR
\ENDFOR \COMMENT{compute compressed predecessors for each vertex} \STATE $T \leftarrow \emptyset$; \FOR{$i=1$ to $N$}
    \STATE let $S$ be the imemediate predecessors of $V[i]$ in $G$;
    \STATE $u \leftarrow argmax_{v \in S} |pred(V[i]) \cap pred(v) |$;
    \STATE add edge $u \rightarrow V[i]$ into $T$;
\ENDFOR \RETURN spanning tree $T$;
\end{algorithmic}

\begin{algorithmic}[1]
\PROCEDURE{BuildReverseTree($T$,$G$)} \STATE $V_R \leftarrow \mbox{Reversed Topological Order of} G$ \COMMENT{Perform
topological sort of $G$} \STATE $N \leftarrow |V|$ \FOR{$i=1$ to $N$}
    \STATE $succ(V_R[i]) \leftarrow \{V_R[i]\}$;
    \FORALL{$v \in Children(V_R[i])$}
        \FORALL{$v^\prime \in succ(v) \cup \{v\}$}
            \IF{$V_R[i]$ cannot reach $v^\prime$ in $T$}
                \STATE $succ(V_R[i]) \leftarrow succ(V_R[i]) \cup \{v^\prime\}$;
            \ENDIF
        \ENDFOR
    \ENDFOR
\ENDFOR \COMMENT{compute compressed successors for each vertex} \STATE $T^{-1} \leftarrow \emptyset$; \FOR{$i=1$ to
$N$}
    \STATE let $S$ be the imemediate successors of $V_R[i]$ in $G$;
    \STATE $u \leftarrow argmax_{v \in S} |succ(V_R[i]) \cap succ(v) |$;
    \STATE add edge $V_R[i] \rightarrow u$ into $T^{-1}$;
\ENDFOR \RETURN reverse tree $T^{-1}$;
\end{algorithmic}

\end{algorithm}


==> Figures/FastCover.tex <==
\begin{algorithm}
\caption{FastCover(G)}
\label{alg:fastcover}
\begin{algorithmic}[1]
\STATE sort vertices in $V$ based on certain order
\STATE $V^\ast \leftarrow \emptyset$
\FORALL{$u \in V$} 
    \IF{NOT covered($u,V^\ast$) \COMMENT{$\{u\} \times S_\epsilon(u)$ is uncovered}} 
        \STATE add $u$ to $V^\ast$
    \ENDIF    
\ENDFOR
\RETURN $V^\ast$;
\PROCEDURE{covered($u,V^\ast$)}
\STATE $depth(u)\leftarrow 0$; $distance(v) \leftarrow \epsilon+1$; 
\STATE add $u$ to $Q$ \COMMENT{priority queue $Q$ ordered by topological order}
\WHILE{$Q \neq \emptyset$}
   \STATE $v \leftarrow Q.pop()$ \COMMENT{the one with least topological order};
   \STATE $v.visited \leftarrow TRUE$;
   \STATE $N(v) \leftarrow \{w: (w,v)\in E \mbox{ and } w.visited=TRUE\}$; \COMMENT{all end vertices of incoming edges of $v$}
   \STATE $depth(v) \leftarrow \min_{w \in N(v)} depth(v)+1$;
   \IF{$v \in V^\ast$} 
       \STATE $distance(v) \leftarrow 0$ 
   \ELSE
       \STATE $distance(v) \leftarrow \min_{w \in N(v)} distance(v) +1$; \comment{each vertex's distance is initalized to be $\epsilon$}
   \ENDIF
   \IF {$depth(v)=\epsilon$ and $distance(v)\leq \epsilon$} 
       \RETURN FALSE; \COMMENT{$(u,v)$ is uncovered}
   \ENDIF
   \STATE add all $v$'s neighbors to $Q$;(if they are not in $Q$)
\ENDWHILE
\RETURN TRUE; \COMMENT{every vertex pair in $\{u\}\times S_\epsilon(u)$ is covered}
\end{algorithmic}
\end{algorithm}


==> Figures/FastReach.tex <==
\begin{algorithm}
\caption{FastReach($u$,$v$)}
\label{alg:fastreach}
\begin{algorithmic}[1]
\REQUIRE $G^\ast$ is the reachability backbone
\STATE Bidirectional online BFS search from $u$ and $v$; 
\IF {meet} \RETURN TRUE \ENDIF;            
\FORALL{$x \in \boldsymbol{\mathcal{B}}^\epsilon_{out}(u)$}
    \IF {$\mathcal{I}_v \subseteq \mathcal{I}_x$} 
        \FORALL{$y \in \boldsymbol{\mathcal{B}}^{\epsilon}_{in}(t)$}
            \IF {$\mathcal{I}_y \subseteq \mathcal{I}_x$} 
                 \IF{{\bf Reach}($x$,$y$|$G^\ast$)}
                     \RETURN TRUE;
                \ENDIF
            \ENDIF
        \ENDFOR
    \ENDIF
\ENDFOR
\RETURN FALSE;
\end{algorithmic}
\end{algorithm}


==> Figures/GroundSetwithPreselection.tex <==
    \begin{algorithm}
    \caption{PartialGroundSetConstruction($G=(V,E)$,$\epsilon$,$v$,$GS$)}
   \label{alg:partialgset}
    \begin{algorithmic}[1]
    \STATE $L \leftarrow \emptyset$; $Q \leftarrow \{v\}$ \COMMENT{queue for BFS};
    \STATE $GS[v] \leftarrow \emptyset$;
    \FORALL{$x \in V$}
        \STATE $life(x)\leftarrow \infty$;
        \STATE $depth(x)\leftarrow \infty$;
    \ENDFOR
    \STATE $depth(v) \leftarrow 0$;
    \WHILE{$Q \neq \emptyset$}
        \STATE $u \leftarrow Q.pop()$ \COMMENT{pop done in topological order};
        \IF {$life(u)==\epsilon$ }
             \STATE continue;
        \ENDIF
        \IF {$isgate(u)\mbox{  } \&\& \mbox{  }1 < depth(u)\leq \epsilon$ }
             \STATE $life(u) \leftarrow 0$;
        \ENDIF
        \IF {$depth(u)==\epsilon+1 \mbox{  }\&\& \mbox{  }life(u)==\infty$ }
             \STATE $L.push(u)$;
             \STATE continue;
        \ENDIF
        \FORALL{$w \in Neighbor(u)$ \COMMENT{$(u,w) \in E$}}
            \IF{$depth(u)+1 < depth(w)$}
                \STATE $depth(w)=depth(u)+1$;
            \ENDIF
            \IF{$life(u)+1 < life(w)$}
                \STATE $life(w)=life(u)+1$;
            \ENDIF
            \IF{$w$ is not visited}
                \STATE $Q.push(w)$;
            \ENDIF
        \ENDFOR
    \ENDWHILE
    \FORALL{$x \in L$}
        \STATE $GS[v].push(x)$;
    \ENDFOR
    \end{algorithmic}
    \end{algorithm}


==> Figures/HierarchyExample.tex <==
\begin{figure*}[t!]
    \label{fig:hierarchyexample}
    \centering
    \mbox{
        \subfigure[Original Graph]{\includegraphics[scale=0.2]{Figures/so2.eps}\label{graph}}
        \hspace{5mm}
        \subfigure[Second Level]{\includegraphics[scale=0.18]{Figures/so1.eps}\label{level2}}
        \hspace{5mm}
        \subfigure["Core" Graph]{\includegraphics[scale=0.13]{Figures/so0.eps}\label{core}}
        \hspace{5mm}
        \subfigure[Lin/Lout Labeling]{\includegraphics[scale=0.2]{Figures/soAllHRTidx.eps}\label{labeling}}
    }
    \vspace*{-1.0ex}
    \caption{{\small Example of building Hierarchy}}
\end{figure*}

Figure 1 shows an example of building the Hierarchy. In the given graph (a) we choose a set of vertices as Backbone $V^{*}$ so that for any pair of vertices $u$ and $v$ with distance $d(u,v) = \epsilon$, there is at least one vertex $x \in V^{*}$, such that $u \rightarrow x$ and $x \rightarrow v$ with $d(u,x) \leq \epsilon$ and $d(x,v) \leq \epsilon$. Then we build the subgraph (b) with vertices  $V^{*}$, and there's an edge from $u$ to $v$ $\iff$ $u$ can reach $v$ in the original graph (a).

We repeat above step until the generated graph cannot be scale up anymore, then we get that we call a "core" graph (c).



==> Figures/HierarchyTwohop.tex <==
\begin{algorithm}
\caption{HierArchyTwoHop($G$)}
\label{alg:ht}
\begin{algorithmic}
\WHILE{$G_i$ can be further scaled up by $FastCover$}
    \STATE Add $G_i$ to graQ;	//graQ stores the hierarchical graphs
    \STATE Generate IDmap between vertex ids in original graph $G$ and $G_i$;
    \STATE Add IDmap to mapQ;	//mapQ stores the id reference between $G$ and $G_i$
\ENDWHILE
\STATE Generate ComputeOrder based on topological order and the highest level certain vertex is on;            								\STATE Initial $L_{in}/L_{out}$ lists;
\FORALL{$G_i \in $ graQ}
    \STATE MarkBitVector(isBackbone, IDmap);
    \IF{$G_i$ is the "core" graph}
        \STATE Assign labels by 2HOP algorithm on $G_i$;
    \ELSE
        \STATE IDmap $\leftarrow$ mapQ.back();
        \FORALL{$v \in computeOrder | v \in currentLevel$}
            \STATE computeLin($G_i, v, L_{in}, isBackbone, IDmap, epsilon$);
        \ENDFOR
        \FORALL{$u \in computeOrder | u \in currentLevel$}
            \STATE computeLout($G_i, u, L_{out}, isBackbone, IDmap, epsilon$);
        \ENDFOR
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

Given $K$ levels of Hierarchy, since using $FastCover$ to discover Backbone structure on one level is $O(\sum_{u \in V} |N_\epsilon(u)|\log|N_\epsilon(u)|
+ |E_\epsilon(u)|)$, the total computational complexity of building this Hierarchy is $O(\sum_{G_K \in graQ}\sum_{u \in V_K} |N_{(G_K,\epsilon(u))}
|\log|N_{(G_K,\epsilon(u))}| + |E_{(G_K,\epsilon(u))}|)$. Generate $ComputeOrder$ is dominated by the time of assign the highest level id to each vertex,
which is $O(\sum_{V_K \in G_K}\sum_{|V_K|} )$. And $computeLin$ and $computeLout$ are $O(\sum_{n \in NN_{(G_K,\epsilon(u))}} (|Lin(n)| + |Lout(n)|))$. The total cost of compute $Lin$ and $Lout$ lists are $O(\sum_{G_K \in graQ}\sum_{n \in N_{(G_K,\epsilon(u))}} (|Lin(n)| + |Lout(n)|))$. To sum up,
the overall computational complexity of $HierArchyTwoHop$ is $O(\sum_{G_K \in graQ}(\sum_{n \in N_{(G_K,\epsilon(u))}} (|Lin(n)| + |Lout(n)|) +
\sum_{u \in V_K} |N_{(G_K,\epsilon(u))}|\log|N_{(G_K,\epsilon(u))}| + |E_{(G_K,\epsilon(u))}|))$


==> Figures/LargeRealDatasets.tex <==
\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{|l|c|c||c|r|}
\hline
Dataset & $|V|$  & $|E|$ & $|V^\ast_F|$ & $|E^\ast_F|$ \\ \hline

citeseer	&	693,947	&	312,282	&	45,920	&	25,442	\\ \hline
go\_uniprot	&	6,967,956	&	34,770,235 &	137,055	&	1,436,198	\\ \hline
mapped\_100K	&	2,658,702	&	2,660,628	&		52,719	&	219,964	\\ \hline
mapped\_1M	&	9,387,448	&	9,440,404	&		184,856	&	825,950	\\ \hline
uniprotenc\_22m	&	1,595,444	&	1,595,442	&	31,909	&	31,908	\\ \hline
uniprotenc\_100m	&	16,087,295	&	16,087,293	&	467,047	&	467,046	\\ \hline
uniprotenc\_150m	&	25,037,600	&	25,037,598	&	1,046,951	&	1,046,950	\\ \hline
citeseerx	&	6,540,399	&	15,011,259 &		336,670	&	1,531,727	\\ \hline
cit-Patents	&	3,774,768	&	16,518,947 &	1,316,773	&	5,879,535	\\ \hline


\end{tabular}
}
\end{center}
\vspace*{-4.0ex}
\caption{Large Real datasets} \label{largerealdata}
\vspace*{-3.0ex}
\end{table}







==> Figures/LargeReal_EqualQuery.tex <==

\begin{table}
\resizebox{3.7in}{!} {
{\small
\begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{Dataset}&  \multicolumn{ 4}{c|}{Using Reachability Backbone} & \multicolumn{3}{c|}{Original(WithoutBackbone)}\\
 \cline{2-8}
 &
\multicolumn{1}{l|}{GRAIL-$G^\ast_F$} & 
\multicolumn{1}{l|}{IN-$G^\ast_F$} &
\multicolumn{1}{l|}{PT-$G^\ast_F$} &  
\multicolumn{1}{l|}{2HOP-$G^\ast_F$} 
& \multicolumn{1}{l|}{DFS} & \multicolumn{1}{l|}{GRAIL}
& \multicolumn{1}{l|}{IN} 
\\ \hline

citeseer	&		34.98	&	27.34	&		26.80	&		30.35	&	26.67	 &	74.02	&	12.87		\\ \hline
go\_uniprot	&		68.74	&	26.30	&		25.07	&		27.56	&	191.90	 &	116.73	&	26.74	\\ \hline
mapped\_100K	&		62.13	&	17.93	&		18.34	&		17.26	&	 154.94	&	349.51	&	6.11		\\ \hline
mapped\_1M	&		42.86	&	19.38	&		23.55	&		20.07	&	131.79	 &	405.41	&	6.47	\\ \hline
uniprotenc\_22m	&		16.69	&	17.08	&		16.39	&		16.47	&	 22.73	&	62.04	&	16.32	\\ \hline
uniprotenc\_100m&	34.89	        &	30.60	&		37.51	&		722.85	&	 34.77	&	112.54	&	21.29		\\ \hline
uniprotenc\_150m&	55.40	        &	81.30	&		---	&		---	&	40.63	&	117.05	&	 37.07		\\ \hline
citeseerx	&		1475.00	&       36.84	&		---	&		---	&	38183.80	&	2148.26	&	 11.33		\\ \hline
cit-Patents	&		528.31	&	109.58	&		---	&		---	&	7449.32	&	556.58	&	 ---		\\ \hline

\end{tabular}
}
}
\vspace{-2.0ex}
\caption{{\small Query Time(ms) on Equal Query of Large Real Graphs}}
\vspace*{-3.0ex}
\label{largerealequalquery}
\end{table}







==> Figures/LargeReal_RandomQuery.tex <==
\begin{table}
\resizebox{3.7in}{!} {
{\small
\begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{Dataset}&  \multicolumn{ 4}{c|}{Using Reachability Backbone} & \multicolumn{3}{c|}{Original(WithoutBackbone)}\\
 \cline{2-8}
 &
\multicolumn{1}{l|}{GRAIL-$G^\ast_F$} & 
\multicolumn{1}{l|}{IN-$G^\ast_F$} &
\multicolumn{1}{l|}{PT-$G^\ast_F$} &  
\multicolumn{1}{l|}{2HOP-$G^\ast_F$} 
& \multicolumn{1}{l|}{DFS} & \multicolumn{1}{l|}{GRAIL}
& \multicolumn{1}{l|}{IN} 
\\ \hline

citeseer	&		10.17	&	9.81	&		9.72	&		9.67	&	22.39	 &	74.06	&	11.38	\\ \hline
go\_uniprot	&		18.97	&	18.13	&		16.13	&		17.17	&	252.83	 &	92.85	&	20.58		\\ \hline
mapped\_100K	&		10.14	&	9.91	&		9.42	&		9.42	&	 11.56	&	396.57	&	8.78	\\ \hline
mapped\_1M	&		11.89	&	12.32	&		12.47	&		13.20	&	12.07	 &	406.03	&	6.93		\\ \hline
uniprotenc\_22m	&		15.00	&	14.47	&		14.55	&		13.65	&	 26.24	&	83.33	&	16.21		\\ \hline
uniprotenc\_100m&	23.77	        &	22.69	&		21.26	&		23.91	&	 39.99	&	96.43	&	25.46	\\ \hline
uniprotenc\_150m&	46.40	        &	75.09	&		---	&		---	&	43.97	&	124.80	&	 32.18	\\ \hline
citeseerx	&		114.83	&	34.16	&		---	&	         ---	&	74121.40	&	2148.33	&	 16.60		\\ \hline
cit-Patents	&		435.32	&	78.68	&		---	&		---	&	15888.80	&	691.70	 &	---	\\ \hline

\end{tabular}
}
}
\vspace{-2.0ex}
\caption{{\small Query Time(ms) on Random Query of Large Real Graphs}}
\vspace*{-3.0ex}
\label{largerealrandomquery}
\end{table}



==> Figures/MPTree.tex <==
\begin{algorithm}
\caption{BatchOptimalTree($G$, $K$)}
\label{alg:mptree}
\begin{algorithmic}[1]
\REQUIRE $K$: Number of Total Groups; 
\STATE Assign each vertex randomly into $K$ groups, $V_1$, $V_2$, $\cdots$, $V_K$;
\FOR{$k=1$ to $K$}
    \STATE $ConditionalTC(G, k)$; \COMMENT{compute $\bigcup_{v \in V} pred(v|V_k)$}
\ENDFOR
\STATE $T \leftarrow MST(G,{\bf w})$;
\RETURN $T$;
\end{algorithmic}

\begin{algorithmic}[1]
\PROCEDURE{ConditionalTC($G$,$k$)}
\REQUIRE $k$: active group id for the current batch;
\FORALL {$v$ in $V$  following the topological order of $G$}
    \IF{$v.group\_id = k$ }
        \STATE $pred(v) \leftarrow \{v\}$; \COMMENT{only add vertices in $V_k$ to the predecessor sets}
    \ELSE 
         \STATE $pred(v) \leftarrow \emptyset$;
    \ENDIF
    \FORALL{$e=(v^\prime,v) \in E(G)$ \COMMENT{$v$'s immediate predecessors}}
        \STATE $pred(v) \leftarrow pred(v) \cup pred(v^\prime)$; 
    \ENDFOR 
\ENDFOR
\FORALL{$e=(v^\prime,v) \in E(G)$}
    \STATE $w_e \leftarrow w_e + |pred(v^\prime)|$; %\COMMENT{the cardinality of conditional transitive closure $pred(v^\prime|V_k)$}
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> Figures/MinEdgeSet.tex <==
\begin{algorithm}
\caption{ComputeInterTreePairs($T^{-1}$, $T$, $E_{T^{-1} \rightarrow T}$)}
\label{alg:minedgeset}
\begin{algorithmic}[1]
\STATE $Topo \leftarrow \mbox{Topological Order of} G$;
\STATE $Topo_R \leftarrow \mbox{Reversed Topological Order of} G$;
\STATE $E^I_{T^{-1} \rightarrow T} \leftarrow \emptyset$;
\WHILE{$E_{T^{-1} \rightarrow T} \neq \emptyset$}
    \STATE $v^\prime \leftarrow argmin_{(u,v) \in E_{T^{-1} \rightarrow T}} Topo(v)$
    \COMMENT{the vertex in $T$ that $T^{-1}$ can reach with minimal topological order};
    \STATE $S$ be the set of vertices which any pair of them cannot reach each other through $T^{-1}$ and all vertices in $S$ link to $v^\prime$ in $E_{T^{-1} \rightarrow T}$;
    \FORALL{$r \in S$}
        \STATE $E^I_{T^{-1} \rightarrow T} \leftarrow E^I_{T^{-1} \rightarrow T} \cup \{r, v^\prime\}$;
        \STATE $E_{T^{-1} \rightarrow T} \leftarrow E_{T^{-1} \rightarrow T} \setminus \{(r,v^\prime)\}$
        \COMMENT{Remove all edges which cross $(r, v^\prime)$};
    \ENDFOR
\ENDWHILE
\RETURN $E^I_{T^{-1} \rightarrow T}$;
\end{algorithmic}
\end{algorithm}


==> Figures/MultiSamplingTree.tex <==
\begin{algorithm}
\caption{OptimalTreeCover($G$)}
\label{alg:opttreecover}
\begin{algorithmic}[1]
\STATE topological sort $G$;
\FORALL {$v$ in $V$  following the topological order of $G$}
    \STATE $pred(v) \leftarrow \emptyset$;
    \FORALL{$(v^\prime, v) \in E(G)$ \comment{$v$'s immediate predecessors}}
        \STATE $pred(v) \leftarrow pred(v) \cup pred(v^\prime)$;
    \ENDFOR
\ENDFOR
\FORALL{$e \in E(G)$ \{where $e=(v^\prime,v)$\}}
    \STATE $w_e \leftarrow |pred(v^\prime)|$; 
\ENDFOR
\STATE $T \leftarrow MST(G,{\bf w})$; \COMMENT{compute maximal spanning tree of weighted DAG $G$}
\RETURN $T$;
\end{algorithmic}
\end{algorithm}


==> Figures/OnlineQuery.tex <==
\begin{algorithm}
\caption{BasicReach($u$,$v$)}
\label{alg:onlinequery}
\begin{algorithmic}[1]
\REQUIRE $G^\ast$ is the reachability backbone
\STATE perform two BFS to compute $B^\epsilon_{out}(u)$ and $B^\epsilon_{in}(v)$; 
\FORALL{$x \in B^{\epsilon}_{out}(u)$}
    \FORALL{$y \in B^{\epsilon}_{in}(t)$}
        \IF{{\bf Reach}($x$,$y$|$G^\ast$)}
            \RETURN TRUE;
        \ENDIF
    \ENDFOR
\ENDFOR
\RETURN FALSE;
\end{algorithmic}
\end{algorithm}


==> Figures/OnlineSearch.tex <==
\begin{algorithm}
\caption{OnlineReach($u$,$v$)}
\label{alg:onlinequery}
\begin{algorithmic}[1]
\REQUIRE $G^\ast$ is the reachability backbone
\STATE perform reversed BFS and $B^\epsilon_{in}(v)$; 
\FORALL{$x \in B^{\epsilon}_{out}(u)$}
    \FORALL{$y \in B^{\epsilon}_{in}(t)$}
        \IF{{\bf Reach}($x$,$y$|$G^\ast$)}
            \RETURN TRUE;
        \ENDIF
    \ENDFOR
\ENDFOR
\RETURN FALSE;
\end{algorithmic}
\end{algorithm}


==> Figures/OptimalOracle.tex <==
\begin{algorithm}
\caption{Optimal\_ScalableOracle(G)}
\label{alg:cl}
\begin{algorithmic}[1]
\STATE Rank vertices in G by $(indegree + 1)*(outdegree + 1)$ in descending order;
\STATE Initial inhibit list;
\FORALL {$u_i \in G$}
    \STATE Set $inhibit_{in}(u_i)$ based on $L_{out}(u_i)$, and $inhibit_{out}(u_i)$ based on $L_{in}(u_i)$;
    \STATE Perform BFS starting from $u_i$, and for each visited vertex $v_j$;
    \IF{$rank(v_j) \leq rank(u_i)$ or $\exists x \in L_{out}(v_j)/L_{in}(v_j)|x \in inhibit_{out}(u_i)/inhibit_{in}(u_i)$}
        \STATE Do not add $u_i$ into $L_{out}(v_j)/L_{in}(v_j)$, nor extend BFS from $v_j$;
    \ELSE
        \STATE Add $u_i$ into $L_{out}(v_j)/L_{in}(v_j)$, extend BFS from $v_j$;
    \ENDIF
    \STATE reset inhibit;
\ENDFOR
\end{algorithmic}
\end{algorithm}

As you can tell from the pseudocode that the main difference between intuitive and optimal ScalableOracle is the initialization of inhibit lists. Even though the overall time complexity of $Optimal\_LinLout$ in worst case is still $O(|V||E|)$, the time cost of BFS for initializing inhibit lists is saved.


==> Figures/OptimalReverseTree.tex <==
\begin{algorithm}
\caption{OptimalCondReverseTreeCover($T$,$G$)}
\label{alg:optreversetree}
\begin{algorithmic}[1]
\STATE topological sort $G$;
\COMMENT{Step 1: Compute compressed successor set}
\FORALL{$v$ in $V$ following the reverse topological order of $G$}
    \STATE $succ(v|T) \leftarrow \emptyset$;
    \FORALL{$(v,v^\prime) \in E(G) $ ($v$'s immediate successors)}
        \FORALL{$x \in succ(v^\prime | T) \cup \{v^\prime\}$}
            \IF{$v$ cannot reach $x$ in $T$}
                \STATE $succ(v|T) \leftarrow succ(v|T) \cup \{x\}$;
            \ENDIF
        \ENDFOR
    \ENDFOR
\ENDFOR

\COMMENT{Step 2: Assign each edge a weight}
\FORALL{$e = (v,v^\prime) \in E(G)$}
    \STATE $w_e \leftarrow |succ(v|T) \setminus succ(v^\prime|T) |$;
\ENDFOR

\COMMENT{Step 3: Compute the maximal spanning tree of weighted $G$}
\STATE $T^{-1} \leftarrow MST(G^{-1},\mathbf{w})$;
\COMMENT{$G^{-1}$ is reversed edge direction of $G$}
\RETURN $T^{-1}$;
\end{algorithmic}
\end{algorithm}


==> Figures/PathtreeQuery.tex <==
\begin{algorithm}
\caption{PathTreeQuery($s$,$t$,$G^\ast$)}
\label{alg:pathtreequery}
\begin{algorithmic}[1]
\REQUIRE $G^\ast$ is gate graph;
\STATE collect local gate vertex sets $N^{out}_\epsilon(s)$ and $N^{in}_\epsilon(t)$ from $s$ and $t$, respectively;
\STATE build the interval tree $T_s$ on intervals $\mathcal{I}_s$ of $N^{out}_\epsilon(s)$;
\FORALL{$y \in N^{in}_\epsilon(t)$}
    \IF{$y$ is reachable from  $N^{out}_\epsilon(s)$ by searching $T_s$}
        \RETURN TRUE;
    \ENDIF
\ENDFOR
\RETURN FALSE;
\end{algorithmic}
\end{algorithm}


==> Figures/Pseudocode.tex <==
\noindent {\bf Pseudocode}

Note node \{ int id; int level; list$<$int$>$ outNeigh; boolean visited; list $M_\epsilon$; list $N_\epsilon$ \};
    Graph \{ list$<$node$>$ nodeList; \} \newline

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{
            u.level$\leftarrow$ 0 \;
            $M_\epsilon(u)\leftarrow \phi$\;
            $Q\leftarrow \phi$\;
            $Q$.enqueue(u)\;
            \While{$Q\neq$ empty}{
                u$\leftarrow$ $Q$.dequeue()\;
                u.visited$\leftarrow$ true\;
                \eIf{u.level$<$$\epsilon+1$}{
                    \ForAll{v$\in$ outNeigh(u)}{
                        \If{v.visited==false}{
                            Q.enqueue(v)\;
                            $M_\epsilon(u)$.insert(v)\;
                        }
                    }
                }{
                    GroundSet(u).insert(v)\;
                }
            }
        }
        \caption{FBFS(node $u$, list$<$int$>$ $M_\epsilon$, list$<$list$<$int$>$ $>$ GroundSet) }
        \label{alg3}
    \end{algorithm}

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{
            u.level$\leftarrow$ 0 \;
            $N_\epsilon(u)\leftarrow \phi$\;
            $Q\leftarrow \phi$\;
            $Q$.enqueue(u)\;
            \While{$Q\neq$ empty}{
                u$\leftarrow$ $Q$.dequeue()\;
                u.visited$\leftarrow$ true\;
                \eIf{u.level$<$$\epsilon+1$}{
                    \ForAll{v$\in$ outNeigh(u)}{
                        \If{v.visited==false}{
                            Q.enqueue(v)\;
                            $N_\epsilon(u)$.insert(v)\;
                        }
                    }
                }{

                }
            }
        }
        \caption{RBFS(node $u$, list$<$int$>$ $N_\epsilon$) }
        \label{alg3}
    \end{algorithm}

 %   \newpage

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{

                    \ForAll{u$\in$ V(G)}{
                        FBFS(u,$M_\epsilon(u)$,GroundSet)\;
                    }
                    \ForAll{u$\in$ V($G'$)}{
                        RBFS(u,$N_\epsilon(u)$)\;
                    }

        }
        \caption{Calculate$M_\epsilon$ $N_\epsilon$(Graph $G$, Reverse Graph $G'$)}
        \label{alg3}
    \end{algorithm}

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{
                    int total$\leftarrow$ 0\;
                    \ForAll{m $\in$ $M_\epsilon(u)$}{
                        \ForAll{m $\in$ $M_\epsilon(u)$}{
                            \If{GroundSet(m).find(v)==true \&\& Covered[m][n]=false}{
                                total++\;
                            }
                        }
                    }
                    return total\;
        }
        \caption{CalculatePotential(node u, GroundSet)}
        \label{alg3}
    \end{algorithm}


    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{
                    \ForAll{m $\in$ $M_\epsilon(u)$}{
                        \ForAll{m $\in$ $N_\epsilon(u)$}{
                            \If{GroundSet(m).find(v)==true}{
                                Covered[m][n]=true;
                            }
                        }
                    }

        }
        \caption{Cover(u,GroundSet,Covered)}
        \label{alg3}
    \end{algorithm}


    candidate\{int id, int potential\};

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{
                    list$<$candidate$>$ potentialList\;
                    \ForAll{u $\in$ V(G)}{
                        potentialList$\leftarrow$candidate(u,CalculatePotential(u, GroundSet)))\;
                    }
                    sort(potentialList, 1,$|V|$)\;
                    \For{i$\leftarrow$ 1 to $|V|$}{
                        candidate c $\leftarrow$ potentialList.get(i)\;
                        Cover(c.u, GroundSet, Covered)\;
                        int max$\leftarrow -\infty$\;
                        \For{j$\leftarrow$ i+1 to |V|}{
                            candidate d $\leftarrow$ potentialList.get(j)\;
                            \eIf{max$>$d.potential}{
                                break\;
                            }{
                                int newPotential$\leftarrow$ CalculatePotential(d.u, GroundSet)\;
                                d.potential $\leftarrow$ newPotential\;
                                \If{newPotential>max}{
                                    max$\leftarrow$ newPotential\;
                                }
                            }
                        }
                        sort(potentialList, i+1,j)\;
                        \If{Covered all true}{
                            break;
                        }
                    }

        }
        \caption{SetCover(GroundSet,G)}
        \label{alg3}
    \end{algorithm}

\comment{ \noindent{\bf Graph Simplification}

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{
                    $G_T\leftarrow$  TOPOLOGICAL-SORT($G$)\;
                    \ForAll{u $\in$ V(G)in TOPOLOGICAL ORDER}{
                        Edge-Reduction(u,$G_T$)\;
                    }


        }
        \caption{GraphSimplification(G)}
        \label{alg3}
    \end{algorithm}


    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{

                    \ForAll{m $\in$ u.InNeigh}{
                        \ForAll{n $\in$ u.InNeigh}{
                            \If {TC(m).find(n)==true}{
                                u.InNeigh.delete(n)\;
                            }
                        }
                    }
                    \ForAll{v $\in$ u.InNeigh}{
                        TC(u)$\leftarrow \phi$\;
                        \eIf{(v,u)==$G_T$.lastEdge(v)}{
                            TC(u)=TC(u)$\cup$TC(v)\;
                            delete(TC(v))\;
                            Mark(v)\;
                        }{
                            TC(u)=TC(u)$\cup$TC(v)$\cup$\{v\}\;
                        }
                    }

        }
        \caption{Edge-Reduction(Node n,$G_T$)}
        \label{alg3}
    \end{algorithm}

    For reducing redundant edges, we employ the \emph{Edge-Reduction()} procedure for each vertex $u$ in topological order. For every vertex $u$, all incoming vertices are considered for redundancy. If an incoming vertex $n$ is already contained in the TC of another incoming vertex $m$, then the edge (n,u) is snubbed. Then we merge the TC of the remaining incoming vertices to produce the TC for $u$.
}

\noindent {\bf Gate Graph Construction:}

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        \Begin{
            map$<$int,int$>$ Mapping, inverseMapping\;
            \ForAll{v $\in$ $V^*$(G)}{
                index = createNode()\;
                Mapping[v]=index\;
                inverseMapping[index]=v\;
            }
            \ForAll{v$\in$ $V^*$(G)}{
                BFS$V^*$(v,isgate)\;
            }
        }
        \caption{$G^*$Construct( List $V^*(G)$, vector<int,int> isgate,int $\epsilon$)}
        \label{alg3}
    \end{algorithm}

    \begin{algorithm}
        \SetAlgoLined
        \KwData{node $u$}
        %\kwResult{Reachability}
        \Begin{
            u.level$\leftarrow$ 0 \;
            $Q\leftarrow \phi$\;
            $Q$.enqueue(u)\;
            \While{$Q\neq$ empty}{
                u$\leftarrow$ $Q$.dequeue()\;

                \eIf{u.level$<$$\epsilon$}{
                    \ForAll{m$\in$ outNeigh(u)}{
                        \If{v.visited==false}{
                            m.level = u.level+1\;
                            m.visited$\leftarrow$ true\;
                            Q.enqueue(m)\;
                            if{isgate(m)==true}{
                                addEdge(Mapping(v),Mapping(m))\;
                            }
                        }
                    }
                }{

                }
            }
        }
        \caption{BFS$V^*$(node $v$, vector$<$boolean$>$ isgate, Map$<$int,int$>$ Mapping) }
        \label{alg3}
    \end{algorithm}


==> Figures/Query.tex <==
\begin{algorithm}
\caption{Query($u$, $v$)}
\label{alg:query}
\begin{algorithmic}[1]
\REQUIRE $T^{-1}$ and $T$ are extracted reverse tree and spanning tree of DAG $G$;
\REQUIRE all {\em Inter-tree Pairs} are organized in the kd-tree of four dimensional space;

\STATE $R_1 \leftarrow [1, x_u^{-1}]$;
\STATE $R_2 \leftarrow [y_u^{-1}, |V|]$;
\STATE $R_3 \leftarrow [1, x_v]$;
\STATE $R_4 \leftarrow [y_v, |V|]$;
\STATE Finding all points indicating inter-tree pairs $(u^\prime, v^\prime)$ in four dimensional space, such that the points are in the range $R_1$, $R_2$, $R_3$ and $R_4$, and store them in the set $S$;
\IF{|S| > 0}
    \RETURN TRUE;
\ENDIF
\RETURN FALSE;
\end{algorithmic}
\end{algorithm}


==> Figures/ScalableoracleExample.tex <==
\begin{figure*}[t!]
    \label{fig:scalabeloracleexample}
    \centering
    \mbox{
        \subfigure[Labeling start from 13]{\includegraphics[scale=0.25]{Figures/soSOidx1.eps}\label{label13}}
        \hspace{5mm}
        \subfigure[Labeling start from 7]{\includegraphics[scale=0.25]{Figures/soSOidx2.eps}\label{label7}}
        \hspace{5mm}
        \subfigure[Labeling start from 25]{\includegraphics[scale=0.25]{Figures/soSOidx3.eps}\label{label25}}
    }
    \vspace*{-1.0ex}
    \caption{{\small Example of Optimal Scalableoracle labeling}}
\end{figure*}

Figure 2 shows an example of the optimal scalable oracle. Where we start labeling from the vertex 13, which has the highest $(indegree + 1)*(outdegree + 1)$ score. Vertex 13 assign it's id to the $L_{in}$ lists of the vertices that it can reach by out-going edges, and to the $L_{out}$ lists of the vertices that it can reach by in-coming edges.

Then we start labeling from vertex 7, which rank the second. Since $L_{out}(7) = {13}$, $inhibit_{in}(7) = {13}$. consequently, when the BFS performed from 7 by out-going edges reached 12, as $L_{in}(12) = {13}$, 7 will not be added into $L_{in}(12)$.

The above steps are repeated until all the vertices are computed. And we will have our final index as shown on (d).



==> Figures/SimpleQuery.tex <==
\begin{algorithm}
\caption{Query($u$,$v$)}
\label{alg:simplequery}
\begin{algorithmic}[1]
\STATE let $P_v$ be the reversed path of spanning tree $T$ starting from root to vertex $v$;
\FORALL{$v^\prime \in P_v$}
    \FORALL{$r \in L(v^\prime)$}
        \IF{$u$ can reach $r$ in $T^{-1}$}
            \RETURN TRUE;
        \ENDIF
    \ENDFOR
\ENDFOR
\RETURN FALSE;
\end{algorithmic}
\end{algorithm}


==> Figures/SmallRealDatasets.tex <==
\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{|l|c|c|c|c|c|r|}
\hline
Dataset & $|V|$  & $|E|$ & $|V^\ast_S|$ & $|E^\ast_S|$ & $|V^\ast_F|$ & $|E^\ast_F|$ \\ \hline

agrocyc	&	12684	&	13408	&	185	&	307	&	410	&	587	\\ \hline
anthra	&	12499	&	13104	&	182	&	292	&	410	&	549	\\ \hline
arXiv	&	6000	&	66707	&	1620	&	42789	&	3191	&	7684	\\ \hline
citeseer	&	10720	&	44258	&	1300	&	4786	&	3951	&	8808	\\ \hline
ecoo	&	12620	&	13350	&	190	&	317	&	409	&	589	\\ \hline
go	&	6793	&	13361	&	1165	&	2499	&	1761	&	3182	\\ \hline
kegg	&	3617	&	3908	&	185	&	187	&	487	&	495	\\ \hline
mtbrv	&	9602	&	10245	&	175	&	306	&	407	&	557	\\ \hline
nasa	&	5605	&	7735	&	938	&	1178	&	1010	&	1467	\\ \hline
pubmed	&	9000	&	40028	&	642	&	3111	&	1899	&	8574	\\ \hline
vchocyc	&	9491	&	10143	&	162	&	268	&	408	&	560	\\ \hline
xmark	&	6080	&	7028	&	780	&	1308	&	744	&	1299	\\ \hline
yago	&	6642	&	42392	&	190	&	697	&	1002	&	4057	\\ \hline

\end{tabular}
}
\end{center}
\vspace*{-4.0ex}
\caption{Small Real datasets} \label{realsmalldata}
\vspace*{-2.0ex}
\end{table}




==> Figures/TCcovExample.tex <==
\begin{figure}[t!]
    \label{fig:exampleofBL}
    \centering
    \mbox{
        \includegraphics[scale=0.2]{Figures/TCcov.eps}\label{TCcov}
    }
    \vspace*{-1.0ex}
    \caption{{\small Example of Basic Labeling}}
\end{figure}



==> Figures/Transform.tex <==
\begin{algorithm}[h]
\caption{Transform($T$)}
\label{alg:transform}
\begin{algorithmic}[1]
\STATE Perform interval labeling on $T$ and assign each vertex $u$ with interval $[x_u, y_u]$;
\STATE $E \leftarrow \emptyset$;
\STATE $NE \leftarrow \emptyset$;
\STATE $T^\prime \leftarrow \emptyset$;
\STATE $PostOrder(root(T), T, E, NE, T^\prime)$;
\RETURN $T^\prime$;
\end{algorithmic}

\begin{algorithmic}[1]
\PROCEDURE{PostOrder($v$, $T$, $E$, $NE$, $T^\prime$)}
\REQUIRE $E$ is a stack recording visited vertices with empty label set;
\REQUIRE $NE$ is a stack recording visited vertices with non-empty label set;
\IF{$v == NULL$}
    \STATE RETURN;
\ENDIF
\FORALL{$u \in Children(v)$}
    \STATE PostOrder($u$, $T$, $E$, $NE$, $T^\prime$);
\ENDFOR
\STATE $visited(v) \leftarrow TRUE$;
\IF{$|Label(v)| > 0$}
    \WHILE{$NE \neq \emptyset$}
        \STATE $u \leftarrow NE.pop()$;
        \STATE add edge $(v, u)$ to transformed tree $T^\prime$;
    \ENDWHILE
    \WHILE{$E \neq \emptyset$}
        \STATE $u \leftarrow E.pop()$;
        \STATE add edge $(v, u)$ to transformed tree $T^\prime$;
    \ENDWHILE
    \STATE $NE \leftarrow NE \cup \{v\}$;
\ELSE
    \STATE $E \leftarrow E \cup \{v\}$;
\ENDIF
\end{algorithmic}

\end{algorithm}


==> Figures/TreecoverQuery.tex <==
\begin{algorithm}
\caption{TreeCoverQuery($s$,$t$,$G^\ast$)}
\label{alg:treecoverquery}
\begin{algorithmic}[1]
\REQUIRE $G^\ast$ is gate graph;
\STATE collect local gate vertex sets $N^{out}_\epsilon(s)$ and $N^{in}_\epsilon(t)$ from $s$ and $t$, respectively;
\STATE sort the intervals $\mathcal{I}_s$ of $N^{out}_\epsilon(s)$ and the intervals $\mathcal{I}_t$ of $N^{in}_\epsilon(t)$ based on their first number;
\STATE $sind \leftarrow 0$ and $tind \leftarrow 0$;
\WHILE{$sind < |\mathcal{I}_s|$ and $tind < |\mathcal{I}_t|$}
    \IF{$\mathcal{I}_s[sind] \subseteq \mathcal{I}_t[tind]$}
        \RETURN TRUE;
    \ELSIF{$\mathcal{I}_s[sind].second < \mathcal{I}_t[tind].first$}
        \STATE $sind \leftarrow sind+1$;
    \ELSE
        \STATE $tind \leftarrow tind+1$;
    \ENDIF
\ENDWHILE
\RETURN FALSE;
\end{algorithmic}
\end{algorithm}


==> Figures/greedy.tex <==
\begin{algorithm}
\caption{greedyCover($U$,$\mathcal{G}=(A \cup B, \mathcal{E})$)}
\label{alg:greedyCover}
\begin{small}
\begin{algorithmic}[1]
\REQUIRE $U$ is the ground set and $\mathcal{G}$ is the bipartite graph for set cover.
\STATE $R \leftarrow \emptyset$;
\STATE $\mathcal{S} \leftarrow \emptyset$;
\WHILE{$R \neq U$}
    \STATE Select a node $v$ from $(A \cup B) \backslash S$ such that $\frac{1}{|S_{v}|+|Z_{v}|}$ is minimum;
    \STATE $S \leftarrow S\cup\{v\}$
    \STATE Add into $R$ new elements covered by edges induced by $v$ and $S_v$.
\ENDWHILE
\RETURN $S$
\end{algorithmic}
\end{small}
\end{algorithm}


==> Figures/syndata.tex <==
\begin{table}[!htb]
%\resizebox{\textwidth}{!} {
{\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{ 2}{c|}{$\epsilon=2$} & \multicolumn{2}{c|}{$\epsilon=3$}  & \multicolumn{2}{c|}{$\epsilon=4$} \\
 \cline{2-7}
 &
\multicolumn{1}{c|}{$|V^\ast_F|$} & \multicolumn{1}{c|}{$|E^\ast_F|$} & \multicolumn{1}{c|}{$|V^\ast_F|$} & \multicolumn{1}{c|}{$|E^\ast_F|$} &
\multicolumn{1}{c|}{$|V^\ast_F|$} & \multicolumn{1}{c|}{$|E^\ast_F|$}
\\ \hline


$SF\_1M$    &   272951  &   948147  &   191208  &   828203  &   148411  &   786808  \\ \hline
$SF\_2M$    &   550860  &   1945895 &   385357  &   1698330 &   298336  &   1613006 \\ \hline
$SF\_3M$    &   823203  &   3037757 &   577754  &   2641205 &   448956  &   2499018 \\ \hline
$SF\_4M$    &   1125023 &   4020338 &   785084  &   3490157 &   605751  &   3303259 \\ \hline
$SF\_5M$    &   1335414 &   4532958 &   907895  &   3930738 &   698639  &   3768870 \\ \hline
$SF\_6M$    &   1597084 &   5509326 &   1077552 &   4766918 &   824395  &   4567924 \\ \hline
$SF\_8M$    &   2130229 &   7348966 &   1437845 &   6413161 &   1100027 &   6199982 \\ \hline
$SF\_10M$   &   2663122 &   9191144 &   1798266 &   8025036 &   1376667 &   7760405 \\ \hline


\end{tabular}
}
%}
\vspace{-2.0ex}
\caption{Size of Reachability Backbone on Scale-Free Graphs}
\vspace*{-3.0ex}
\label{syndata}
\end{table}


==> Framework.tex <==
\section{Reachability Backbone and \\ Its Discovery}
\label{backbone}

\comment{
Let $G=(V,E)$ be a directed acyclic graph (DAG), where $V=\{1,2,..., N\}$ is the vertex set and $E \subseteq V \times V$ is the edge set of graph $G$.
We use $(u,v)$ to denote the edge from vertex $u$ to vertex $v$, and $P_{v_0,v_p}=(v_0,v_1,...,v_p)$ to denote a simple path from vertex $v_0$ to vertex $v_p$.
The length of a simple path in the graph is the number of edges in the path.
The distance from vertex $u$ to vertex $v$ in the graph $G$ is denoted as $d(u,v)$, which is the minimal length of all paths from $u$ to $v$.
In reachability indexing schemes, each vertex $u$ will be assigned with two sets of labels $L_{out}(u)$ and $L_{in}(u)$ which can be used for answering queries.
}

\subsection{Reachability Backbone Definition}
\label{definition}

The reachability backbone plays a center role in SCARAB for scaling the reachability computation. 
Intuitively,  it is designed to  a number of desired features: 
1)  first, the reachability backbone has be able to scale-down the original graphs so that the existing reachability index can be applied; 
2)  second, it has to carry sufficient topological information to help the reachability computation in the original graph; 
3)  third,  it should be easy to access for any vertex in the original graph. 
To satisfy these features, SCARAB explicitly separates the {\em local} vertex pair and {\em non-local} vertex pair, and tries to utilize the backbone for recovering the reachability for the non-local reachable pairs.  
For the local pairs, no global topological information is needed to recover their reachability and can be dealt locally. 
Furthermore, the separation measure between {\em local} and {\em non-local} vertex pairs is determined through a threshold parameter $\epsilon$ which can be used not only to facilitate the access of backbone vertices, but also to help control the backbone size. 
Formally,  given a {\em locality threshold} $\epsilon$, for any pair of vertices $u$ and $v$, if $u$ can reach $v$ within $\epsilon$ intermediate vertices, i.e., the distance between from $u$ to $v$ is no longer than $\epsilon$, then $(u,v)$ is referred to as a {\bf local pair}, and if $u$ can reach $v$ but through at least $\epsilon+1$ intermediate vertices, i.e., their distance is longer than $\epsilon$, then $(u,v)$ is referred to as a {\bf non-local pair}. 
If $u$ can not reach $v$, then, $(u,v)$ is referred to as a {\bf unreachable} pair. 
Given this, the reachability backbone is defined as follows: 

\bdefin({\bf Reachability Backbone}) 
Given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, a reachability backbone $G^\ast=(V^\ast,E^\ast)$, where $V^\ast \subseteq V$ and $E^\ast$ may contain edges not in $E$, has the following property: 
 for every non-local pair $(u,v)$ in graph $G$, iff there exists two vertices $u^\ast$ and $v^\ast$ (in $V^\ast$), such that $(u,u^\ast)$ and $(v^\ast,v)$ are both local pairs in $G$ and $u^\ast$ can reach $v^\ast$ in $G^\ast$. 
edefin

In other words,  a reachability backbone can help determine between any non-local and unreachable vertex pair through a {\em reachability join test} between $B_{out}^\epsilon(u)$ and $B_{in}^\epsilon(v)$:  
let $B_{out}^\epsilon(u)$ be all backbone vertices $u$ can reach within $\epsilon$ hops, i.e. $B_{out}^\epsilon(u)=\{
x \in V^\ast | d(u,x) \leq \epsilon\}$, and 
let $B_{in}^\epsilon(v)$ be all backbone vertices which can reach $v$ within $\epsilon$ hops, i.e., $B_{out}^\epsilon(v)=\{ y \in V^\ast | d(y,v) \leq \epsilon\}$, 
if $B_{out}^\epsilon(u) \rightarrow B_{in}^\epsilon(v)$ (meaning there exists $x \in B_{out}^\epsilon(u)$ and $y \in B_{in}^\epsilon(v)$, $x \rightarrow y$ in the backbone $G^\ast$), then $u \rightarrow v$ in $G$ and not otherwise. 
Since  the reachability backbone $G^\ast$ aims to scale-down the original graph $G$, its size should be as small as possible while still maintaining its property for reachability computation. 
Given this, we introduce the {\bf minimal reachability backbone} (MRB) discovery problem: {\em given a DAG $G=(V,E)$ and the locality threshold $\epsilon$, the minimal reachability backbone is the one with the smallest number of backbone vertices, i.e., $\arg\min_{|V^\ast|} G^\ast$. }
Note that here we utilize the number of vertices as the criterion for scaling down the original graph. 
This is because most of the very large graphs are generally very sparse and thus the number of vertices is more essential to determine the capability of reachability indexing. 
Furthermore, as we will see later that the backbone edges ($E^\ast$) can be rather easily constructed from the original graph $G$ once the backbone vertices ($V^\ast$) are determined. 



To answer the first question, we introduce the concept of reachability backbone to be the {\em minimal} graph structure (in terms of the number of vertices), which enables for any pair of vertices $\epsilon$-hops away in the original graph, both can access the backbone using only a local search  (within $\epsilon$-hops), and their corresponding access vertices are connected in the backbone. In other words, the backbone structure carries the reachability information and can be used for recovering for any non-local reachability pairs. To discover the backbone, we develop a set-cover approach which can approximate the minimal backbone with guaranteed bound and more importantly, the backbone discovery algorithm  scales almost linearly with respect to the size of the original graph. 

In this subsection, we focus on the first component aiming at generating simplified graph over original one while retaining the essential reachability information.
The goal is to significantly reduce the size of original graph and produce a small graph which can be handled by indexing algorithms in the subsequent step.
To facilitate the indexing step and query answering step, the most critical characteristics that simplified graph should hold are:
1) reachability information between pair of vertices in simplified graph should be preserved;
2) the reachability of any pair of vertices in the original graph can be easily recovered with the help of simplified graph.
Our approach is inspired by the ``gate graph'' proposed in~\cite{} to simplify graph while preserving pairwise shortest distance.
Gate graph is made up of a set of gate vertices and essential connections among them.
Given a predefined locality parameter $\epsilon$, we say any pair of vertices with distance smaller than or equal to $\epsilon$ is ``local'' pair and ``non-local'' vertex pair is defined conversely.
For any ``non-local'' vertex pair, their shortest-path distance is guaranteed to be recovered by consecutive ``local'' walks through gate vertices.
We extend this idea to reachability based simplification problem.

\subsubsection{Gate Vertex Set Discovery}
\label{gatevertexset}

In the following, we first formally define the gate vertex set discovery problem based on reachability.
After that, a efficient mining algorithm is presented to obtain the gate vertices and generate resulting gate graph.
In reachability scenario, gate vertices is considered as key intermediates to recover one path (not necessary shortest path in distance problem) of the long-range (``non-local'' vertex pair) connections in the original graph.
Smaller size of gate vertex set are able to achieve smaller index size in the subsequent processing.
Therefore, we define the minimum gate-vertex set discovery problem based on reachability as follows:

\bdefin({\bf Minimum Gate-Vertex Set Discovery (MGS) Problem})
\label{gatevertexset}
Given a DAG $G=(V,E)$ and user-defined threshold $\epsilon>0$, vertex set $V^\ast \subseteq V$ is called a gate-vertex set if $V^\ast$ satisfies the following property: for any {\bf non-local pair} $u$ and $v$ ($d(u,v) \ge \epsilon+1$),
there is a vertex sequence formed by consecutive {\bf local pairs} from $u$ to $v$, $(u,v_1,v_2, \cdots, v_k,v)$ where $v_1, v_2, \cdots, v_k \in V^\ast$, such that $d(u,v_1)\le \epsilon$, $d(v_1,v_2) \le \epsilon$, $\cdots$ , $d(v_k,v) \le \epsilon$.
The gate vertex set discovery problem seeks a set of gate vertices with smallest cardinality.
\edefin


\blemma
\label{lemma1}
Let $G$($V$,$E$) be the original graph and $V^*$ the gate vertex set.
For any $u,v \in V$ with $d(u,v)=\epsilon+1$ there exists a vertex $x\in V^*$ such that $d(u,x)\leq\epsilon$ and $d(x,v)\leq\epsilon$.
Then, for any $u,v \in V$ with $d(u,v)\geq\epsilon+1$ there exists vertices $x,y\in V^*$ such that $d(u,x)\leq\epsilon$, $d(y,v)\leq\epsilon$, and $x\rightarrow y$.
\elemma

\bproof
When $d(u,v)=\epsilon+1$, the case is trivial and $x$=$y$.
Now, let $d(u,v)>\epsilon+1$. In that case, there is a vertex $w$ such that $d(u,w)=\epsilon+1$ and $w\rightarrow v$.
Based on the postulate, we can find a vertex $x\in V^*$ such that $d(u,x)\leq\epsilon$ and $d(x,w)\leq\epsilon$.
So, the proof is reduced to $d(x,v)$. We apply the same procedure until we reach an $x$ with $d(x,v)\leq\epsilon$.
That follows the lemma.
\eproof

The above lemma allows us to transform the minimum gate-vertex set discovery problem into an instance of set cover problem.
Let $U=\{(u,v) | d(u,v) = \epsilon+1\}$ be the ground set, which includes all the non-local pairs with distance equal to $\epsilon+1$.
Each vertex $x$ in the graph is associated with a set of vertex pairs $C_x=\{(u,v) | d(u,x) \le \epsilon, d(x,v)\le \epsilon, d(u,v)=\epsilon+1\}$,
where $C_x$ includes all of the non-local pairs with distance equal to $\epsilon+1$, and $x$ is within the local incoming range of $v$ and outgoing range of $u$.
Given this, in order to discover the minimum gate-vertex set, we seek {\em a subset of vertices $V^\ast \in V$ to cover the ground set,
i.e., $U = \bigcup_{v \in V^\ast} C_v$, with the minimum cost $|V^\ast|$.}
Basically, $V^\ast$ serves as the index for the selected candidate sets to cover the ground set.

\noindent{\bf Set Cover Instance Construction: }
In order to adopt the aforementioned set-cover based algorithm to discover the gate-vertex set, we first have to generate the ground set $U$ and each candidate subset $C_x$ associating with vertex $x$.
Though we only need the non-local pairs with distance $\epsilon+1$, whose number is much smaller than all non-local pairs,
the straightforward approach still needs to find and explicitly record all vertex pair with distance no greater than $\epsilon+1$,
and then apply such information to generate each candidate set.
For large graphs, such computational and memory cost can still be rather expensive.

Here, we introduce a method to generate ground set and candidate set individually.
More importantly, we do not need to explicitly store all vertex pair with distance no greater than $\epsilon+1$.
Specifically, we first perform a local BFS for each vertex to visit its neighbors with distance no greater than $\epsilon+1$ in order to collect entire ground set.
To generate candidate set, for each vertex, we perform two BFS traversals by considering incoming edges and outgoing edges, respectively.
For each vertex $u$, let us denote $N^\prime_{\epsilon}(u)$ and $N_\epsilon(u)$ to be a set of vertices which can reach $u$ with distance no greater than $\epsilon$,
and a set of vertices which is reachable from $u$ with distance no greater than $\epsilon$.
We also call them incoming $\epsilon$-neighborhood and outgoing $\epsilon$-neighborhood.
Then, we check each vertex pair $(x,y) \in N^\prime_\epsilon(u) \times N_\epsilon(u)$ to see if it belongs to ground set.
If so, this vertex pair is appended to candidate set $C_u$.
Note that, $N^\prime_\epsilon$ and $N_\epsilon$ only serve as temporary data structure and avoid the expensive memory cost.
The procedure is outlined in Algorithm~\ref{alg:candiateset}.
The implementation utilizes bit vector to represent $N_\epsilon$ in order to speedup checking operation.

\input{Figures/ComputeSCInstance.tex}

\noindent{\bf Complexity Analysis: }
The set cover instance procedure mainly contains two parts: ground set collection and candidate set computation.
The cost of collecting ground set takes $O(\sum_{v \in V} (N_{\epsilon+1}(v)+E_{\epsilon+1}(v)))$, where $|N_{\epsilon+1}(v)|$ ($|E_{\epsilon+1}(v)|$) is the number of vertices (edges) in the $v$'s outgoing $\epsilon+1$-neighborhood.
Assuming checking the existence of $(x,y)$ in the ground set (Line 12 in Algorithm~\ref{alg:candiateset}) takes constant time by using hash table,
the candidate set computation takes $O(\sum_{v \in V}(N_\epsilon(v)+ E_\epsilon(v) + N^\prime_\epsilon(v)+ E^\prime_\epsilon(v) + N_\epsilon(v)\times N^\prime_\epsilon(v)))$ time,
where $|N^\prime_{\epsilon}(v)|$ ($|E^\prime_{\epsilon}(v)|$) is the number of vertices (edges) in the $v$'s incoming $\epsilon$-neighborhood.



\noindent{\bf Scalable Set-Cover based Discovery}
Given ground set and candidate set, the straightforward way is to apply greedy set cover algorithm to discover the gate vertex set.
However, a potential issue of this approach for handling large graph is that ground set and candidate set should be explicitly materialized,
which might be too large to be hold in the memory.
To deal with this challenge, we adopt preselecting strategy to highly reduce the size of set cover instance.

The basic idea is that some ``important'' vertices are preselected as gate vertices based on certain criteria with lower computational cost,
and then the remaining vertex pairs with distance $\epsilon+1$ which are not covered by those preselected ones will be processed in set cover framework.
In the following, two issues we have to addressed in order to make the method work:
1) how to evaluate the ``importance'' of vertex with respect to set cover framework?
2) given preselected gate vertices, how can we efficiently construct the set cover instance for remaining vertex pairs?
We focus on the first question here.
Intuitively, a vertex with a large number of incoming edges and outgoing edges has high probability to be the intermediate node of many paths.
Motivated by this intuition, we define the ``importance'' of vertex $u$ by the product of indegree $indeg(u)$ and outdegree $outdeg(u)$, i.e., $I(u) = indeg(u) \times outdeg(u)$.
We sort all vertices in the decreasing order of their importance and pick top $5\%$ vertices as gate vertices.

The second question is answered in Algorithm~\ref{alg:partialgset}.

\input{Figures/GroundSetwithPreselection.tex}


\noindent{Complexity Analysis: }
Given that the branching factor (density) of the graph is $b$, and the largest depth attainable by the algorithm is $2\alpha$, the running time complexity is $O(b^{2\alpha})$.



\subsubsection{Size of Gate Vertex Set}
\label{sizegatevertexset}

In this subsection, we discuss the upper bound of the cardinality of minimum gate-vertex set.
The notion of VC-dimension originally introduced by Vladimir Vapnik and Alexey Chervonenkis in \cite{VC1971} is widely used to measure the expressive power a set system.
To save the space, interested readers please refer to \cite{VC1971} for details.
First of all, we report our result by using VC-dimension and $\epsilon$-net theorem.

\bthm
\label{minsizebound}
Given DAG $G=(V,E)$ with locality parameter $\epsilon$,
the size of minimum gate-vertex set with respect to reachability problem is bounded by $O(\frac{|V|}{\epsilon} \log \frac{|V|}{\epsilon})$.
\ethm

As we know, authors in~\cite{} has build interesting connection between minimum gate vertex set with respect to distance problem and VC-dimension theory.
This problem tries to seek a set of vertices $V^\ast$ which are able to restore the shortest path of any ``non-local'' vertex pair by a sequence of vertices from $V^\ast$,
such that the distance of any two consecutive vertices in the sequence is no greater than $\epsilon$.
They have derived a upper bound on the size of minimum gate vertex set as follows.

\bthm
\label{distancebound}
Given graph $G=(V,E)$ with parameter $\epsilon$,
the size of minimum gate-vertex set with respect to distance problem is bounded by $O(\frac{|V|}{\epsilon} \log \frac{|V|}{\epsilon})$.
\ethm

It is not hard to see that any gate vertex set on distance problem is also a feasible solution to our reachability problem.
Therefore, the size of minimum gate vertex set on reachability problem is guaranteed to be no larger than that one on distance problem.
Furthermore, the upper bound of minimum gate vertex set on distance problem can also serve as the upper bound of minimum gate vertex set on reachability problem.
Considering those together, we say theorem~\ref{minsizebound} follows.



\subsubsection{Gate Graph Construction}
\label{gategraph}

Given those gate vertices, we can easily generate gate graph by adding the edge to each pair of vertices with distance no greater than $\epsilon$.
The following lemma guarantees that gate graph maintains the reachability information among all gate vertices.
Again, this gate graph can also be used for recovering reachability between any pair of vertices in the original graph.

\blemma
\label{lemma2}
$G^*$=($V^*$,$E^*$) is the gate graph where $u, v\in V^\ast$ and $(u,v)\in E^*$ if $d(u,v)\leq\epsilon$ in $G$.
Then for any $u, v \in V^\ast$ if reachable in G, $u\rightarrow v$ in $G^*$=($V^*$,$E^*$).
\elemma

\bproof
If $d(u,v)\leq\epsilon$, then $u\rightarrow v$ in $G^*$=($V^*$,$E^*$) by definition.
If $d(u,v)=\epsilon+1$, then based on Lemma 1, there exists a $x\in V^*$ such that $d(u,x)\leq\epsilon$ and $d(x,v)\leq\epsilon$.
So, based on the definition of $G^*$, $u\rightarrow v$. Now, if $d(u,v)>\epsilon+1$, then there is a vertex $w$ such that $d(u,w)=\epsilon+1$ and $w\rightarrow v$.
Based on Lemma 1, we can find a vertex $x\in V^*$ such that $d(u,x)\leq\epsilon$ and $d(x,w)\leq\epsilon$.
So, the proof is reduced to $d(x,v)$. We apply the same procedure until we reach a vertex $y\in V^*$ with $d(y,v)\leq\epsilon$.
Then, based on the definition of $G^*$, $u\rightarrow v$.
\eproof


\subsection{Online Query}
\label{onlinequery}

In the following, we introduce the basic query answering scheme purely using gate graph.
That is, no indexing approach is employed.
Clearly, this is the most memory-efficient way as no index is assigned to each vertex,
however, this query performance would become slow compared to the approach utilizing graph indexing.

As discussed in the previous subsection, one of paths between any ``non-local'' vertex pair $(s,t)$ is guaranteed to be recovered.
Along this line, our online query processing actually tries to restore such paths $P_{s,t} = (s,u_1,..., u_k, t)$,
where distance between any two consecutive vertices is no greater than $\epsilon$,
and all vertices except source and target are gate vertices.
According to the definition of gate graph, we can see that subpath $P_{u_1,u_k}$ should exist in the gate graph.
Therefore, the main idea is to check whether there is a path $P_{u,v}$ in the gate graph such that $u$ can be reached from $s$ locally and $t$ is reachable from $v$ locally (i.e., $d(s,u) \le \epsilon$ and $d(v,t) \le \epsilon$).
If not, we can say $s$ cannot reach $t$ in the original graph.
It is not hard to see that the checking procedure can be achieved using any traverse method, like depth-first-search (DFS) or breath-first-search (BFS).

For each vertex $u$, we have two {\em local gate vertex sets} $N^{out}_\epsilon(u) = \{x | u \rightarrow x, x \in V^\prime \mbox{ and } d(u,x) \le \epsilon \}$ and $N^{in}_\epsilon(u)=\{y | y \rightarrow t, y\in V^\prime \mbox{ and } d(y,u)\le \epsilon \}$.
The query procedure is composed of two steps: local gate vertices collection and reachability checking.
In the first step, we start from source $s$ and destination $t$, and try to collect the vertex set $N^{out}_\epsilon(s)$ and $N^{in}_\epsilon(t)$.
They can easily be collected by BFS.
Then, we need to check the reachability of every pair of vertices $(x,y)$ ($x\in N^{out}_\epsilon(s)$ and $y \in N^{in}_\epsilon$) only in the gate graph.
We say $s$ cannot reach $t$ if and only none vertex pair is reachable in the gate graph.
The algorithm is sketched in Algorithm~\ref{alg:onlinequery}.

\input{Figures/OnlineQuery.tex}


\subsubsection{Speedup Online Query}
\label{speeduponline}

Note that, the performance of Algorithm~\ref{alg:onlinequery} is affected by the online collecting gate vertices and online reachability checking.
To address this issue, two techniques are proposed to avoid fully online processing and eventually speedup the query.
For each vertex, the first method, namely gate materialization, is to explicitly record the gate vertices within $\epsilon$ steps away (precompute Line 1 in Algorithm~\ref{alg:onlinequery}).
The second method is to reduce the times of pairwise reachability checking by incorporating quick rejection idea from GRAIL~\cite{} (speedup Line 2 to 8 in Algorithm~\ref{alg:onlinequery}).


{\bf Gate Materialization: }
Two strategies are considered in this method: full gate materialization and partial gate materialization.
In the first strategy, for each vertex $u$, we perform local BFS within $\epsilon$ steps to collect $N^{out}_\epsilon(u)$ and $N^{in}_\epsilon(u)$.
The basic idea of partial gate materialization strategy is that, instead of storing all vertices' local gate vertex set, we only explicitly record some vertices' local gate vertex set, where their gate vertices' size is no larger than certain value.
Especially, given a threshold $k$, we only collect vertex $u$'s $N^{out}_\epsilon(u)$ and $N^{in}_\epsilon(u)$ if  $|N^{out}_\epsilon(u)| \le k$ and $|N^{in}_\epsilon(u)| \le k$.
For remaining vertices, we still apply online collection process.

{\bf Pruning Strategy: }
This method is motivated by the pruning technique introduced in GRAIL~\cite{}.
In GRAIL, each vertex $u$ is assigned with a list of intervals $L_u$ generated by randomized DFS labeling.
To answer the reachability query from $s$ to $t$, they utilize refined DFS based on assigned intervals to reduce search space.
Especially, during search procedure, we say vertex $v$ can be expanded if and only if $L_t \subseteq L_v$.
Otherwise, we immediately conclude that $v \nrightarrow t$ and avoid the further DFS traversal from $v$.
Borrowing this idea, we assigned each gate vertex a list of intervals by randomized DFS labeling on gate graph.
For each pair of gate vertices $(x,y)$ ($x\in N^{out}_\epsilon(s)$ and $y \in N^{in}_\epsilon(t)$), we first check whether $L_y \subseteq L_x$.
If not, we do not need to perform DFS on gate graph to check their reachability.
Therefore, only gate vertex pair $(x,y)$ with $L_y \subseteq L_x$ will be checked by DFS.
A good DFS labeling can generate effective labeling list and help us considerably reduce the number of gate vertex pairs checking by DFS.


\section{Gate Graph Indexing and Reachability Querying}
\label{gateindexing}

Online query procedure actually offers a general search framework based on gate graph.
Its query performance highly depends on how to check reachability between a pair of gate vertices (Line 4 in Algorithm~\ref{alg:onlinequery}).
We know that many literatures have proposed different graph indexing schemes to improve the efficiency of query procedure.
Here, we utilize them to generate reachability index for each gate vertex in the gate graph.
Basically, two categories of algorithms are considered: 1) tree-based approaches, such as tree cover and path-tree;
2) hop-based approaches, such as 2hop.
Besides that, the corresponding querying procedure and some speedup strategies are also presented.
More importantly, we will introduce a scalable 2hop algorithm to handle large graphs in an efficient way.
Note that, since the reachability on ``local'' vertex pairs can be efficiently answered by local BFS under smaller value of $\epsilon$,
we concentrate on addressing the reachability query on ``non-local'' vertex pairs.


\subsection{Tree-based Indexing}
\label{treeindexing}

As the basic ideas of tree cover indexing and path-tree indexing algorithm have been well surveyed in the related work,
we directly go to the query processing.
The most straightforward way is to apply query algorithm used in tree-based approaches to replace DFS search in Algorithm~\ref{alg:onlinequery}.
To further speedup the query efficiency, we will consider the reachability from set viewpoint,
i.e., from gate vertex set $N^{out}_\epsilon(s)$ to gate vertex set $N^{in}_\epsilon(t)$ instead of each pair of vertices.


\input{Figures/TreecoverQuery.tex}

\noindent{\bf Tree Cover: }
The query procedure is outlined in Algorithm~\ref{alg:treecoverquery}.
Firstly, we sort the intervals associated with local gate vertex sets based on interval's first value.
If one interval $[a,b]$ of $u$ is contained by another interval $[c,d]$ of $v$, the interval $[a,b]$ can be removed during sorting,
because the vertices which can be reached by $u$ are guaranteed to be reachable from $v$.
Also, the intervals of vertices $I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$ are sorted similarly.
Given this, we linearly scan those two interval lists to see if there is one interval from $I_s$ containing one interval from $I_t$.
If so, we say $s$ can reach $t$. Otherwise, vertex $t$ is not reachable from vertex $s$.
The sorting step takes $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$ time
and scanning step takes $O(|N_\epsilon^{out}(s)|+|N_\epsilon^{in}(t)|)$ time.
Therefore, the time complexity of query procedure is $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$.


\input{Figures/PathtreeQuery.tex}

{\bf Path-Tree: }
Each gate vertex $u$ in path-tree is assigned with 3 numbers and also records a list of vertices $L(u)$ which can be reached by $u$ while path-tree cover does not cover it.
To answer the reachability from vertex $u$ to vertex $v$, we need to check whether $u$ can reach $v$ by path-tree cover and whether any vertex $w$ in $L(u)$ can $v$.
An efficient query scheme based on interval tree is proposed in the paper to process each query in $O(\log^2 k)$ time, where $k$ is the number of paths in path decomposition.
Motivated by this method, we consider all vertices $I_s = \cup_{x \in N_\epsilon^{out}(s)} L(x)$ together to construct a ``large'' interval tree $T_s$.
Indeed, this is equivalent to creating a virtual node with all reachability information from $I_s$.
Then, for each vertex $y \in I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$, we can efficiently check whether it can be reached by some vertex from $I_s$ in $O(\log^2(dk))$ time,
where $d= |N_\epsilon^{out}(s)|$ and $k$ is the number of path generated by path decomposition on gate graph.
The time complexity of searching on interval tree is $O(d^\prime  \log^2 (dk))$ since the size of $N_\epsilon^{in}(t)$ is $d^\prime$ and we need to invoke such single query $d^\prime$ times.
Considering the sorting and interval tree building steps together, the running time is $O(d^\prime \log^2 (dk))$ in total.
We describe the procedure in Algorithm~\ref{alg:pathtreequery}.


\subsection{Hop-based Indexing (Scalable 2HOP)}
\label{hopindexing}

2-Hop is most well-known algorithm in this category.
However, due to its high computational and memory cost, it is even hard to apply it for medium sized graph with tens of thousands of vertices.
To deal with this challenge, we introduce a scalable 2hop approach based on bipartite set cover (BSC) framework and still achieve the logarithmic bound.

Before go to solution, we first introduce general concept of bipartite set cover framework.
Let $S$ be the ground set to be covered.
Let $\mathcal{G}=(A\cup B,\mathcal{E})$ be a bipartite graph where an edge in $\mathcal{E}$ connects two vertices from $A$ and $B$, respectively.
Each edge $e$ is associated with a subset $S_e \subseteq S$ and $S = \cup_{e \in \mathcal{E}} S_e$.
Let $\mathcal{X}$ and $\mathcal{Y}$ be subsets of $A$ and $B$, respectively.
Let $\mathcal{G}[\mathcal{X} \cup \mathcal{Y}]$ be the {\em induced} subgraph of $\mathcal{X}$ and $\mathcal{Y}$, i.e., it contains all the edges whose both ends are in $\mathcal{X} \cup \mathcal{Y}$.
Let $\mathcal{E}[\mathcal{X} \cup \mathcal{Y}]$ be the edge set of the induced subgraph $\mathcal{G}[\mathcal{X} \cup \mathcal{Y}]$.
Let $\mathcal{C}(\mathcal{E}[\mathcal{X} \cup \mathcal{Y}])$ be the union of sets covering all its edges, i.e.,
$\mathcal{C}(\mathcal{E}[\mathcal{X} \cup \mathcal{Y}])=\bigcup_{e \in \mathcal{E}[\mathcal{X} \cup \mathcal{Y}]} S_e$
Further, we associate a weight with each vertex $z$ in $A \cup B$, denoted as $cost(z)$.
Given this, the bipartite set cover problem is defined as follows.

\bdefin{\bf (Bipartite Set Cover (BSC) Problem)}
Given the ground set $S$ and a bipartite graph $\mathcal{G}=(A\cup B,\mathcal{E})$, where $S=\cup_{e \in \mathcal{E}} S_e$,
we seek vertex subsets $\mathcal{X} \cup \mathcal{Y}$ ($\mathcal{X} \subseteq A$ and $\mathcal{Y} \subseteq B$) to cover the ground set, i.e., $S=\mathcal{C}(\mathcal{E}[\mathcal{X} \cup \mathcal{Y}])$, with the minimal cost,
$\sum_{z \in \mathcal{X} \cup \mathcal{Y}} cost(z)$.
\edefin

By reducing the classical set-cover problem to BSC, we can prove that the bipartite set covering (BSC) problem is NP-hard.
Now, we transform the minimum 2-hop labeling problem to the simplified version of BSC problem as follows.

Let the ground set $S=TC(G)$, i.e., it contains any vertex pair $(u,v)$ in $G$, such as $u \rightarrow v$.
To cover a pair $(u,v)$ means we can restore their reachability in the labeling scheme.
We construct a bipartite graph $\mathcal{G}=(A\cup B,\mathcal{E})$ for the covering purpose:
a vertex in $A$ corresponds to a tuple: $(u, x_i)$, where $u$ is a starting vertex, $x_i$ is a candidate vertex can be reached from $u$;
a vertex in $B$ corresponds to a tuple: $(y_i, v)$, where $v$ is a destination vertex, $y_j$ is a candidate vertex which can reach $v$.
Given this, for any four vertices, $(u,x_i,y_j,v)$, if $x_i = y_j$,
we will add vertex $(u, x_i)$ to $A$, add vertex $(y_i,v)$ to $B$, and add an edge from the first vertex to the latter one.
In addition, in the edge, we will associate a singleton $\{(u,v)\}$.
Further, we assign a unit cost  to each vertex in the bipartite graph, i.e., $cost(e)=1$.
It is not hard to see that if we can find vertex subsets $\mathcal{X} \cup \mathcal{Y}$ ($\mathcal{X} \subseteq A$ and $\mathcal{Y} \subseteq B$) to cover the ground set, we basically are able to restore transitive closure matrix of graph $G$.
Specifically, we have the following relationship:
{\small
\beqnarr
(u,x_i) \in \mathcal{X} &\Longleftrightarrow&  x_i \in L_{out}(u); \nonumber \\
(y_i,v) \in \mathcal{Y} &\Longleftrightarrow&  y_i \in L_{in}(v). \nonumber
\eeqnarr}

\subsubsection{Bipartite Set Cover Algorithm}
\label{bscalg}

The bipartite set cover can be considered as a special case of set-cover-with-pairs problem~\cite{}.
From the perspective of graph formulation, the input of set-cover-with-pairs (SCP) problem is a complete graph while it is bipartite graph in BSC.
Therefore, we can directly apply the existing greedy algorithm for SCP~\cite{} to the BSC problem.
This greedy algorithm have been proved to yield an $O(\sqrt{N \log N})$ approximation ratio, where $N$ is the cardinality of the ground set $N=|U|$ for cardinality BSC problem.
Since $U=TC(G)$ and $N=|TC(G)|$ in 2-hop labeling problem, the approximation bound can be downgraded to $O(n \sqrt{\log n})$, which is not attractive.

Here, we present a fast greedy algorithm that yields $\frac{2}{1-\alpha}(\ln N+1) $ approximation ratio for our BSC problem. For simplicity, we focus on our special case, where each node has a unit cost and each edge is associated with only a singleton.
Our greedy algorithm works as follows: {\em each time we select a node in the bipartite graph $\mathcal{G}=(A \cup B, \mathcal{E})$ according to our defined criterion, until all the elements in the ground set, i.e.,  all pair shortest distance of $G$ in our HCL problem, have been covered.}
To describe our node-selection criterion, we introduce the following definitions:
Let $U$ be the ground set and $R$ be the set recording the already covered elements: $R\subseteq U$.
Let $S$ be the set of already selected nodes in the bipartite graph and let $\overline{S}$ denote the unused nodes in the bipartite graph, $\overline{S}=(A\cup B) \backslash S$.
Assume at some iteration, node $v$ is to be selected. Let $\mathcal{E}(v)$ be the set of edges in $\mathcal{G}$ adjacent to $v$. Then $\mathcal{E}(v)$ covers a set of elements in $U\backslash R$. We are classify these covered elements on the edges adjacent to $v$ into two parts:
1) one part is immediately covered by selecting $v$;
in other worlds, $v$ will work directly on those already selected nodes in $S$, denoted as $S_{v}$, to cover this part of the elements;
2) the other part is those elements which may be covered in the future when selecting nodes in $Z_{v}$, where $Z_{v}\subseteq \overline{S}$ and each node in $Z_{v}$ is adjacent to $v$.
It is easy to see $|S_{v}|$ is exactly how many new elements will be covered if we select $v$ at step $i$,
and $|Z_{v}|$ is how many new elements will be {\em potentially} covered as a consequence of selecting $v$.
In other words, $|S_{v}|+|Z_{v}|$ is the upper bound of the number of elements which can be covered by selecting node $v$.
In our algorithm, at each iteration, we select node $v$ from $\overline{S}$ with minimum $\frac{1}{|S_{v}|+|Z_{v}|}$.

\input{Figures/greedy.tex}

We describe the entire procedure in Algorithm~\ref{alg:greedyCover}.
This algorithm is proved to produce an $O(\frac{2}{1-\alpha}(\ln N+1))$ approximation bound, formally stated in theorem~\ref{approxbound}.

\bthm
\label{approxbound}
The greedyCover algorithm (Algorithm~\ref{alg:greedyCover}) has\\
$\frac{2}{1-\alpha}(\ln N+1) $ approximation ratio solution with respect to the optimal solution, where $\alpha=\frac{1}{|S|}\sum_{v\in S}\frac{|\Delta_{Z_v}|}{|S_v|+|Z_v|}$.
\ethm

The original 2-Hop labeling algorithm has prohibitive computational complexity $O(n^3|TC(G)|)$~\cite{DBLP:conf/sigmod/JinXRF09}.
Now, we can apply our general BSC solver to deal with the bipartite graph ($\mathcal{G}_0$) generated by $2$-hop.
We note that the greedy algorithm runs in $O(\sum_{u\in V} (|L_{out}(u)|+|L_{in}(u)|))$ steps.
Each step, using the speedup queue technique, assuming we only need visit $k<<|V|$ nodes in the queue, takes $O(k(\log |TC|+|V|))$ time to extract and update the queue.
In addition, maintaining the covered set takes $O(|TC|)$ time. Clearly, the time complexity is much lower than the original $2$-hop approach.

\subsubsection{Query Processing of 2HOP}
\label{2hopquery}

We apply above scalable 2hop labeling on gate graph, and each vertex $u$ will be assigned with a set of vertices $L_{out}(u)$ which can be reached by $u$ and a set of vertices $L_{in}(u)$ which can reach $u$.
The query scheme using both gate graph and 2hop labels is quite similar to query scheme of tree cover approach.
Specifically, to answer the reachability from vertex $s$ to vertex $t$, we first collect local gate vertex sets $N_\epsilon^{out}(s)$ and $N_\epsilon^{in}(t)$.
Then, we sort both sets and linearly scan them to check if there is one vertex $x$ in the path from $s$ to $t$, such that $x \in N_\epsilon^{out}(s) \cap N_\epsilon^{in}(t)$.


\subsection{Label Materialization}
\label{labelmater}

It is not hard to see that both gate materialization and pruning strategy for online query can be applied here to improve graph indexing-based query.
Even through, during the query answering process, we still need to access local gate vertices' labels for reachability checking.
To further improve the query efficiency, we can precollect the labels of each vertex's local gate vertex set and organize them in an appropriate way to facilitate online processing.
However, in most of cases, available memory resource is limited and it is impossible to explicitly record those labels for every vertex.
In this sense, a question is naturally arisen: given memory budget, how to select a set of most ``important'' vertices for precomputation where their computational cost fits into memory budget and overall online query performance will be maximally improved?












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{
This category of algorithms uses the tree-like structure to compress the transitive closure of a DAG.
The representatives include tree cover, dual labeling and path-tree.
Those algorithms need to precompute the transitive closure which becomes memory bottleneck in processing large-scale graphs.
However, gate graph is supposed to be small under the appropriate parameter $\epsilon$,
thus memory issue on computing transitive closure can be omitted.

In these algorithms, a tree-like structure is extracted to compress the transitive closure matrix.
Basically, each vertex is assigned with several integers which is used to maintain reachability information within tree-like structure.
Besides that, each vertex $u$ needs to record a list of vertices $L(u)$ which are reachable from $u$ while their reachability are not covered in tree-like structure.
In contrast to transitive closure covered by tree-like structure, the union of $L(u)$ indicates the uncovered transitive closure.
We apply those methods to build index on gate graph.

\noindent{\bf Tree-based Query }
Instead of online checking reachability of gate vertex pair (Line 4 in Algorithm~\ref{alg:onlinequery}),
we use graph indices to quickly determine whether they are reachable.
The most straightforward way is to directly utilize the existing query methods based on corresponding graph indexing to answer reachability query.
However, it is worthwhile to note that, we actually want to check the reachability from a set of vertices $N^{out}_\epsilon(s)$ to another set of vertices $N^{in}_\epsilon(t)$.
We consider the query processing on two sets in the following.

\input{Figures/TreecoverQuery.tex}

{\bf Tree Cover: }
Each gate vertex is assigned with a pair of numbers (i.e., an interval $[a,b]$).
If gate vertex $u$ can reach gate vertex $v$, the interval of $u$ contains the interval of $v$.
Moreover, each gate vertex $u$ also records a list of vertices $L(u)$ which it can reach in the gate graph and their reachability are not covered in the tree.
Now, for starting vertex $s$, we consider all vertices $I_s = \cup_{x \in N_\epsilon^{out}(s)} L(x) $ together.
Firstly, we sort the intervals attached with those vertices based on their first value.
If one interval $[a,b]$ is contained by another interval $[c,d]$, the interval $[a,b]$ can be removed during sorting,
because the vertices which can be reached by this vertex are guaranteed to be reachable from the one with interval $[c,d]$.
Also, the intervals of vertices $I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$ are sorted similarly.
Given this, we can linearly scan those two interval lists to see if there is one interval from $I_s$ containing one interval from $I_t$.
If so, we say $s$ can reach $t$. Otherwise, vertex $t$ is not reachable from vertex $s$.
The query procedure is outlined in Algorithm~\ref{alg:treecoverquery}.
The sorting step takes $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$ time
and scanning step takes $O(|N_\epsilon^{out}(s)|+|N_\epsilon^{in}(t)|)$ time.
Therefore, the time complexity of query procedure is $O(|N_\epsilon^{out}(s)| \log |N_\epsilon^{out}(s)| + |N_\epsilon^{in}(t)| \log |N_\epsilon^{in}(t)|)$.

\input{Figures/PathtreeQuery.tex}

{\bf Path-Tree: }
Each gate vertex $u$ in path-tree is assigned with 3 numbers and also records a list of vertices $L(u)$ which can be reached by $u$ and path-tree cover does not cover it.
To answer the reachability from vertex $u$ to vertex $v$, we need to check whether $u$ can reach $v$ by path-tree cover and whether any vertex $w$ in $L(u)$ can $v$.
An efficient query scheme based on interval tree is proposed to process each query in $O(\log^2 k)$ time, where $k$ is the number of paths in path decomposition.
Motivated by this method, we consider all vertices $I_s = \cup_{x \in N_\epsilon^{out}(s)} L(x)$ together to construct a ``large'' interval tree $T_s$.
Indeed, this is equivalent to creating a virtual node with all reachability information from $I_s$.
Then, for each vertex $y \in I_t = \cup_{y \in N_\epsilon^{in}(t)} L(y)$, we can efficiently check whether it can be reached by some vertex from $I_s$ in $O(\log^2(dk))$ time,
where $d= |N_\epsilon^{out}(s)|$ and $k$ is the number of path generated by path decomposition on gate graph.
The time complexity of searching on interval tree is $O(d^\prime k \log^2 (dk))$ since the size of $N_\epsilon^{in}(t)$ is $d^\prime$ and we need to invoke such single query $d^\prime$ times.
Considering the sorting and interval tree building steps together, the running time is $O(d^\prime k \log^2 (dk))$ in total.
We describe the procedure in Algorithm~\ref{alg:pathtreequery}.


{\bf Speedup Tree-based Query Processing: }
To improve the query efficiency, we precompute some intermediate results and explicitly record them for online processing.
That is, local gate vertices collection and interval sorting in Algorithm~\ref{alg:treecoverquery},
and local gate vertices collection and interval tree building in Algorithm~\ref{alg:pathtreequery} can be performed beforehand.
Clearly, extra memory is needed to store those intermediate results.
For tree cover, each vertex $u$ needs to record sorted interval list of local gate vertices with size $O(dm)$, where $m=|L(u)|$.
For path tree, each vertex $u$ needs to record the interval tree build on top of local gate vertices with size $O(dk)$.
Furthermore, to fit those extra cost into available memory size, the partial materialization strategy introduced in subsection~\ref{speeduponline} can be applied here.
In other words, only the vertex whose local gate vertex sets' sizes are no greater than certain threshold will be preprocessed.
}




\comment{
To answer second question, a novel method based on two level BFS traversals is introduced.
For each unselected vertices, we will online perform local BFS within $\epsilon+1$ steps and add all vertex pairs which are not covered by existing gate vertices into ground set.
For each vertex $u$, assuming its $\epsilon+1$-neighborhood is $N_\epsilon(u)$,
our goal is to eliminate some vertices $x$ from them such that $(u,x)$ can be covered by existing gate vertices.
Two cases can lead to elimination of vertex $x$: 1) some gate vertices is in the shortest path from $u$ to $x$;
2) some gate vertices $v$ is not in the shortest path $P_{ux}$ but satisfies the condition $d(u,v) \le \epsilon$ and $d(v,x) \le \epsilon$.
The first case can be easily checked by local BFS, while the second case needs extra BFS from observed gate vertex to certain depth.
The entire procedure is described in Algorithm~\ref{alg:partialgset}.
In the algorithm, each vertex $u$ is associated with value $c(u)$ to indicate the closest gate vertex which can reach it.
For $u$'s any $\epsilon+1$-neighbor $x$, if its $c(x)$ is assigned with some value, then case 1 is discovered and vertex pair $(u,x)$ has been covered.
In order to check case 2, we need to perform local BFS from gate vertex to see if some $u$'s $\epsilon+1$-neighbors can be reached within $\epsilon$ steps.
If so, case 2 is observed and certain vertex pair can also be omitted in ground set.

\input{Figures/GroundSetwithPreselection.tex}
}

\comment{
The algorithms in this category employs intermediate hops (i.e., vertex in 2hop and chain in 3hop) to store reachability information.
In these methods, each vertex $u$ is assigned with a list of intermediate vertices $L_{out}(u)$ which it can reach and a list of intermediate vertices $L_{in}(u)$ which is reachable from this vertex.
To answer the reachability from source $s$ to destination $t$,
we perform join operation on $L_{out}(s)$ and $L_{in}(t)$ to check if there is some intermediate hops in the path from $s$ to $t$.
The minimization of total number of intermediate vertices builds on top of set cover framework, which is costly for very large graph.
As mentioned, gate graph is significantly smaller than original one, which is possible to be handled by those algorithms.
We apply hop-based indexing algorithm to assign each vertex two lists of vertices $L_{out}$ and $L_{in}$.

In the following, we discuss how to process queries based on gate graph in 2hop and 3hop schemes, respectively.
Basically, we still need to consider the query processing from source's local gate vertex set to target's local gate vertex set.
Assume we try to answer the reachability from $s$ to $t$.
For 2hop, we first collect local gate vertex sets $N_\epsilon^{out}(s)$ and $N_\epsilon^{in}(t)$.
Then, we sort both sets and linearly scan them to check if there is one vertex $x$ in the path from $s$ to $t$, such that $x \in N_\epsilon^{out}(s) \cap N_\epsilon^{in}(t)$.

For 3hop, we introduce our method in high-level by following the idea of query processing proposed in~\cite{}.
Let us assume the local gate vertex sets $N_\epsilon^{out}(s)$ and $N_\epsilon^{in}(t)$ have been extracted.
As we know, chain generated by graph decomposition is used as intermediate hop to serve the communication between source and destination,
as highway in the transportation system.
To tell if vertex $s$ can reach vertex $t$ in the graph, our query scheme generally consists of three steps:

\noindent 1) we collect the entry points $X$ on intermediate chains which can be reached by $s$ through its local gate vertex set;

\noindent 2) we collect the exit points $Y$ on intermediate chains which can reach $t$ through its local gate vertex set;

\noindent 3) we check if there is a pair $(x,y)$ such that $x \in X$, $y \in Y$ and $x$ can reach $y$ in one chain. If so, we say $x \rightarrow y$.
Otherwise, $y$ is not reachable from $x$.

The algorithm is quite similar to the 3hop contour query processing algorithm stated in the original paper.
The difference is that each entry point $x \in X$ is the smallest vertices in its chain which can be reached by all vertices in $N^{out}_\epsilon(s)$ through their out-anchor vertex
instead of only source $s$.

\subsection{Improvement on Indexing-based Query}
\label{improveindexquery}

Clearly, local gate vertex sets can be precomputed and stored to improve the performance of online processing by sacrificing some memory cost.
Another question is that do we need to broadcast the indices of local gate vertex set as well?
That is, for each vertex $u$, should we explicitly record all indices of local gate vertices instead of only gate vertices?
Supposing any pair of vertices has equal probability to be queried,
our goal is to select a set of vertices whose online cost is most expensive and precomputation can significantly improve their query performance.
To proceed, we first define an unified measure to evaluate the saving of each vertex achieved by precomputation as follows.
\beqnarr
S(u) = \sum_{x \in TC(u)} N^{in}_\epsilon(x) \nonumber
\eeqnarr
}

\comment{
Most of indexing based approaches cannot handle very large graph due to their large index size or even the size of transitive closure needed for index construction.
Although we are able to overcome those questions by storing them into disks, the I/O cost for reading indices from disk might considerably affect the performance of query processing.
Our goal here is to scale reachability indexing algorithms for very large graphs without sacrificing the query efficiency.
In this section, we propose a unified reachability computation framework based on graph simplification and graph indexing to address scalability issue in large-scale graphs (with up to tens of millions of vertices).
In addition, some useful strategies are provided to flexibly balance the index size (memory usage) and query performance.
We will conduct comprehensive empirical study on the trade-off between index size and query efficiency.


\subsection{Overview of Computation Framework}
\label{overview}

The computation framework mainly consists of three components: graph simplification, reachability indexing and query processing (illustrated in Figure~\ref{fig:framework}).
The graph simplification component serves as preprocessing step for subsequent procedure.
It aims at extracting a high-level topological view of original graph while preserving essential reachability information.
In other words, the high-level topological view, namely gate graph, is able to recover the reachability between any pair of vertices in the original graph.
The second component is reachability indexing with the goal of building indices for each vertex to facilitate the reachability query answering.
Generally, each vertex is assigned with a set of labels and whether one vertex can be reached by another one is determined by their corresponding label sets.
Given the gate graph and graph indices, we are able to answer the reachability queries in query processing component.
Note that, even without graph indexing, we still can answer reachability queries purely based on gate graph.
Clearly, though the performance of purely online search is not good as the one on top of graph indexing, the memory bottle is completely removed.

Our computation framework is very flexible, such that most of existing reachability indexing methods, like tree cover, pathtree, 2hop and 3hop can be incorporated.
Aside that, by specifying the parameter in graph simplification component,
we are able to control the size of gate graph which eventually influences the resulting index size in graph indexing step.
To speedup the query processing using available memory size,
for some vertices, we adopt partial materialization strategy to explicitly record intermediate results from their close neighbors.
The details will be discussed later.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/Framework.eps,scale=0.5}
\end {tabular}
\caption {Overview of computation framework}
\label{fig:framework}
\end{figure}

\subsection{Notation}
\label{notation}
}




==> MultiTree.tex <==
\section{Multi-Tree Indexing}

In this section, we further push the limit of tree-based indexing. 
In the last section, we have presented a double-tree index method which can further reduced the size of {\em compressed transitive closure} produced from a single tree. 
However, the compression capacity is determined by the two trees and  the  query time is compromised. 
Given this, we develop a {\em multi-tree index} scheme which can apply multiple trees to compress the transitive closure. 
In addition, the query performance of the new index can always be faster than  the single tree index. 

\subsection{Basic Ideas of Multi-Tree Index} 
\label{basic}
The basic idea of the multi-tree index is based on the following observation: 
suppose there are multiple spanning trees $T_1$, $T_2$, $\cdots T_k$ in DAG $G$, for a given vertex $u$, it has also different compressed transitive closure (successor sets), such as $succ(u|T_1)$, $succ(u|T_2)$, $\cdots$, $succ(u|T_k)$. 
Thus, we can simply assign vertex $u$ to the tree $T_i$, which has the minimal compressed transitive closure, i.e., 
$T_i=\arg\min_{1\leq i \leq k} |succ(i|T_1)|$. 
Clearly, using multiple tree can reduce the cost of compressed transitive closure. 
However, the downside is that we have to pay the extra cost of the interval labeling for each additional tree. 

To better understand the tradeoff between the reduced size of the compressed transitive closure and the extra cost of using additional trees, let us draw an analogy between the multi-tree index scheme and  statistical model fitting~\cite{}. 
Recall that in the well-known {\em Minimal Description Length} (MDL) principle, we study how data $\mathcal{D}$ can be best  represented using statistical model $\mathcal{M}$. 
Here, the overall model complexity is based on the the cost of using the model to represent the data, denoted as $L(\mathcal{D}|\mathcal{M})$ plus the complexity of model itself $L(\mathcal{M})$. 
The MDL is the one which minimize the summation of these two costs. 
In the multi-tree indexing scheme, the compressed transitive closure of each node corresponds to how each data point fits the given model. 
In other words, the total cost of compressed transitive closure is simply the  cost of data representation based on the model $L(\mathcal{D}|\mathcal{M})$. 
Specifically, for each vertex $u$, let $C_u=\min_{1\leq i \leq k} |succ(i|T_1)|$, and thus the total labeling cost, denote as $L_1$, is $\sum_{u \in V} C_u$. 
Then, the interval labeling cost of the trees, denoted as $L_2$, is the complexity of the model $L(\mathcal{M})$. 
Specifically, if we have $k$ trees, the labeling cost $L_2=2 k N$, where $N$ is the number of vertices in $G$. 
Given this, the optimal multi-tree indexing scheme is to search for the optimal $k$ trees such that $L_1+L_2$ is minimized. 

How to determine the number of trees is needed for the indexing is a hard question. In the following, we first focus on the following questions: 
for a fixed number $k$, discover the optimal $k$ trees which can minimize the total cost of compressed transitive closure ($L_1$ costs). 
To solve this problem, we propose an iterative algorithm which can guarantee to converge to a local minimum. 
The algorithm performs in a $k$-means fashion and therefore we refer to it as {\em $K$-Tree } algorithm. 
It starts with $k$ trees (they can be random chosen, or constructed by heuristics). 
Then, we assign each vertex $u$ in graph $G$ to their closest match, i.e., the tree $T_i$ with the smallest compressed transitive closure. 
Thus, we partition the vertices in $G$ into $K$ groups, $V_1$, $V_2$, $\cdots V_K$. 
Then for each group $V_i$, we construct the new optimal tree $T_i^\prime$ which can minimize the total compressed transitive closure of all vertices in the group, i.e., $\sum_{v \in V_i} succ(v|T_i^\prime)$.  
We repeat this process until further reduction of the total compressed transitive closure size: $\sum_{i=1}^K \sum_{v \in V_i} succ(v|T_i^\prime)$. 

\input{Figures/KTree.tex}

The correctness of this algorithm is determined by the following theorem. 
\bthm{(\bf Convergence)}
Let $T_1^j$, $T_2^j$ $\cods T_k^j$ be the tree constructed in the $j$-th iteration. 
Then, we have 
\beqnarr 
\sum_{i=1}^K \sum_{v \in V_i} succ(v|T_i^j) \geq \sum_{i=1}^K \sum_{v \in V_i} succ(v|T_i^{j+1}) \nonumber 
\eeqnarr
\ethm

The computational complexity of this algorithm is $O(LKMN)$, where $L$ is the number of iterations. 
This is because at each iteration, we have to compute $succ(u|T_i)$ ($1 \leq i \leq K$) for each vertex $u$, which can take up to $O(MN)$ for each tree.  Thus the total cost for $K$ tree is $O(KMN)$. 
In addition, we have to construct the optimal tree cover for the $K$ groups and this takes up to $O(\sum_{i=1}^{K} MV_i)=O(MN)$ time. 
Thus the total cost is in the order $O(LKMN)$. 

\subsection{Scalable Implementation}
\label{scalableMulti}

1. How to apply sampling for tree generation?
To reduce the computational cost, we use a set of samples. 
Clearly, we may randomly choose nodes in the graphs and apply those nodes to sample. 
For any node, if its $|succ(u|S)|$ is large, we should extract those points out as the main target to reduce their costs. 
The most $succ(u|S)$, we consider to reduce them
2. How to decide the initial trees? 
3. A partial computation procedure for $pred()$. Or $|succ(u|S)|$. 


==> Scalable.tex <==
\section{Scalable Tree Cover Construction}
\label{scalable}

In this section, we will solve the first problem: how we can construct an optimal tree cover which can handle very graphs with millions of vertices. 
The main goal is that as long as the index size of the tree cover can be held in the main memory, we should be able to construct the index. 
When the index size exceeds the memory size, we can still generate the index on the disk. However, its query performance will become to slow and even worse than the online search scheme. 
Thus, in this section, our goal is to push the boundary of optimal tree cover. 
In addition, the technique developed in this section can also be applied to other methods, such as path-tree in the first category, and for the methods we will develop to further compress the index size produced by the tree cover. 

\subsection{Preliminary: Optimal-Tree Cover Construction}

\input{Figures/OptimalTreeCover.tex}
To proceed, let us first revisit the optimal tree cover approach introduced in ~\cite{}. 
Here, we assume that all vertices without predecessors are connected to a virtual root. 
First, for each vertex, we compute all its predecessors $pred(v)$, which contains all the vertices which can reach $v$ (including itself). This is essentially the classical fast transitive closure computation~\cite{}, which produce the predecessor sets of each vertex iteratively following the topological order. 
Then, for each edge $e=(v^\prime,v)$, we assign an edge weight, which is the size of $v$'s predecessor set.
Finally, the optimal tree cover is to select the incoming edge of the maximal weight for each vertex $v$, and thus the maximal spanning tree of the DAG based on the weight assignment ~\cite{}. 

To see why this method can produce the optimal index size, let us look at the {\em compressed transitive closure} of $G$ of a tree $T$. 
Given a tree $T$, the transitive closure for each vertex $u$ ($u$'s successor) of $G$ can be organized into pair-wise disjoint subtrees, and then each subtree can be represented by only its root vertex. 
In other words, the compressed transitive closure of $u$ records only those vertices which $u$ can reach but without any of their corresponding ancestors in the tree. 
Given this, we can see that if any vertex $v$ has an immediate successor $v^\prime$ in the tree, then the predecessors of $v^\prime$ $(pred(v^\prime))$ will not record $v$ in their compressed transitive closure ($v^\prime$ is the ancestor of $v$ in the tree).
However, all the predecessors of $v$ except those of $v^\prime$, i.e.,  $pred(v) \backslash pred(v^\prime)$, have to record $v$. 
Thus, we can see the size of the compressed transitive closure ($TC_c$) is equal to the number of those predecessors, i.e. ,
{\small
\beqnarr
|TC_c| &=& \sum_{(v^\prime,v) \in E_T} |pred(v) \backslash pred(v^\prime)| ~~~~(pred(v^\prime) \subseteq pred(v)) \nonumber \\
  &=&  \sum_{(v^\prime,v) \in E_T} |pred(v)| - |pred(v^\prime)| =  |TC| - \sum_{(v^\prime,v) \in E_T} w_e \nonumber 
\eeqnarr}
Based on this equation, we can see that maximal weighted spanning tree of $G$ can minimize the  the compressed transitive closure $TC_c$. 

Given this, we can see that even though the compressed transitive closure is very small (much smaller than the $TC$), in order to generate optimal tree cover, we still have to compute the complete predecessor ($TC$) sets in Algorithm~\cite{}. 
In addition to the computation cost, the memory cost to materialize $TC$ is also very expensive. 
For most of the construction stage, the $TC$ is often run out of the main memory in the first stage and thus is the leading reason for constructing tree index for large graphs. 
We note that a simple modification to reduce the memory cost is to drop the predecessor set of a vertex $v^\prime$ once all the predecessors of its immediate successors in $G$ has been computed and we only needs to record it cardinality $|pred(v^\prime)|$ instead.
However, such solution does not reduce the computational cost and its memory cost can still be too large to be scalable. 


\subsection{Removing Memory Bottleneck}

In the following,  we first introduce a method which can help remove the memory bottleneck of the tree cover algorithm. 
Later, we will built on top of this method to further handle the computational cost. 
The basic idea we will explore is to instead of computing the entire predecessor set of each vertex at the same time for edge weight $w(v^\prime,v)$, 
we will decompose $w(v^\prime,v)=|pred(v)|$ into the sum of individual vertex's own contribution. 
This is because our target is the total cardinality of $pred(v)$ not the set itself. 
 
Now, we introduce a basic notation {\em conditional transitive closure} which allows to decompose the entire transitive close into disjoint subsets: 
 
\bdefin{\bf (Conditional Transitive Closure) }
Given DAG $G=(V,E)$ and any vertex subset $S$, the conditional transitive closure of vertex $v$ based on this set 
is denoted as 
\beqnarr
pred(v |S) = pred(v) \cap S
\eeqnarr
\edefin

The conditional transitive closure provides the basic tool to handle the predecessor sets through decomposition, and thus to compute its cardinality $|pred(v)|$ from individual parts: 

\blemma
\label{summation}
For any vertex set decomposition, $V_1$, $V_2$, $\cdots$, $V_K$, such that $V_1 \cup V_2 \cup \cdots V_K=V$ and $V_i \cap V_j=\emptyset$, then, 
\beqnarr
|pred(v)|=\sum_{i=1}^{K} |pred(v|V_i)|
\eeqnarr
\elemma

This lemma serves as the foundation to construct the scalable optimal tree cover. 
The first implication is that we can decompose the vertex set into disjoint groups $V_1$, $V_2$, $\cdots$, $V_K$; process each group independently to get $|pred(v|V_i)|$ for each vertex; and then aggregate individual group contribution to produce the overall edge weight $w(v^\prime,v)=|pred(v^\prime)|$ .
Since we can control the cardinality of each subset $|V_i|$ (typically between hundreds to thousands), we can effectively remove the memory bottleneck for computing the optimal tree cover. 
The memory bound is reduced from $|TC|$ to $\max (\sum_v |pred(v) \cap V_i|)\approx |TC|/K$ where $K$ can be set up to be $|V|$. 

The sketch of this computing procedure without memory bottleneck is outlined in Algorithm \ref{alg:mptree}.
We first randomly partition all vertices in graph $G$ into $K$ equal size groups (Line $1$). 
Then, we will compute the conditional transitive closure for each group $V_k$, $1 \leq k \leq K$ (Line  $2-4$). 
Specifically, for each group $V_k$, we will invoke the {\em ConditionalTC} procedure to  compute $pred(v|V_k)$ for each vertex $v$ in the graph. It is very similar to the full predecessor set computation in Algorithm~\ref{alg:opttreecover} except we only put vertices in the active group $V_k$ into consideration (Line $2-6$). 
If a vertex is not currently in $V_k$, it will not appear in any predecessor set in the current batch. 
Finally, when the entire conditional transitive closure is available, we will apply them to update the edge weight (Line $11$-$13$, Lemma~\ref{summation}). 
Thus, we all the groups are processed, the exact edge weight $w(v^\prime,v)=|pred(v^\prime)|$ has been calculated, and we can then compute the maximal spanning tree to get the optimal tree cover for $G$. 


\input{Figures/MPTree.tex}




The memory requirement of this algorithm has reduced to $O(n g)$ where $g$ is the group size $n/K$ from $O(TC)$ (worst case $O(n^2)$) in the original optimal tree cover algorithm (Algorithm~\ref{alg:opttreecover}).  
Especially, we can set the group size to be a constant (around thousands) and thus can easily handle graphs with millions of the vertices. 
However, it still takes $O(\sum_k m|V_k|)=O(mn)$ time complexity which is the same as Algorithm~\ref{alg:opttreecover}.  
This is clearly too time consuming for large graphs. 
To speedup the construction time, in the following, we consider the extract a tree cover which can compress the transitive closure very close to the optimal tree with high probability. 
At high level, we will random sample $s$ groups out of the all $K$ groups to produce an approximate tree whose total edge weights are close to the optimal one. 
The empirical study show that using very few groups ($s \ll K$) we can discover a very good tree cover and this thus leads to significant improvement of computational efficiency.

\subsection{Fast Approximate Optimal Tree} 
The quality of an approximation optimal tree is defined as follows. 
Let $T_o$ be the optimal tree cover discovered in Algorithm~\ref{alg:opttreecover} (and ~\ref{alg:mptree}). 
The total weight of a tree $T$ is denoted as $W(T)=\sum_{(v^\prime,v) \in E(T)} w(v^\prime,v)$. 
Given a DAG $G$,  an $(\epsilon,\delta)$ {\bf approximate optimal tree} $T_a$ is the one with high probability (at least $1-\delta$) such that the relative difference between its total weight $W(T_a)$ and the true optimal tree weight $W(T_o)$ is very close (no greater than $\theta$):
\beqnarr
\label{approxrt}
Pr(\frac{W(T_o) - W(T_a)}{W(T_o)} \le \theta) \ge 1-\delta
\eeqnarr

In order to solve this problem, we need to use samples and probability inequality to actually estimate (and bound) $W(T_o)$, and $W(T_a)$ accurately.
Recall for each edge  $e=(v^\prime,v)$, the edge weight $w_e=|pred(v^\prime)|=\sum_{u \in V} |pred(v^\prime|u)|$. 
Also let $y_u(T)=\sum_{e=(v^\prime, v) \in E_T} |pred(v^\prime|u)|$, which records the cardinality of $u$'s successor set, i.e., those vertices record $u$ as one of their predecessors.
For any tree $T$, its total tree weight $W(T)$ is 
\beqnarr 
W(T)&=&\sum_{e \in E_T} w_e = \sum_{e=(v^\prime, v) \in E_T} \sum_{u \in V} |pred(v^\prime|u)| \nonumber \\
        &=&\sum_{u \in V}  \sum_{e=(v^\prime, v) \in E_T} |pred(v^\prime|u)| \nonumber \\ 
& & \mbox {let } y_u(T)=\sum_{e=(v^\prime, v) \in E_T} |pred(v^\prime|u)| \nonumber \\
         &=& \sum_{u \in V} y_u(T) 
\eeqnarr 
If we have $n$ sample vertices in $S=\{v_1, v_2, \cdots, v_n\}$, 
we can apply the following estimator for  $W(T)$: 
\beqnarr 
\hat{W}(T)=\frac{\sum_{u \in S} {y_u(T)}}{n} \times N  
\eeqnarr

It is very easy to see that $\hat{W}(T)$ is an unbiased estimator, i.e., 
\beqnarr 
E(\hat{W}(T))=N/n  E(\sum_{u \in S} {y_u(T)})=N (\sum_{u \in V} y_u(T)/N)=W(T) \nonumber
\eeqnarr
In addition, since each $y_u(T)$ is bounded between $0$ to $N$, the direct application of Hoeffding bound can get 
\beqnarr
Pr((|\frac{\hat{W}(T)}{N}-\frac{W(T)}{N}| \geq \epsilon_1 N) \leq \delta_1,  \mbox{ where } \delta_1=2e^{- 2 \epsilon_1^2 n}
\eeqnarr 
Thus, the in order to achieve $(\epsilon_1,\delta_)$ approximation for the tree weight, we need approximately 
$n=\frac{1}{2\epsilon_1^2} \ln {\frac{2}{\delta_1}}$ samples. 
For instance, for $\epsilon$ to be $1\%$, and $\delta_1=1\%$, then we approximately need $n=26491$ vertices. If we want to make $\epsilon_1$ even smaller, the sample size can also increase rather shaply (inverse to the square of $\epsilon_1$).  
To address of this problem, we may apply more accurate probabilistic bound (Hoeffding bound is a very loose bound).
For instance, we apply the Central Limit Theorem~\cite{}, we can achieve a much accurate bound and thus the sample size can be reduced significantly:   
\beqnarr
Pr(|\frac{\hat{W}(T)}{N}-\frac{W(T)}{N}| \geq \epsilon_1 N) \approx O(e^{-\frac{n \epsilon_1^2 N^2}{2 \sigma^2}})
\eeqnarr
where, $\sigma^2\approx \frac{1}{n-1}\sum_{u \in S} (y_u(T)- \hat{W}(T)/N)^2$. 

Given this, we can determine whether the weight of the maximal spanning tree discovered so far based on the sample set is close enough to the weight of the optimal spanning tree:  
\bthm
\label{condtheorem}
Given $n$ sampling vertices in $S$, let $T_a$ is the maximal weighted spanning tree discovered using sampling (here the approximate edge weight is denoted as $\hat{w}_e=(\sum_{u \in S} pred(v|u)) \frac{N}{n}$, 
if the following condition is satisfied then $T_a$ is an $(\epsilon,\delta)$ approximate optimal tree: 
\beqnarr
\label{condition}
\frac{2\epsilon_1 N}{\hat{W}(T)-\epsilon_1 N} \leq \epsilon, \nonumber
\mbox{ where } \epsilon_1=\sqrt{\frac{1}{2n} \ln \frac{2}{\delta_1}}, and \delta_1=\delta/2 \nonumber \\
\Longrightarrow Pr(\frac{W(T_o) - W(T_a)}{W(T_o)} \le \theta) \ge 1-\delta \nonumber 
\eeqnarr
\ethm

The correctness of Theorem~\ref{condtheorem} follows our discussion on the Hoeffding inequality and it proof is omitted for simplicity. If we apply CLT, then each tree can have different error bound. In this case, a technique developed in ~\cite{} can be used to handle such situation. 
To implement the sampling technique, in Algorithm~\ref{alg:mptree}, instead of visiting every group, we just need to visit a few of them. 
Specifically, after each invoke of {\em ConditionalTC}, we apply the test criteria in Theorem~\ref{condtheorem} to determine whether the approximate optimal tree is discovered. 
We continue visiting next group until $T_a$ is found.  
We note that this algorithm has the same memory requirement as Algorithm~\ref{alg:mptree} (thus no memory bottleneck) while its computational complexity has been reduced to $O(Mn)$ where the sample size $n \ll N$ (Section ~\cite{expr}).
 

\comment{
\bproof
If $2e^{2nt^2} \le \delta$, we have
\[ 1 - \delta \le 1 - 2e^{2nt^2}  \]
In addition, from the Chernoff-Hoeffding bound, we have
\[ Pr(W(T^{-1}_o) - W(T^{-1}_o) \le nt) \ge 1 - 2e^{-2nt^2}  \]
\[ Pr(W(T^{-1}) - W(T^{-1}) \le nt) \ge 1 - 2e^{-2nt^2}  \]
By definition, we have
\[ W_n(T^{-1}_o) \le W_n(T^{-1}) \mbox{ and } W(T^{-1}_o) \ge W(T^{-1}) \]
Putting those together, we have
\[ Pr(W_n(T^{-1}) - nt \le W(T^{-1}) \le W(T^{-1}_o) \le W_n(T^{-1})+nt) \ge 1 - 2e^{-2nt^2} \]
Hence, the following inequalities hold:
\beqnarr
Pr(W(T^{-1}_o) - W(T^{-1}) < 2nt) \ge 1 - 2e^{-2nt^2} \\
Pr(W_n(T^{-1}) - nt \le W(T^{-1}_o)) \ge 1 - 2e^{-2nt^2}
\eeqnarr
In this sense, if $\frac{2nt}{W_n(T^{-1})-nt} \le \theta$, with the probability of $1 - 2e^{-2nt^2}$, we have
\[ \frac{W(T^{-1}_o) - W(T^{-1})}{W(T^{-1}_o)} \le  \frac{2nt}{W_n(T^{-1})-nt} \le \theta \]
That is, combing with $1 - \delta \le 1 - 2e^{2nt^2}$, the following inequality holds:
\[ Pr(\frac{W(T^{-1}_o) - W(T^{-1})}{W(T^{-1}_o)} \le \theta) \ge 1 - 2e^{2nt^2} \ge 1-\delta  \]
\eproof}



\comment{ 
However, it is still time consuming such that we have to perform the computation of partial transitive closure $K$ times,
where $K$ is the number of non-overlapping vertices groups.
Here, we propose an efficient method to generate approximate double tree utilizing sampling technique.
The method is motivated by the {\em law of large number} which describes the result of performing the same experiment a certain number of times.
According to the law, if we repeat the same trail in many times, the average result obtained from those experiments is getting closer to the expected value as the increase of number of trails.

The basic idea of our method is to randomly sample $n$ groups out of all $K$ groups to generate the double tree whose total edge weights are close to the optimal one.
The empirical studies will show that the approximate double tree is reasonable good even with small sample size $n \ll K$.
This eventually leads to the significant improvement of computational efficiency.
The double tree construction using sampling technique is outlined in Algorithm \ref{alg:sampling}.
The algorithm is quite similar to the batch processing method.
The only different thing is that we only process the groups which are randomly sampled from $K$ non-overlapping partitions.}


%\input{Figures/MultiSamplingTree.tex}







 





\comment{
Given DAG $G=(V,E)$ and vertex $u \in V$, for each vertex $v \in V$, the conditional predecessor $pred(v|u)$ denotes whether $u$ can reach $v$.
If it is reachable, $pred(v|u) = \{u\}$, otherwise, $pred(v|u) =\emptyset$.
In other words, $pred(v|u)=pred(v) \cap \{u\}$. 
Given this, the transitive closure of vertex $v$ is the union of its all conditional transitive closure, i.e., 
\beqnarr
pred(v)= \bigcup_{u \in S} pred(v|u) 
\eeqnarr
Further, for any vertex subset $S$, the conditional transitive closure of vertex $v$ based on this set 
is denoted as 
\beqnarr
pred(v |S) = \bigcup_{u \in S} pred(v | u) = pred(v) \cap $S$
\eeqnarr
\edefin

The conditional transitive closure provides the basic tool to handle the predecessor sets through decomposition, and thus to compute its cardinality $|pred(v)|$ from individual parts: 

\blemma
\label{summation}
For any vertex set decomposition, $V_1$, $V_2$, $\cdots$, $V_k$, such that $V_1 \cup V_2 \cup \cdots V_k=V$ and $V_i \cap V_j=\emptyset$, then, 

\beqnarr
For a vertex $v$, each of its conditional transitive closure based on individual vertex is disjoint and thus  
\benqarr
|pred(v)|=\sum_{u \in V} |pred(v|u)|   \nonumber 
\eeqnarr
Further, given any two disjoint vertex sets $S_1$ and $S_2$ ($S_1 \cap S_2 =\emptyset$), then, 
\beqnarr
|pred(v | S_1 \cup S_2)|=|pred(v|S_1)| \cup |pred(v|S_2)|\]
\eeqnarr
For any vertex set decomposition, $V_1$, $V_2$, $\cdots$, $V_k$, such that $V_1 \cup V_2 \cup \cdots V_k=V$ and $V_i \cap V_j=\emptyset$, then, 
\beqnarr
\eeqnarr 
\elemma
}



==> uniform.tex <==
\section{the Uniform Framework of Reachability Query}

Any scheme to answer reachability query can be regarded as a set cover approach: Given a DAG $G$, let's define $<x,y>$ to be a reachability pair of vertices that vertex $x$ can reach vertex $y$. Then the transitive closure of our DAG $G$ can be viewed as a full set of reachability pairs, which we name as $RP$ where $RP=\{<x,y>| x\rightarrow y$ in $G$ $\}$. If some graph structure $\Lambda$, e.g. a path or a tree, answers reachability queries between some vertices, then we can say $\Lambda$ covers a subset of $RP$. 

In order to propose an effective scheme to answer reachability query, we would like to first find out how efficient available schemes are. Here our "effective" and "efficient" mostly refer to the index size. Therefore, we define cover efficiency of a graph structure $\Lambda$ to be the number of elements (reachability pairs) it can cover in $RP$ over the index size of $\Lambda$. We will consider the cover efficiency in best case, average case and worst case.

{\bf Path decomposition:} Given a path of $n$ vertices, it can cover $\frac{n(n-1)}{2}$ reachability pairs. The standard index size of a path is $2n$ (Each vertex has a vertex id and a path id) if query time is $O(k)$ ($k$ is the number of paths in path decomposition). Therefore, the cover efficiency of a path is $\frac{n-1}{4}$. However, a path decomposition has $k$ paths. If each path has the same number of vertices, then the $k$ paths cover $\frac{n(\frac{n}{k}-1)}{2}$ reachability pairs, and the cover efficiency is $\frac{\frac{n}{k}-1}{2}$.

{\bf tree cover and its variations:}  Given a tree of $n$ vertices, it can cover $\frac{n(n-1)}{2}$ reachability pairs if the tree is a path in one extreme case. In another extreme case when the tree is a complete binary tree it can cover $[\log_2(n+1)-2](n+1)-2$ reachability pairs. Trees are index by assigning each vertex an interval therefore the index size of trees are $2n$.

{\bf 2-hop cover (bipartite graph cover):} It's easy to show that a 2-hop cover is essentially a bipartite graph cover, i.e. a set of bipartite graph relationships that covers $RP$. Given a $a\times b$ bipartite graph, it covers $ab$ reachability pairs. By 2-hop its index size is $a+b$ and its cover efficiency is $\frac{ab}{a+b}$. When $a=b=n$ the cover efficiency of the bipartite graph is $\frac{n}{2}$.

 
